Optimization Modulo Theories with Linear Rational Costs

In the contexts of automated reasoning (AR) and formal verification (FV), important decision problems are effectively encoded into Satisfiability Modulo Theories (SMT). In the last decade efficient SMT solvers have been developed for several theories of practical interest (e.g., linear arithmetic, arrays, bit-vectors). Surprisingly, little work has been done to extend SMT to deal with optimization problems; in particular, we are not aware of any previous work on SMT solvers able to produce solutions which minimize cost functions over arithmetical variables. This is unfortunate, since some problems of interest require this functionality. In the work described in this paper we start filling this gap. We present and discuss two general procedures for leveraging SMT to handle the minimization of linear rational cost functions, combining SMT with standard minimization techniques. We have implemented the procedures within the MathSAT SMT solver. Due to the absence of competitors in the AR, FV and SMT domains, we have experimentally evaluated our implementation against state-of-the-art tools for the domain of linear generalized disjunctive programming (LGDP), which is closest in spirit to our domain, on sets of problems which have been previously proposed as benchmarks for the latter tools. The results show that our tool is very competitive with, and often outperforms, these tools on these problems, clearly demonstrating the potential of the approach.

==> TAGS <==

algo_binsearch.tex,1232
\label{algo:binsearch}algo:binsearch4,120
\renewcommand{\varphicost}\varphicost7,167
$ \label{algobin:init}algobin:init15,415
\label{algobin:constraints}algobin:constraints19,607
\WHILE{($\currlb < \currub $ )} \label{algobin:while}algobin:while25,857
   \IF{(\dopivoting{})} \label{algobin:pivoting}algobin:pivoting26,911
   \ENDIF \label{algobin:endpivoting}algobin:endpivoting31,1191
   \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmt(\varphicost)$ \label{algobin:smtsolver}algobin:smtsolver32,1229
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algobin:min}algobin:min34,1362
\label{algobin:add}algobin:add37,1524
      \STATE $\currlb \leftarrow \currub$ \label{algobin:end}algobin:end40,1614
     \STATE $\currlb \leftarrow \pivot$ \label{algobin:lbound}algobin:lbound42,1754
     \STATE $\varphicost \leftarrow \varphicost \setminus \set{\pivotatom}$\label{algobin:poppivot}algobin:poppivot43,1817
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algobin:pushnegpivot}algobin:pushnegpivot44,1920
\label{algobin:endwhile}algobin:endwhile48,2057
\RETURN $\pair{\calm}{\currub}$ \label{algobin:return}algobin:return49,2082

algo_linsearch.tex,759
\label{algo:linsearch}algo:linsearch4,107
\renewcommand{\varphicost}\varphicost7,156
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$ \label{algolin:constraints}algolin:constraints17,432
\WHILE{($\currlb < \currub $)} \label{algolin:while}algolin:while18,534
   \STATE $\tuple{\status,\mu} \leftarrow \incrementalsmt(\varphicost)$ \label{algolin:smtsolver}algolin:smtsolver19,587
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algolin:min}algolin:min22,796
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}$ \label{algolin:add}algolin:add23,885
\label{algolin:endwhile}algolin:endwhile30,1187
\RETURN \pair{\calm}{\currub} \label{algolin:return}algolin:return31,1212

algo_mixsearch.tex,1653
\label{algo:mixsearch}algo:mixsearch4,128
\renewcommand{\varphicost}\varphicost7,176
$ \label{algomix:init}algomix:init19,500
\label{algomix:constraints}algomix:constraints21,597
\WHILE{($\currlb < \currub $ )} \label{algomix:while}algomix:while23,677
   \IF[Binary-search Mode]{(\dopivoting{})} \label{algomix:pivotingcond}algomix:pivotingcond24,731
\label{algomix:initpivoting}algomix:initpivoting25,804
       \pivotatom}$ \label{algomix:addpivot}algomix:addpivot30,1051
\label{algomix:smtsolverone}algomix:smtsolverone34,1216
   \smtcoreextract(\varphicost)$ \label{algomix:smtsolvercore}algomix:smtsolvercore38,1312
\ENDIF\label{algomix:endpivoting}algomix:endpivoting43,1560
   \STATE $\tuple{\status,\mu} \leftarrow \incrementalsmt(\varphicost)$ \label{algomix:smtsolver}algomix:smtsolver46,1626
   \IF{$(\status = \satres)$}\label{algomix:issat}algomix:issat51,1921
      \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algomix:min}algomix:min52,1973
\label{algomix:add}algomix:add56,2243
   \IF{$({\pivotatom \not\in \eta}) $} \label{algomix:unsatcondition}algomix:unsatcondition59,2354
      \STATE $\currlb \leftarrow \currub$ \label{algomix:end}algomix:end60,2424
     \STATE $\currlb \leftarrow \pivot$ \label{algomix:lbound}algomix:lbound62,2564
     \set{\ \pivotatom}$\label{algomix:poppivot}algomix:poppivot64,2688
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algomix:pushnegpivot}algomix:pushnegpivot66,2787
\label{algomix:endwhile}algomix:endwhile71,2976
\RETURN $\pair{\calm}{\currub}$ \label{algomix:return}algomix:return72,3001

algorithms_inline.tex,1923
  \label{fig:algo_inline}fig:algo_inline25,914
Algorithm~\ref{algo:mixsearch}algo:mixsearch54,1857
\ref{algomix:init}algomix:init55,1896
]\currlb,\currub[$, and the (possibly new) atom $\pivotatom\defasas77,2641
mimics steps \ref{algomix:initpivoting}algomix:initpivoting79,2782
in Algorithm~\ref{algo:mixsearch}algo:mixsearch80,2845
mirrors steps \ref{algomix:issat}algomix:issat94,3497
Algorithm~\ref{algo:mixsearch}algo:mixsearch95,3552
scenario\ignoreinshort{\ (see Figure~\ref{fig:algo_inline}fig:algo_inline103,3874
\ref{algomix:lbound}algomix:lbound114,4413
Algorithm~\ref{algo:mixsearch}algo:mixsearch115,4464
Algorithm~\ref{algo:mixsearch}algo:mixsearch120,4642
The same facts \ref{item:approximatesolution}item:approximatesolution134,5245
found, not only $(\cost < \minvalue)$ but also $\pivotatom\defas(\costas(\cost154,6030
(In Algorithm~\ref{algo:mixsearch}algo:mixsearch160,6404
is not popped from \vi before step \ref{algomix:add}algomix:add161,6482
with a simple modification of the algorithm in \cite{demoura_cav06}demoura_cav06183,7232
$C^*\defas\neg\eta\vee\neg(\cost<\currub)$ is used do drive backjumpingas\neg\eta\vee\neg(\cost<\currub)$186,7346
and learning instead of $C\defas\neg\eta\vee\neg\pivotatom$.as\neg\eta\vee\neg\pivotatom$.187,7418
$C_1\defas\neg\eta\vee\neg(\cost<\maxvalue)$ and as\neg\eta\vee\neg(\cost<\maxvalue)$196,7839
$C_2\defas\neg\pivotatom\vee(\cost<\maxvalue)$ are as\neg\pivotatom\vee(\cost<\maxvalue)$197,7889
$C\defas\neg\eta\vee\neg\pivotatom$.as\neg\eta\vee\neg\pivotatom$.199,7992
\label{ex:tightening}ex:tightening213,8484
Consider the formula $\vi\defas\psi\wedge(\cost \ge a+15)\wedge(a\geas\psi\wedge(\cost214,8506
binary-search deciding $\pivotatom\defas(\cost<8)$, the \laratsolveras(\cost<8)$,216,8635
$C\defas as219,8725
$C_1\defasas233,9101
C_2\defas\neg\pivotatom \vee (\cost<15)as\neg\pivotatom240,9177

algorithms_offline.tex,2038
is displayed in Algorithm~\ref{algo:mixsearch}algo:mixsearch9,249
Algorithm~\ref{algo:mixsearch}algo:mixsearch30,1171
the range \currrange (row \ref{algomix:constraints}algomix:constraints50,1776
\ref{algomix:while}algomix:while60,2116
steps \ref{algomix:initpivoting}algomix:initpivoting74,2693
\ref{algomix:lbound}algomix:lbound75,2756
\ref{algomix:smtsolver}algomix:smtsolver80,2892
\ref{algomix:unsatcondition}algomix:unsatcondition95,3453
is added to $\vi$ (row \ref{algomix:add}algomix:add114,4153
condition~\ref{algomix:while}algomix:while117,4302
(steps \ref{algomix:initpivoting}algomix:initpivoting128,4667
the (possibly new) atom $\pivotatom\defas(\cost<\pivot)$ is pushedas(\cost<\pivot)$132,4887
\cite{lynce_unsatcore_sat04}lynce_unsatcore_sat04144,5409
Algorithm~\ref{algo:mixsearch}algo:mixsearch170,6480
(see e.g. \cite{cimattigs11_unsatcore}cimattigs11_unsatcore181,6949
Theorem~\ref{teo:main}teo:main212,8222
Algorithm~\ref{algo:mixsearch}algo:mixsearch221,8323
\ref{algomix:min}algomix:min225,8507
\item Algorithm~\ref{algo:mixsearch}algo:mixsearch232,8802
\item Algorithm~\ref{algo:mixsearch}algo:mixsearch238,9040
\subsubsection{Handling strict inequalities}Handling250,9314
\laratsolver of \cite{demoura_cav06}demoura_cav06256,9552
We recall that the algorithm in \cite{demoura_cav06}demoura_cav06259,9685
 \cite{demoura_cav06}demoura_cav06297,11122
\cite{demoura_cav06}demoura_cav06310,11549
\cite{demoura_cav06}demoura_cav06316,11741
\subsubsection{Discussion.}Discussion.360,13296
\item \label{item:approximatesolution}item:approximatesolution373,13678
If Algorithm~\ref{algo:mixsearch}algo:mixsearch375,13726
In Algorithm~\ref{algo:mixsearch}algo:mixsearch399,14599
\cite{BSST09HBSAT}BSST09HBSAT409,15076
\item \label{item:lowerboundpruning}item:lowerboundpruning432,16109
minimum cost \currub returned in row~\ref{algomix:min}algomix:min448,16479
\item \label{item:binvslin}item:binvslin453,16613
(see \cite{sellmannk08}sellmannk08470,17408

algorithms_omlaratplus.tex,995
Theorems~\ref{teo:main}teo:main5,101
\ref{teo:muedi-extension}teo:muedi-extension6,155
As suggested by Theorem~\ref{teo:mued-extension}teo:mued-extension12,323
$\eta\defas\mu\wedge\mued$ as in Definition~\ref{as\mu\wedge\mued$17,601
~\ref{teo:main}teo:main23,997
truth assignments $\rho\defas\mu\wedge\mueid$as\mu\wedge\mueid$33,1402
as in Definition~\ref{def:muedi-extension}def:muedi-extension34,1448
~\ref{teo:main}teo:main40,1830
Algorithm~\ref{algo:mixsearch}algo:mixsearch50,2136
\ref{algomix:smtsolverone}algomix:smtsolverone54,2231
Then in step \ref{algomix:min}algomix:min58,2395
    \muei \defas & \{as64,2628
{\em Delayed Theory Combination} \cite{bozzanobcjrrs06}bozzanobcjrrs0685,3341
$\rho\defas\mu_{as\mu_92,3610
Definition~\ref{def:muedi-extension}def:muedi-extension93,3667
\cite{bozzanobcjrrs06}bozzanobcjrrs06119,4643
Theorem~\ref{teo:muedi-extension}teo:muedi-extension121,4717
Theorem~\ref{teo:muedi-extension}teo:muedi-extension125,4860

algorithms.tex,145
\cite{ST-ijcar12-extended}ST-ijcar12-extended58,2117
refer the reader, e.g., to \cite{MSLM09HBSAT,BSST09HBSAT}MSLM09HBSAT,BSST09HBSAT59,2186

appendix.tex,1877
\subsection{Proof of Theorem~\ref{teo:main}}Proof2,1
\label{lemma:main_totalass}lemma:main_totalass7,129
$\cale  \defas \{as9,224
\label{lemma:partvstotalass}lemma:partvstotalass28,886
\label{eq:induced_assignment}eq:induced_assignment48,1555
\eta \defasas49,1585
The proof of Theorem~\ref{teo:main}teo:main70,2258
\label{teo:main_appendix}teo:main_appendix77,2423
$\calm  \defas \{as80,2516
Definition~\ref{def:omlaratplus}def:omlaratplus91,2880
    By Proposition~\ref{prop:cost_monotonicity}prop:cost_monotonicity100,3178
    By Lemma~\ref{lemma:partvstotalass}lemma:partvstotalass103,3266
By lemma~\ref{lemma:main_totalass}lemma:main_totalass108,3463
    From Lemma~\ref{lemma:main_totalass}lemma:main_totalass114,3684
From Proposition~\ref{prop:cost_monotonicity}prop:cost_monotonicity127,4118
\subsection{Proof of Theorem~\ref{teo:mued-extension}}Proof148,4533
\label{teo:mued-extension2}teo:mued-extension2155,4632
  Definition~\ref{def:mued-extension}def:mued-extension157,4681
\mu' \defas \mu \wedge \bigwedge_{as196,5426
\item By Theorem~\ref{teo:NO}teo:NO204,5778
Let $\mu'\defas \mu\wedge(\cost=c)$. Since $(\cost=c)$ is aas228,6639
$\eta'\defas\eta\wedge(\cost=c)$.as\eta\wedge(\cost=c)$.233,6905
the hypothesis of Theorem~\ref{teo:NO}teo:NO236,7019
the hypothesis of Theorem~\ref{teo:NO}teo:NO252,7575
\subsection{Proof of Theorem~\ref{teo:muedi-extension}}Proof272,8018
\label{teo:muedi-extension2}teo:muedi-extension2276,8092
  Definition~\ref{def:mued-extension}def:mued-extension278,8142
\label{eq:augmentedass}eq:augmentedass309,8930
  \mu^{*}&\defas &as310,8954
\item By Theorem~\ref{teo:smt_foundations}teo:smt_foundations335,9595
Thus, by Theorem~\ref{teo:NO}teo:NO347,10061
Let $\mu'\defas \mu\wedge(\cost=c)$.as374,11187
$\rho'\defas\rho\wedge(\cost=c)$.as\rho\wedge(\cost=c)$.385,11532

appendix_tocl.tex,1825
\subsection{Proof of Theorem~\ref{teo:main}}Proof2,1
\label{lemma:main_totalass}lemma:main_totalass7,129
$\cale  \defas \{as9,224
\label{lemma:partvstotalass}lemma:partvstotalass28,886
\label{eq:induced_assignment}eq:induced_assignment48,1555
\eta \defasas49,1585
The proof of Theorem~\ref{teo:main}teo:main70,2258
$\calm  \defas \{as80,2531
Definition~\ref{def:omlaratplus}def:omlaratplus91,2898
    By Proposition~\ref{prop:cost_monotonicity}prop:cost_monotonicity100,3193
    By Lemma~\ref{lemma:partvstotalass}lemma:partvstotalass103,3281
By lemma~\ref{lemma:main_totalass}lemma:main_totalass108,3478
    From Lemma~\ref{lemma:main_totalass}lemma:main_totalass114,3700
From Proposition~\ref{prop:cost_monotonicity}prop:cost_monotonicity127,4134
\subsection{Proof of Theorem~\ref{teo:mued-extension}}Proof148,4546
\label{teo:mued-extension2}teo:mued-extension2155,4669
  Definition~\ref{def:mued-extension}def:mued-extension157,4718
\mu' \defas \mu \wedge \bigwedge_{as196,5466
\item By Theorem~\ref{teo:NO}teo:NO204,5818
Let $\mu'\defas \mu\wedge(\cost=c)$. Since $(\cost=c)$ is aas228,6675
$\eta'\defas\eta\wedge(\cost=c)$.as\eta\wedge(\cost=c)$.233,6941
the hypothesis of Theorem~\ref{teo:NO}teo:NO236,7055
the hypothesis of Theorem~\ref{teo:NO}teo:NO252,7611
\subsection{Proof of Theorem~\ref{teo:muedi-extension}}Proof272,8056
\label{teo:muedi-extension2}teo:muedi-extension2276,8154
  Definition~\ref{def:mued-extension}def:mued-extension278,8204
\label{eq:augmentedass}eq:augmentedass309,8995
  \mu^{*}&\defas &as310,9019
\item By Theorem~\ref{teo:smt_foundations}teo:smt_foundations335,9660
Thus, by Theorem~\ref{teo:NO}teo:NO347,10126
Let $\mu'\defas \mu\wedge(\cost=c)$.as374,11248
$\rho'\defas\rho\wedge(\cost=c)$.as\rho\wedge(\cost=c)$.385,11593

background_gdlp.tex,1161
Programming (LP) involving both discrete and continuous variables \cite{lodi}lodi4,114
\begin{equation} \label{eq:milp}eq:milp6,233
\emph{branch-and-cut} approach (see e.g. \cite{lodi}lodi16,720
(see \cite{Achterberg08}Achterberg0820,870
\cite{lodi}lodi52,2229
\cite{Egon19983}Egon1998365,2808
\label{disjset}disjset71,2977
\label{disjset}disjset84,3346
\label{disjset2}disjset291,3538
and the branch-and-bound schema (see, e.g., \cite{BalasB07}BalasB07115,4591
\cite{RamanGross94}RamanGross94120,4778
problem \cite{RamanGross94,VecchGross04,SawayaG05,SawayaGrossmann2012}RamanGross94,VecchGross04,SawayaG05,SawayaGrossmann2012133,5306
The general formulation of a LGDP problem is the following \cite{RamanGross94}RamanGross94145,5651
\label{eq:lgdp}eq:lgdp164,6334
\begin{eqnarray} \label{eq:lgdp}eq:lgdp187,7052
and linear inequalities as follows \cite{RamanGross94}RamanGross94232,8881
\begin{equation}\label{eq:bm}eq:bm246,9473
\begin{eqnarray}\label{eq:bm}eq:bm261,10088
\begin{equation}\label{eq:cm}eq:cm295,11840
\begin{eqnarray}\label{eq:cm}eq:cm309,12617
Sawaya and Grossman \cite{SawayaG05}SawayaG05325,13530

background_sat_long.tex,578
  \caption{Schema of a conflict-driven \dpll SAT solver.\label{fig:dpll}fig:dpll84,3578
is reported in Figure~\ref{fig:dpll}fig:dpll94,3828
on the {two-watched-literal scheme}~\cite{moskewicz01chaff}moskewicz01chaff140,6012
(see, e.g., \cite{moskewicz01chaff,zhang01learning}moskewicz01chaff,zhang01learning145,6132
\cite{zhang01learning}zhang01learning162,7066
  incremental interface} (see e.g. \cite{eensorensson:sat2003}eensorensson:sat2003180,7771
$\Phi\defas\set{as\set183,7960
  formula, see e.g. \cite{lynce_unsatcore_sat04}lynce_unsatcore_sat04205,8985

background_sat.tex,538
\cite{MSLM09HBSAT}MSLM09HBSAT5,135
CNF-ized as in \cite{plaisted6}plaisted68,264
on the {\em two-watched-literal scheme}, see \cite{MSLM09HBSAT}MSLM09HBSAT35,1424
the {\em conflict clause} $\psi'\defas\neg\eta$ is added to $\varphi$as\neg\eta$91,3469
e.g. \cite{MSLM09HBSAT,nieot-jacm-06}MSLM09HBSAT,nieot-jacm-06105,4068
  incremental interface} (see e.g. \cite{eensorensson:sat2003}eensorensson:sat2003109,4167
$\Phi\defas\set{as\set113,4359
  formula, see e.g. \cite{lynce_unsatcore_sat04}lynce_unsatcore_sat04139,5491

background_smt.tex,786
$\mu$ to be checked by the \Tsolver \cite{sebastiani07}sebastiani07113,4622
\cite{nieot-jacm-06,sebastiani07,BSST09HBSAT}nieot-jacm-06,sebastiani07,BSST09HBSAT131,5273
in order to decide \larat \cite{demoura_cav06}demoura_cav06163,6471
\cite{griggio-jsat11}griggio-jsat11164,6529
simplex-based algorithm by Dutertre and de Moura \cite{demoura_cav06}demoura_cav06175,6944
  exists a rational number $\epsilon > 0$ such that $\Gamma_\epsilon \defasas190,7712
  $S_\epsilon \defas \{as192,7849
The idea of \cite{demoura_cav06}demoura_cav06195,7937
 (We refer the reader to \cite{demoura_cav06}demoura_cav06202,8272
Remarkably, in \cite{demoura_cav06}demoura_cav06208,8424
  $\vplus{v}+\vplus{u}\defas\pair{as\pair222,9039
  $a\vplus{v}\defas\vplus{as\vplus223,9103

background.tex,72
\label{remark:constantsvsvariables}remark:constantsvsvariables54,1404

concl.tex,61
in \mathsat{}{\ \cite{griggio-jsat11}griggio-jsat1136,1294

expeval_enc.tex,156
in (\ref{eq:ldgp_enc}eq:ldgp_enc4,80
  conversion of  \cite{plaisted6}plaisted675,2604
\label{eq:enc1}eq:enc193,3311
\label{eq:enc2}eq:enc2137,4714

expeval_lgdp_disc.tex,805
The table of Figure \ref{fig:plots_sp}fig:plots_sp2,1
The scatter-plots of Figure \ref{fig:plots_sp}fig:plots_sp11,343
The table of Figure \ref{fig:plots_js}fig:plots_js18,629
The scatter-plots of Figure \ref{fig:plots_js}fig:plots_js28,1050
in Figures~\ref{fig:plots_sp}fig:plots_sp38,1470
point~\ref{item:binvslin}item:binvslin77,3040
the cost variables $\cost\defas L$ [resp. $\cost\defas M$]as89,3566
\label{remark:binvslin}remark:binvslin97,4012
\cite{VecchGross04,SawayaG05,SawayaGrossmann2012}VecchGross04,SawayaG05,SawayaGrossmann2012108,4395
\label{fig:comp_time}fig:comp_time206,8354
\subsubsection{Analysis of \optmathsat performances.}Analysis211,8407
\label{sec:expeval_lgdp_analysis}sec:expeval_lgdp_analysis212,8461
Figure~\ref{fig:comp_time}fig:comp_time229,9073

expeval_lgdp_js.tex,487
\label{fig:plots_js}fig:plots_js31,1509
{(See Figure~\ref{fig:lgdp}fig:lgdp50,2075
The LGDP model provided by \cite{SawayaG05}SawayaG0554,2183
\label{eq:lgdp_js}eq:lgdp_js58,2290
We encoded the corresponding LGDP model (\ref{eq:lgdp_js}eq:lgdp_js84,3353
\label{eq:js_enc}eq:js_enc88,3468
\vi & \defas & (\cost = M) \wedge \bigwedge_{as90,3505
The table of Figure \ref{fig:plots_js}fig:plots_js110,4527
The scatter-plots of Figure \ref{fig:plots_js}fig:plots_js120,4948

expeval_lgdp_sp.tex,614
\label{fig:plots_sp}fig:plots_sp48,2658
We considered the LGDP model provided by \cite{SawayaG05}SawayaG0565,3121
{(See Figure~\ref{fig:lgdp}fig:lgdp70,3342
The LGDP model provided by \cite{SawayaG05}SawayaG0573,3449
\label{eq:lgdp_sp}eq:lgdp_sp82,3674
We express straightforwardly the LGDP model (\ref{eq:lgdp_sp}eq:lgdp_sp125,5078
\label{eq:sp_enc}eq:sp_enc129,5196
\vi & \defas & (\cost = L) \wedge \bigwedge_{as131,5233
used by \cite{SawayaG05}SawayaG05150,6153
The table of Figure \ref{fig:plots_sp}fig:plots_sp174,7256
The scatter-plots of Figure \ref{fig:plots_sp}fig:plots_sp183,7598

expeval_lgdp.tex,134
\cite{VecchGross04,SawayaG05,SawayaGrossmann2012}VecchGross04,SawayaG05,SawayaGrossmann201215,593
\label{fig:lgdp}fig:lgdp63,2271

expeval_pb.tex,980
MaxSMT benchmarks from \protect\cite{cimattifgss10}cimattifgss1022,691
\label{fig:pb_results}fig:pb_results48,1916
As a fourth comparison, in Figure~\ref{fig:pb_results}fig:pb_results51,1953
on the problem sets used in \cite{cimattifgss10}cimattifgss1053,2034
\cite{cimattifgss10}cimattifgss1056,2182
\footnote{A comparison against the tool in \cite{cimattifgss10}cimattifgss1058,2292
implementations is in \cite{cgss_sat13_maxsmt}cgss_sat13_maxsmt61,2492
As described in \cite{cimattifgss10}cimattifgss1067,2676
\subsubsection{Discussion}Discussion82,3317
The results are presented in Figure~\ref{fig:pb_results}fig:pb_results85,3346
Remark~\ref{remark:binvslin}remark:binvslin114,4604
 \label{remark:binvslin2}remark:binvslin2127,5210
The scatter-plots in Figure~\ref{fig:pb_results}fig:pb_results132,5253
As a side note, in \cite{cgss_sat13_maxsmt}cgss_sat13_maxsmt140,5545
We refer the reader to \cite{cgss_sat13_maxsmt}cgss_sat13_maxsmt145,5864

expeval_sal_disc.tex,111
\label{fig:plots_clauses}fig:plots_clauses12,400
The figure~\ref{fig:plots_clauses}fig:plots_clauses16,456

expeval_sal.tex,533
\label{fig:plots_sal}fig:plots_sal43,1762
in Figure~\ref{fig:plots_sal}fig:plots_sal52,1906
of invariants \cite{biere-cimatti-tacas}biere-cimatti-tacas57,2150
and K-Induction (\kind) \cite{SheeranSS00}SheeranSS0058,2192
\cite{acks_forte02}acks_forte0273,2864
produced the formulas in the CVC3 language \cite{cvc3}cvc3110,4412
problems of the SAL model in CVC3 language \cite{cvc3}cvc3131,5164
\subsubsection{Discussion}Discussion167,6469
The results are presented in Figure~\ref{fig:plots_sal}fig:plots_sal170,6509

expeval_smtlib.tex,317
  \label{fig:generalresults}fig:generalresults35,1884
in Figure~\ref{fig:generalresults}fig:generalresults55,2357
\subsubsection{Discussion}Discussion153,6657
Remark~\ref{rem:infiniteprec}rem:infiniteprec158,6949
  \label{fig:smtlib_general}fig:smtlib_general202,8758
\label{fig:smtlib}fig:smtlib237,9899

expeval.tex,861
 \cite{mathsat5_tacas13}mathsat5_tacas138,269
v23.7.1 \cite{gams}gams45,1786
required by specific solvers, like \cplex \cite{cplex}cplex53,2059
convex-hull (CH) methods \cite{RamanGross94,SawayaGrossmann2012}RamanGross94,SawayaGrossmann201267,2518
use \cplex v12.2 \cite{cplex}cplex68,2588
default options, as suggested by the authors \cite{Vecchietti11}Vecchietti1170,2720
augmented by Pseudo-Boolean (PB) optimization \cite{cimattifgss10}cimattifgss1073,2836
\label{rem:infiniteprec}rem:infiniteprec82,3165
 (default $\epsilon\defas10^{as10^94,3570
  \jams authors \cite{VecchGross04,SawayaG05,SawayaGrossmann2012}VecchGross04,SawayaG05,SawayaGrossmann2012104,3955
\item (\sref{sec:expeval_pb}) the MaxSMT problems from \cite{cimattifgss10}cimattifgss10113,4347
they are subject to licencing restrictions,  see \cite{gams}gams177,6667

extended.tex,1990
\renewcommand{\topfraction}\topfraction3,32
\renewcommand{\bottomfraction}\bottomfraction4,63
\renewcommand{\textfraction}\textfraction5,97
\renewcommand{\ignoreinshort}\ignoreinshort43,913
\renewcommand{\ignoreinlong}\ignoreinlong48,992
\section{Introduction}Introduction78,1389
\input{intro}\label{sec:intro}sec:intro79,1412
\section{Backgrond}Backgrond81,1471
\input{background}\label{sec:background}sec:background82,1491
\subsection{Linear Generalized Disjunctive Programming}Linear83,1532
\input{background_gdlp}\label{sec:background_lgdp}sec:background_lgdp84,1588
\subsection{SAT and CDCL SAT Solvers}SAT85,1639
\input{background_sat}\label{sec:background_sat}sec:background_sat86,1677
\subsection{SMT and Lazy SMT Solvers}SMT89,1864
\input{background_smt}\label{sec:background_smt}sec:background_smt90,1902
\section{Optimization in Satisfiability Modulo \larat}Optimization92,1989
\input{optsmt}\label{sec:optsmt}sec:optsmt94,2075
\section{Optimization Procedures for \omlarat} Optimization96,2137
\input{algorithms.tex}\label{sec:algorithms}sec:algorithms97,2185
\subsection{A Linear-Search Procedure for \omlarat} A98,2230
\input{algorithms_lin.tex}\label{sec:algorithms_lin}sec:algorithms_lin99,2283
\subsection{A Mixed Linear/Binary-Search Procedure for \omlarat}A101,2346
\input{algorithms_bin.tex}\label{sec:algorithms_bin}sec:algorithms_bin102,2411
\section{An experimental Evaluation}An105,2529
\input{expeval}\label{sec:expeval}sec:expeval106,2566
\subsubsection{The strip-packing problem.}The107,2601
\input{expeval_sp}\label{sec:expeval_sp}sec:expeval_sp108,2644
\subsubsection{The zero-wait jobshop problem.}The109,2685
\input{expeval_js}\label{sec:expeval_js}sec:expeval_js110,2732
\subsubsection{Discussion.}Discussion.111,2773
\input{expeval_disc}\label{sec:expeval_disc}sec:expeval_disc112,2801
\section{Conclusions and Future Work}Conclusions117,2985
\input{concl}\label{sec:concl}sec:concl118,3023

intro.tex,976
\ignoreinshort{(See \cite{sebastiani07,BSST09HBSAT}sebastiani07,BSST09HBSAT19,717
\ignoreinlong{(See \cite{BSST09HBSAT}BSST09HBSAT20,788
E.g., in (SMT-based) {\em planning with resources} \cite{wolfman1}wolfman138,1463
\ignoreinshort{(e.g. \cite{acks_forte02,AudemardBCS05}acks_forte02,AudemardBCS0543,1796
\ignoreinlong{(e.g. \cite{acks_forte02}acks_forte0244,1853
disjunctive programming (LDP)} \cite{Egon19983}Egon1998354,2304
\cite{RamanGross94,SawayaGrossmann2012}RamanGross94,SawayaGrossmann201257,2411
 \cite{RM09HBSAT,LM09HBSAT,nieuwenhuis_sat06,cimattifgss10,cgss_sat13_maxsmt}RM09HBSAT,LM09HBSAT,nieuwenhuis_sat06,cimattifgss10,cgss_sat13_maxsmt60,2547
\cite{nieuwenhuis_sat06,cimattifgss10,st-ijcar12,dilligdma12,cgss_sat13_maxsmt,manoliosp13}nieuwenhuis_sat06,cimattifgss10,st-ijcar12,dilligdma12,cgss_sat13_maxsmt,manoliosp1371,3082
at IJCAR~2012~conference~\cite{st-ijcar12}st-ijcar1290,3947
\cite{mathsat5_tacas13}mathsat5_tacas13113,4823

macros_specific.tex,3838
\newcommand{\length}\length3,35
\renewcommand{\todo}\todo5,111
\newenvironment{rsoldchange}rsoldchange10,290
\renewenvironment{rschange}rschange11,352
\renewcommand{\RSCHANGE}\RSCHANGE12,408
\newcommand{\STCHANGE}\STCHANGE13,460
\newcommand{\onlyinsilviathesis}\onlyinsilviathesis16,578
\renewcommand{\ignoreinshort}\ignoreinshort19,619
\renewcommand{\ignoreinlong}\ignoreinlong24,708
\renewcommand{\marg}\marg33,871
\newcommand{\maybeignore}\maybeignore36,929
\newcommand{\pr}\pr39,1016
\newcommand{\omtlcf}\omtlcf42,1104
\newcommand{\omtlcft}\omtlcft43,1141
\newcommand{\omtlcfla}\omtlcfla44,1203
\newcommand{\lb}\lb45,1270
\renewcommand{\ub}\ub46,1320
\newcommand{\omtplus}\omtplus47,1372
\newcommand{\omlarat}\omlarat48,1435
\newcommand{\omlaratplus}\omlaratplus49,1497
\newcommand{\varphicost}\varphicost50,1569
\newcommand{\pivot}\pivot51,1625
\newcommand{\status}\status52,1681
\renewcommand{\status}\status53,1739
\newcommand{\smtlaratplus}\smtlaratplus55,1797
\newcommand{\laratplus}\laratplus56,1853
\renewcommand{\cost}\cost58,1912
\newcommand{\currlb}\currlb62,1976
\newcommand{\currub}\currub63,2029
\newcommand{\range}\range64,2082
\newcommand{\currrange}\currrange65,2133
\newcommand{\lpivotrange}\lpivotrange66,2196
\newcommand{\rpivotrange}\rpivotrange67,2260
\newcommand{\computepivot}\computepivot68,2324
\newcommand{\dopivoting}\dopivoting70,2457
\newcommand{\ubliti}\ubliti72,2526
\newcommand{\lbliti}\lbliti73,2584
\newcommand{\pivotatom}\pivotatom74,2646
\newcommand{\currlblit}\currlblit75,2704
\newcommand{\currublit}\currublit76,2771
\newcommand{\currubliti}\currubliti77,2834
\newcommand{\negcurrubliti}\negcurrubliti78,2906
\newcommand{\minvalue}\minvalue81,2987
\newcommand{\maxvalue}\maxvalue82,3044
\newcommand{\mvalue}\mvalue83,3101
\renewcommand{\mincost}\mincost84,3154
\newcommand{\minimize}\minimize86,3219
\newcommand{\isminimum}\isminimum87,3281
\newcommand{\incrementalsmt}\incrementalsmt89,3420
\newcommand{\smtcoreextract}\smtcoreextract90,3500
\newcommand{\incrementalsmtcore}\incrementalsmtcore91,3580
\newcommand{\laqliterals}\laqliterals92,3677
\renewcommand{\Tsolver}\Tsolver94,3752
\renewcommand{\Tsolvers}\Tsolvers95,3816
\newcommand{\laratsolver}\laratsolver96,3882
\newcommand{\laratsolvers}\laratsolvers97,3952
\newcommand{\laratlemma}\laratlemma98,4024
\newcommand{\laratlemmas}\laratlemmas99,4072
\newcommand{\vplus}\vplus101,4123
\newcommand{\optimathsat}\optimathsat105,4213
\newcommand{\ar}\ar110,4391
\newcommand{\mat}\mat111,4451
\renewcommand{\ar}\ar112,4512
\renewcommand{\mat}\mat113,4564
\newcommand{\ari}\ari115,4618
\newcommand{\mati}\mati116,4684
\renewcommand{\ari}\ari117,4751
\renewcommand{\mati}\mati118,4809
\newcommand{\enc}\enc120,4869
\renewcommand{\enc}\enc121,4935
\newcommand{\cplex}\cplex123,4982
\newcommand{\fakesubsubsection}\fakesubsubsection131,5166
\newcommand{\trueval}\trueval134,5332
\newcommand{\falseval}\falseval135,5384
\newcommand{\eqij}\eqij143,5620
\newcommand{\neqij}\neqij144,5670
\newcommand{\dij}\dij145,5725
\newcommand{\dji}\dji146,5774
\newcommand{\mularat}\mularat148,5873
\newcommand{\mubool}\mubool149,5929
\newcommand{\mue}\mue151,5989
\newcommand{\mud}\mud152,6036
\newcommand{\mui}\mui153,6083
\newcommand{\mued}\mued154,6130
\newcommand{\muei}\muei155,6179
\newcommand{\mueid}\mueid156,6228
\newcommand{\IE}\IE158,6280
\newcommand{\IEplus}\IEplus159,6338
\newcommand{\IEminus}\IEminus160,6404
\newcommand{\IEminusg}\IEminusg161,6474
\newcommand{\IEminusl}\IEminusl162,6542
\newcommand{\Tk}\Tk165,6632
\newcommand{\edmuext}\edmuext168,6677
\newcommand{\edimuext}\edimuext169,6743
\renewcommand{\algorithmiccomment}\algorithmiccomment173,6871

main.tex,2555
\renewcommand{\topfraction}\topfraction5,57
\renewcommand{\bottomfraction}\bottomfraction6,88
\renewcommand{\textfraction}\textfraction7,122
\newcommand{\mytitle}\mytitle51,1058
\section{Introduction}Introduction119,1939
\label{sec:intro}sec:intro120,1962
\section{Background}Background127,2043
\label{sec:background}sec:background128,2064
 \subsection{Linear Generalized Disjunctive Programming}Linear129,2105
 \label{sec:background_lgdp}sec:background_lgdp130,2162
\subsection{SAT and CDCL SAT Solvers}SAT131,2214
\label{sec:background_sat}sec:background_sat132,2252
\subsection{SMT and Lazy SMT Solvers}SMT133,2301
\label{sec:background_smt}sec:background_smt134,2339
\section{Optimization in \smtlaratplus }Optimization137,2429
\label{sec:optsmt}sec:optsmt139,2501
\section{Procedures for \omlarat and \omlaratplus} Procedures141,2564
\label{sec:algorithms}sec:algorithms142,2616
\subsection{An Offline Schema for \omlarat }An143,2657
\label{sec:algorithms_offline}sec:algorithms_offline144,2702
\subsection{An Inline Schema for \omlarat}An146,2769
\label{sec:algorithms_inline}sec:algorithms_inline147,2812
\subsection{Extensions to \omlaratplus}  Extensions149,2870
\label{sec:algorithms_omlaratplus}sec:algorithms_omlaratplus150,2912
\section{Experimental Evaluation}Experimental155,3059
\label{sec:expeval}sec:expeval156,3093
\subsection{Encodings.}Encodings.158,3130
\label{sec:expeval_enc}sec:expeval_enc159,3154
\subsection{Comparison on LGDP Problems}Comparison161,3199
\label{sec:expeval_lgdp}sec:expeval_lgdp162,3240
\subsubsection{The strip-packing problem.}The163,3285
\label{sec:expeval_sp}sec:expeval_sp164,3328
\subsubsection{The zero-wait jobshop problem.}The165,3374
\label{sec:expeval_js}sec:expeval_js166,3421
\subsubsection{Discussion.}Discussion.167,3467
\label{sec:expeval_disc}sec:expeval_disc168,3495
\subsection{Comparison on SMT-LIB Problems}Comparison169,3545
\label{sec:expeval_smtlib}sec:expeval_smtlib170,3589
\subsection{Comparison on SAL Problems}Comparison171,3638
\label{sec:expeval_sal}sec:expeval_sal172,3678
\subsection{Comparison on Pseudo-Boolean SMT Problems}Comparison174,3723
\label{sec:expeval_pb}sec:expeval_pb175,3778
\section{Related work.} %Related182,3939
\label{sec:related}sec:related183,3965
\section{Conclusions and Future Work}Conclusions188,4049
\label{sec:concl}sec:concl189,4087
\appendix198,4286
\section{Appendix: Proof of the Theorems}Appendix:199,4296
\label{sec:appendix}sec:appendix200,4338

optsmt.tex,5133
\subsection{Basic Definitions and Notation}Basic12,386
\label{sec:optsmt_formal}sec:optsmt_formal13,430
\label{def:omtplus}def:omtplus21,629
theories  with equality (``Nelson-Oppen theories'' \cite{nelson3}nelson338,1269
\label{def:omlaratplus}def:omlaratplus49,1653
\laratplus formulas are {\em pure} \cite{nelson3}nelson378,2551
Although the purity assumption is not necessary (see \cite{bds02}bds0285,2866
every non-pure formula can be easily purified \cite{nelson3}nelson388,3079
\label{def:cost_polarity}def:cost_polarity101,3434
\label{def:bounds}def:bounds116,4032
\subsection{Theoretical Results}Theoretical139,4962
\label{sec:optsmt_results}sec:optsmt_results140,4995
The proofs of the novel results are reported in Appendix~\ref{sec:appendix}sec:appendix143,5087
The following facts follow straightforwardly from Definition~\ref{def:omlaratplus}def:omlaratplus147,5167
\label{prop:cost_monotonicity}prop:cost_monotonicity150,5273
\label{def:complete_assignment_set}def:complete_assignment_set168,5829
\begin{theorem}[\cite{sebastiani07}sebastiani07177,6168
\label{teo:smt_foundations}teo:smt_foundations178,6205
Theorem~\ref{teo:smt_foundations}teo:smt_foundations187,6528
\Tsolver. Notice that in Theorem~\ref{teo:smt_foundations}teo:smt_foundations191,6799
Here we extend Theorem~\ref{teo:smt_foundations}teo:smt_foundations194,6932
\label{teo:main}teo:main201,7080
$\calm  \defas \{as204,7163
  $min_{\mu\in\calm}\mincost(\mu)\defas+\infty$ if $\cal M$ is empty.)}as+\infty$213,7418
\larat constraints, so that Theorem~\ref{teo:main}teo:main223,7809
\label{def:interfaceequalities}def:interfaceequalities236,8299
As common practice (see e.g. \cite{TinHar-FROCOS-96}TinHar-FROCOS-96255,8868
\mbox{$\IE{\vi}\defas\{as\261,9171
\begin{theorem}[\cite{TinHar-FROCOS-96}TinHar-FROCOS-96274,9583
\label{teo:NO}teo:NO275,9624
let $\mu \defas\mu_{as\mu_279,9761
  \cite{TinHar-FROCOS-96}TinHar-FROCOS-96312,11046
\label{eq:no}eq:no316,11097
   \mued \defas \mue \wedge \mud,\ \ s.t. \as320,11235
\mue\defas\bigwedge_{as\bigwedge_321,11279
\mud\defas\bigwedge_{as\bigwedge_322,11332
Theorem~\ref{teo:NO}teo:NO338,11759
Theorem~\ref{teo:NO}teo:NO355,12318
theories \cite{bozzanobcjrrs06}bozzanobcjrrs06357,12451
$\mu$ can be written as $\mu \defasas367,12896
\label{def:mued-extension}def:mued-extension381,13327
    Let $\mu \defas \mubool\wedge \mularat\wedge\mut$ be a as382,13354
the set $\edmuext\defas\{as\389,13693
\label{teo:mued-extension}teo:mued-extension396,13925
  Definition~\ref{def:mued-extension}def:mued-extension398,13973
Thus, by combining Theorems~\ref{teo:main}teo:main425,14637
\cite{demoura_cav06}demoura_cav06432,14969
\label{def:muedi-extension}def:muedi-extension446,15588
Let $\mu$ be as in  Definition~\ref{def:mued-extension}def:mued-extension447,15616
the set $\edimuext\defas\{as\450,15740
where $\mued$ is as in Definition~\ref{def:mued-extension}def:mued-extension452,15863
\label{teo:muedi-extension}teo:muedi-extension470,16436
  Definition~\ref{def:mued-extension}def:mued-extension472,16485
\item \label{item:a}item:a476,16553
\item \label{item:b}item:b478,16663
\item \label{item:c}item:c480,16739
\item \label{item:d}item:d484,16925
Thus, by combining Theorems~\ref{teo:main}teo:main500,17298
\subsection{\omlaratplus wrt. other Optimization Problems}\omlaratplus511,17687
\label{sec:optsmt_comparison}sec:optsmt_comparison512,17746
\omlarat{} (see~\cite{ST-ijcar12-extended}ST-ijcar12-extended518,17945
 $\vi\defas\vi'\wedge(\cost = \sum_{as\vi'\wedge(\cost527,18184
(\ref{disjset}disjset537,18487
\ignoreinshort{and (\ref{disjset2}disjset2538,18504
\label{eq:ldp_encoding}eq:ldp_encoding558,19049
 CNF-ization process of \cite{plaisted6}plaisted6568,19444
\label{eq:ldgp_enc}eq:ldgp_enc580,19795
\vi&\defas&  (\cost = \sum_{as&582,19834
 CNF-ization process of \cite{plaisted6}plaisted6628,20640
Pseudo-Boolean (PB) constraints (see \cite{RM09HBSAT}RM09HBSAT640,20986
\label{eq:pb2smt-encoding}eq:pb2smt-encoding657,21764
A partial weighted MaxSMT problem (see \cite{nieuwenhuis_sat06,cimattifgss10,cgss_sat13_maxsmt}nieuwenhuis_sat06,cimattifgss10,cgss_sat13_maxsmt676,22312
\label{eq:maxsmt2pb-encoding}eq:maxsmt2pb-encoding691,23141
\vi' \defas \vi_{as694,23193
\cost \defas \sum_{as696,23265
\tuple{\vi',\cost\defas \sum_j \ari{as701,23427
\label{eq:pb2maxsmt-encoding}eq:pb2maxsmt-encoding703,23520
\vi_{h} \defas \vi';as706,23572
\vi_{s} \defas \bigcup_{as708,23597
 MaxSAT/ MaxSMT) addressed in \cite{nieuwenhuis_sat06,cimattifgss10}nieuwenhuis_sat06,cimattifgss10725,24146
\cite{bebmaxsat,Xing2005MaxSolver,HerasLO08,RM09HBSAT,Barth95adavis-putnam,bebmethods}bebmaxsat,Xing2005MaxSolver,HerasLO08,RM09HBSAT,Barth95adavis-putnam,bebmethods738,24773
and SMT \cite{NieuwenhuisOliveras2006SAT,CimattiFGSS10}NieuwenhuisOliveras2006SAT,CimattiFGSS10739,24861
\cite{NieuwenhuisOliveras2006SAT,CimattiFGSS10}NieuwenhuisOliveras2006SAT,CimattiFGSS10743,25100
and writing the cost function as in (\ref{cfsum}cfsum748,25372

related.tex,1086
Oliveras \cite{nieuwenhuis_sat06}nieuwenhuis_sat0610,280
Cimatti et al. \cite{cimattifgss10}cimattifgss1019,722
The SMT solvers \yices \cite{yices_sd}yices_sd26,1066
Ans{\'o}tegui et al. \cite{AnsoteguiBPSV11}AnsoteguiBPSV1137,1390
Cimatti et al. \cite{cgss_sat13_maxsmt}cgss_sat13_maxsmt42,1587
Dillig et al. \cite{dilligdma12}dilligdma1270,2530
\footnote{Quoting an example from \cite{dilligdma12}dilligdma1274,2762
given the  formula {$\vi\defas(x+y+w>0)\vee(x+y+z+w<5)$}as(x+y+w>0)\vee(x+y+z+w<5)$75,2817
Manolios and Papavasileiou \cite{manoliosp13}manoliosp1386,3273
 Notice that the approach of \cite{manoliosp13}manoliosp1398,3724
 (See Definition 2 in  \cite{manoliosp13}manoliosp13101,3862
\cite{li_popl14}li_popl14123,4533
\cite{st-ijcar12}st-ijcar12128,4686
\footnote{More precisely, in \cite{li_popl14}li_popl14139,5163
Then \cite{li_popl14}li_popl14145,5481
of \cite{st-ijcar12}st-ijcar12147,5581
of the \zthree SMT solver \cite{z3}z3149,5660
version described in \cite{st-ijcar12}st-ijcar12157,6087
\cite{li_popl14}li_popl14161,6223

rgb.tex,16818
\definecolor {inecolor18,747
\definecolor {inecolor19,804
\definecolor {inecolor20,861
\definecolor {inecolor21,918
\definecolor {inecolor22,975
\definecolor {inecolor23,1032
\definecolor {inecolor24,1089
\definecolor {inecolor25,1146
\definecolor {inecolor26,1203
\definecolor {inecolor27,1260
\definecolor {inecolor28,1317
\definecolor {inecolor29,1374
\definecolor {inecolor30,1431
\definecolor {inecolor31,1488
\definecolor {inecolor32,1545
\definecolor {inecolor33,1602
\definecolor {inecolor34,1659
\definecolor {inecolor35,1716
\definecolor {inecolor36,1773
\definecolor {inecolor37,1830
\definecolor {inecolor38,1887
\definecolor {inecolor39,1944
\definecolor {inecolor40,2001
\definecolor {inecolor41,2058
\definecolor {inecolor42,2115
\definecolor {inecolor43,2172
\definecolor {inecolor44,2229
\definecolor {inecolor45,2286
\definecolor {inecolor46,2343
\definecolor {inecolor47,2400
\definecolor {inecolor48,2457
\definecolor {inecolor49,2514
\definecolor {inecolor50,2571
\definecolor {inecolor51,2628
\definecolor {inecolor52,2685
\definecolor {inecolor53,2742
\definecolor {inecolor54,2799
\definecolor {inecolor55,2856
\definecolor {inecolor56,2913
\definecolor {inecolor57,2970
\definecolor {inecolor58,3027
\definecolor {inecolor59,3084
\definecolor {inecolor60,3141
\definecolor {inecolor61,3198
\definecolor {inecolor62,3255
\definecolor {inecolor63,3312
\definecolor {inecolor64,3369
\definecolor {inecolor65,3426
\definecolor {inecolor66,3483
\definecolor {inecolor67,3540
\definecolor {inecolor68,3597
\definecolor {inecolor69,3654
\definecolor {inecolor70,3711
\definecolor {inecolor71,3768
\definecolor {inecolor72,3825
\definecolor {inecolor73,3882
\definecolor {inecolor74,3939
\definecolor {inecolor75,3996
\definecolor {inecolor76,4053
\definecolor {inecolor77,4110
\definecolor {inecolor78,4167
\definecolor {inecolor79,4224
\definecolor {inecolor80,4281
\definecolor {inecolor81,4338
\definecolor {inecolor82,4395
\definecolor {inecolor83,4452
\definecolor {inecolor84,4509
\definecolor {inecolor85,4566
\definecolor {inecolor86,4623
\definecolor {inecolor87,4680
\definecolor {inecolor88,4737
\definecolor {inecolor89,4794
\definecolor {inecolor90,4851
\definecolor {inecolor91,4908
\definecolor {inecolor92,4965
\definecolor {inecolor93,5022
\definecolor {inecolor94,5079
\definecolor {inecolor95,5136
\definecolor {inecolor96,5193
\definecolor {inecolor97,5250
\definecolor {inecolor98,5307
\definecolor {inecolor99,5365
\definecolor {inecolor100,5422
\definecolor {inecolor101,5479
\definecolor {inecolor102,5536
\definecolor {inecolor103,5593
\definecolor {inecolor104,5650
\definecolor {inecolor105,5707
\definecolor {inecolor106,5764
\definecolor {inecolor107,5821
\definecolor {inecolor108,5878
\definecolor {inecolor109,5935
\definecolor {inecolor110,5992
\definecolor {inecolor111,6049
\definecolor {inecolor112,6106
\definecolor {inecolor113,6163
\definecolor {inecolor114,6220
\definecolor {inecolor115,6277
\definecolor {inecolor116,6334
\definecolor {inecolor117,6391
\definecolor {inecolor118,6448
\definecolor {inecolor119,6505
\definecolor {inecolor120,6562
\definecolor {inecolor121,6619
\definecolor {inecolor122,6676
\definecolor {inecolor123,6733
\definecolor {inecolor124,6790
\definecolor {inecolor125,6847
\definecolor {inecolor126,6904
\definecolor {inecolor127,6961
\definecolor {inecolor128,7018
\definecolor {inecolor129,7075
\definecolor {inecolor130,7132
\definecolor {inecolor131,7189
\definecolor {inecolor132,7246
\definecolor {inecolor133,7303
\definecolor {inecolor134,7360
\definecolor {inecolor135,7417
\definecolor {inecolor136,7474
\definecolor {inecolor137,7531
\definecolor {inecolor138,7588
\definecolor {inecolor139,7645
\definecolor {inecolor140,7702
\definecolor {inecolor141,7759
\definecolor {inecolor142,7816
\definecolor {inecolor143,7873
\definecolor {inecolor144,7930
\definecolor {inecolor145,7987
\definecolor {inecolor146,8044
\definecolor {inecolor147,8101
\definecolor {inecolor148,8158
\definecolor {inecolor149,8215
\definecolor {inecolor150,8272
\definecolor {inecolor151,8329
\definecolor {inecolor152,8386
\definecolor {inecolor153,8443
\definecolor {inecolor154,8500
\definecolor {inecolor155,8557
\definecolor {inecolor156,8614
\definecolor {inecolor157,8671
\definecolor {inecolor158,8728
\definecolor {inecolor159,8785
\definecolor {inecolor160,8842
\definecolor {inecolor161,8899
\definecolor {inecolor162,8956
\definecolor {inecolor163,9013
\definecolor {inecolor164,9070
\definecolor {inecolor165,9127
\definecolor {inecolor166,9184
\definecolor {inecolor167,9241
\definecolor {inecolor168,9298
\definecolor {inecolor169,9355
\definecolor {inecolor170,9412
\definecolor {inecolor171,9469
\definecolor {inecolor172,9526
\definecolor {inecolor173,9583
\definecolor {inecolor174,9640
\definecolor {inecolor175,9697
\definecolor {inecolor176,9754
\definecolor {inecolor177,9811
\definecolor {inecolor178,9868
\definecolor {inecolor179,9925
\definecolor {inecolor180,9982
\definecolor {inecolor181,10039
\definecolor {inecolor182,10096
\definecolor {inecolor183,10153
\definecolor {inecolor184,10210
\definecolor {inecolor185,10267
\definecolor {inecolor186,10324
\definecolor {inecolor187,10381
\definecolor {inecolor188,10438
\definecolor {inecolor189,10495
\definecolor {inecolor190,10552
\definecolor {inecolor191,10609
\definecolor {inecolor192,10666
\definecolor {inecolor193,10723
\definecolor {inecolor194,10780
\definecolor {inecolor195,10837
\definecolor {inecolor196,10894
\definecolor {inecolor197,10951
\definecolor {inecolor198,11008
\definecolor {inecolor199,11065
\definecolor {inecolor200,11122
\definecolor {inecolor201,11179
\definecolor {inecolor202,11236
\definecolor {inecolor203,11293
\definecolor {inecolor204,11350
\definecolor {inecolor205,11407
\definecolor {inecolor206,11464
\definecolor {inecolor207,11521
\definecolor {inecolor208,11578
\definecolor {inecolor209,11635
\definecolor {inecolor210,11692
\definecolor {inecolor211,11749
\definecolor {inecolor212,11806
\definecolor {inecolor213,11863
\definecolor {inecolor214,11920
\definecolor {inecolor215,11977
\definecolor {inecolor216,12034
\definecolor {inecolor217,12091
\definecolor {inecolor218,12148
\definecolor {inecolor219,12205
\definecolor {inecolor220,12262
\definecolor {inecolor221,12319
\definecolor {inecolor222,12376
\definecolor {inecolor223,12433
\definecolor {inecolor224,12490
\definecolor {inecolor225,12547
\definecolor {inecolor226,12604
\definecolor {inecolor227,12661
\definecolor {inecolor228,12718
\definecolor {inecolor229,12775
\definecolor {inecolor230,12832
\definecolor {inecolor231,12889
\definecolor {inecolor232,12946
\definecolor {inecolor233,13003
\definecolor {inecolor234,13060
\definecolor {inecolor235,13117
\definecolor {inecolor236,13174
\definecolor {inecolor237,13231
\definecolor {inecolor238,13288
\definecolor {inecolor239,13345
\definecolor {inecolor240,13402
\definecolor {inecolor241,13459
\definecolor {inecolor242,13516
\definecolor {inecolor243,13573
\definecolor {inecolor244,13630
\definecolor {inecolor245,13687
\definecolor {inecolor246,13744
\definecolor {inecolor247,13801
\definecolor {inecolor248,13858
\definecolor {inecolor249,13915
\definecolor {inecolor250,13972
\definecolor {inecolor251,14029
\definecolor {inecolor252,14086
\definecolor {inecolor253,14143
\definecolor {inecolor254,14200
\definecolor {inecolor255,14257
\definecolor {inecolor256,14314
\definecolor {inecolor257,14371
\definecolor {inecolor258,14428
\definecolor {inecolor259,14485
\definecolor {inecolor260,14542
\definecolor {inecolor261,14599
\definecolor {inecolor262,14656
\definecolor {inecolor263,14713
\definecolor {inecolor264,14770
\definecolor {inecolor265,14827
\definecolor {inecolor266,14884
\definecolor {inecolor267,14941
\definecolor {inecolor268,14998
\definecolor {inecolor269,15055
\definecolor {inecolor270,15112
\definecolor {inecolor271,15169
\definecolor {inecolor272,15226
\definecolor {inecolor273,15283
\definecolor {inecolor274,15340
\definecolor {inecolor275,15397
\definecolor {inecolor276,15454
\definecolor {inecolor277,15511
\definecolor {inecolor278,15568
\definecolor {inecolor279,15625
\definecolor {inecolor280,15682
\definecolor {inecolor281,15739
\definecolor {inecolor282,15796
\definecolor {inecolor283,15853
\definecolor {inecolor284,15910
\definecolor {inecolor285,15967
\definecolor {inecolor286,16024
\definecolor {inecolor287,16081
\definecolor {inecolor288,16138
\definecolor {inecolor289,16195
\definecolor {inecolor290,16252
\definecolor {inecolor291,16309
\definecolor {inecolor292,16366
\definecolor {inecolor293,16423
\definecolor {inecolor294,16480
\definecolor {inecolor295,16537
\definecolor {inecolor296,16594
\definecolor {inecolor297,16651
\definecolor {inecolor298,16708
\definecolor {inecolor299,16765
\definecolor {inecolor300,16822
\definecolor {inecolor301,16879
\definecolor {inecolor302,16936
\definecolor {inecolor303,16993
\definecolor {inecolor304,17050
\definecolor {inecolor305,17107
\definecolor {inecolor306,17164
\definecolor {inecolor307,17221
\definecolor {inecolor308,17278
\definecolor {inecolor309,17335
\definecolor {inecolor310,17392
\definecolor {inecolor311,17449
\definecolor {inecolor312,17506
\definecolor {inecolor313,17563
\definecolor {inecolor314,17620
\definecolor {inecolor315,17677
\definecolor {inecolor316,17734
\definecolor {inecolor317,17791
\definecolor {inecolor318,17848
\definecolor {inecolor319,17905
\definecolor {inecolor320,17962
\definecolor {inecolor321,18019
\definecolor {inecolor322,18076
\definecolor {inecolor323,18133
\definecolor {inecolor324,18190
\definecolor {inecolor325,18247
\definecolor {inecolor326,18304
\definecolor {inecolor327,18361
\definecolor {inecolor328,18418
\definecolor {inecolor329,18475
\definecolor {inecolor330,18532
\definecolor {inecolor331,18589
\definecolor {inecolor332,18646
\definecolor {inecolor333,18703
\definecolor {inecolor334,18760
\definecolor {inecolor335,18817
\definecolor {inecolor336,18874
\definecolor {inecolor337,18931
\definecolor {inecolor338,18988
\definecolor {inecolor339,19045
\definecolor {inecolor340,19102
\definecolor {inecolor341,19159
\definecolor {inecolor342,19216
\definecolor {inecolor343,19273
\definecolor {inecolor344,19330
\definecolor {inecolor345,19387
\definecolor {inecolor346,19444
\definecolor {inecolor347,19501
\definecolor {inecolor348,19558
\definecolor {inecolor349,19615
\definecolor {inecolor350,19672
\definecolor {inecolor351,19729
\definecolor {inecolor352,19786
\definecolor {inecolor353,19843
\definecolor {inecolor354,19900
\definecolor {inecolor355,19957
\definecolor {inecolor356,20014
\definecolor {inecolor357,20071
\definecolor {inecolor358,20128
\definecolor {inecolor359,20185
\definecolor {inecolor360,20242
\definecolor {inecolor361,20299
\definecolor {inecolor362,20356
\definecolor {inecolor363,20413
\definecolor {inecolor364,20470
\definecolor {inecolor365,20527
\definecolor {inecolor366,20584
\definecolor {inecolor367,20641
\definecolor {inecolor368,20698
\definecolor {inecolor369,20755
\definecolor {inecolor370,20812
\definecolor {inecolor371,20869
\definecolor {inecolor372,20926
\definecolor {inecolor373,20983
\definecolor {inecolor374,21040
\definecolor {inecolor375,21097
\definecolor {inecolor376,21154
\definecolor {inecolor377,21211
\definecolor {inecolor378,21268
\definecolor {inecolor379,21325
\definecolor {inecolor380,21382
\definecolor {inecolor381,21439
\definecolor {inecolor382,21496
\definecolor {inecolor383,21553
\definecolor {inecolor384,21610
\definecolor {inecolor385,21667
\definecolor {inecolor386,21724
\definecolor {inecolor387,21781
\definecolor {inecolor388,21838
\definecolor {inecolor389,21895
\definecolor {inecolor390,21952
\definecolor {inecolor391,22009
\definecolor {inecolor392,22066
\definecolor {inecolor393,22123
\definecolor {inecolor394,22180
\definecolor {inecolor395,22237
\definecolor {inecolor396,22294
\definecolor {inecolor397,22351
\definecolor {inecolor398,22408
\definecolor {inecolor399,22465
\definecolor {inecolor400,22522
\definecolor {inecolor401,22579
\definecolor {inecolor402,22636
\definecolor {inecolor403,22693
\definecolor {inecolor404,22750
\definecolor {inecolor405,22807
\definecolor {inecolor406,22864
\definecolor {inecolor407,22921
\definecolor {inecolor408,22978
\definecolor {inecolor409,23035
\definecolor {inecolor410,23092
\definecolor {inecolor411,23149
\definecolor {inecolor412,23206
\definecolor {inecolor413,23263
\definecolor {inecolor414,23320
\definecolor {inecolor415,23377
\definecolor {inecolor416,23434
\definecolor {inecolor417,23491
\definecolor {inecolor418,23548
\definecolor {inecolor419,23605
\definecolor {inecolor420,23662
\definecolor {inecolor421,23719
\definecolor {inecolor422,23776
\definecolor {inecolor423,23833
\definecolor {inecolor424,23890
\definecolor {inecolor425,23947
\definecolor {inecolor426,24004
\definecolor {inecolor427,24061
\definecolor {inecolor428,24118
\definecolor {inecolor429,24175
\definecolor {inecolor430,24232
\definecolor {inecolor431,24289
\definecolor {inecolor432,24346
\definecolor {inecolor433,24403
\definecolor {inecolor434,24460
\definecolor {inecolor435,24517
\definecolor {inecolor436,24574
\definecolor {inecolor437,24631
\definecolor {inecolor438,24688
\definecolor {inecolor439,24745
\definecolor {inecolor440,24802
\definecolor {inecolor441,24859
\definecolor {inecolor442,24916
\definecolor {inecolor443,24973
\definecolor {inecolor444,25030
\definecolor {inecolor445,25087
\definecolor {inecolor446,25144
\definecolor {inecolor447,25201
\definecolor {inecolor448,25258
\definecolor {inecolor449,25315
\definecolor {inecolor450,25372
\definecolor {inecolor451,25429
\definecolor {inecolor452,25486
\definecolor {inecolor453,25543
\definecolor {inecolor454,25600
\definecolor {inecolor455,25657
\definecolor {inecolor456,25714
\definecolor {inecolor457,25771
\definecolor {inecolor458,25828
\definecolor {inecolor459,25885
\definecolor {inecolor460,25942
\definecolor {inecolor461,25999
\definecolor {inecolor462,26056
\definecolor {inecolor463,26113
\definecolor {inecolor464,26170
\definecolor {inecolor465,26227
\definecolor {inecolor466,26284
\definecolor {inecolor467,26341
\definecolor {inecolor468,26398
\definecolor {inecolor469,26455
\definecolor {inecolor470,26512
\definecolor {inecolor471,26569
\definecolor {inecolor472,26626
\definecolor {inecolor473,26683
\definecolor {inecolor474,26740
\definecolor {inecolor475,26797
\definecolor {inecolor476,26854
\definecolor {inecolor477,26911
\definecolor {inecolor478,26968
\definecolor {inecolor479,27025
\definecolor {inecolor480,27082
\definecolor {inecolor481,27139
\definecolor {inecolor482,27196
\definecolor {inecolor483,27253
\definecolor {inecolor484,27310
\definecolor {inecolor485,27367
\definecolor {inecolor486,27424
\definecolor {inecolor487,27481
\definecolor {inecolor488,27538
\definecolor {inecolor489,27595
\definecolor {inecolor490,27652
\definecolor {inecolor491,27709
\definecolor {inecolor492,27766
\definecolor {inecolor493,27823
\definecolor {inecolor494,27880
\definecolor {inecolor495,27937
\definecolor {inecolor496,27994
\definecolor {inecolor497,28051
\definecolor {inecolor498,28108
\definecolor {inecolor499,28165
\definecolor {inecolor500,28222
\definecolor {inecolor501,28279
\definecolor {inecolor502,28336
\definecolor {inecolor503,28393
\definecolor {inecolor504,28450
\definecolor {inecolor505,28507
\definecolor {inecolor506,28564
\definecolor {inecolor507,28621
\definecolor {inecolor508,28678
\definecolor {inecolor509,28735
\definecolor {inecolor510,28792
\definecolor {inecolor511,28849
\definecolor {inecolor512,28906
\definecolor {inecolor513,28963
\definecolor {inecolor514,29020
\definecolor {inecolor515,29077
\definecolor {inecolor516,29134
\definecolor {inecolor517,29191
\definecolor {inecolor518,29248
\definecolor {inecolor519,29305

rs_macros_colors.tex,390
\newcommand<>{<>28,1245
\newcommand<>{<>29,1282
\newcommand<>{<>30,1323
\newcommand<>{<>31,1371
\newcommand<>{<>32,1406
\newcommand<>{<>33,1449
\newcommand<>{<>34,1498
\newcommand<>{<>35,1539
\newcommand<>{<>36,1588
\newcommand<>{<>37,1633
\newcommand<>{<>38,1679
\newcommand<>{<>39,1716
\newcommand<>{<>40,1755
\newcommand<>{<>41,1794
\newcommand<>{<>42,1835

rs_macros_dl.tex,2455
\newcommand{\en}\en7,256
\newcommand{\den}\den8,287
\newcommand{\mc}\mc10,334
\newcommand{\msf}\msf11,381
\newcommand{\snomed}\snomed13,429
\newcommand{\geneonto}\geneonto14,477
\newcommand{\nci}\nci15,530
\newcommand{\galen}\galen16,569
\newcommand{\shsnomed}\shsnomed18,613
\newcommand{\shnci}\shnci19,663
\newcommand{\shgalen}\shgalen20,705
\newcommand{\shfullgalen}\shfullgalen21,753
\newcommand{\shgeneontology}\shgeneontology22,808
\newcommand{\conj}\conj24,866
\newcommand{\disj}\disj25,893
\newcommand{\exr}\exr26,920
\newcommand{\subs}\subs28,958
\newcommand{\sups}\sups29,990
\newcommand{\norm}\norm30,1022
\newcommand{\comp}\comp31,1053
\newcommand{\topt}\topt33,1080
\newcommand{\bott}\bott34,1125
\newcommand{\conjt}\conjt35,1170
\newcommand{\disjt}\disjt36,1227
\newcommand{\exrt}\exrt37,1284
\newcommand{\equivt}\equivt38,1342
\newcommand{\subst}\subst39,1400
\newcommand{\supst}\supst40,1462
\newcommand{\pr}\pr44,1639
\newcommand{\prc}\prc45,1687
\newcommand{\sel}\sel46,1738
\newcommand{\selc}\selc47,1787
\newcommand{\goal}\goal49,1840
\newcommand{\goalsure}\goalsure50,1896
\newcommand{\tgoal}\tgoal51,1957
\newcommand{\igoal}\igoal52,2019
\newcommand{\sgoal}\sgoal53,2088
\newcommand{\isgoal}\isgoal54,2142
\newcommand{\nsgoal}\nsgoal55,2205
\newcommand{\assumptiongoal}\assumptiongoal57,2275
\newcommand{\assumptionsgoal}\assumptionsgoal58,2353
\newcommand{\aenc}\aenc60,2420
\newcommand{\wffsubs}\wffsubs61,2476
\newcommand{\wffsubsnotrans}\wffsubsnotrans62,2531
\newcommand{\wffmina}\wffmina63,2603
\newcommand{\wffminarule}\wffminarule64,2661
\newcommand{\wffminaT}\wffminaT65,2728
\newcommand{\wffminaTrule}\wffminaTrule66,2791
\newcommand{\wffallmina}\wffallmina67,2858
\newcommand{\wffallminarule}\wffallminarule68,2919
\newcommand{\wffallminaT}\wffallminaT69,2991
\newcommand{\wffallminaTrule}\wffallminaTrule70,3057
\newcommand{\wffallminaO}\wffallminaO71,3132
\newcommand{\wffallminaruleO}\wffallminaruleO72,3197
\newcommand{\pinpointingwff}\pinpointingwff74,3271
\newcommand{\pinpointingwffall}\pinpointingwffall75,3334
\newcommand{\hatT}\hatT77,3399
\newcommand{\Tp}\Tp78,3448
\newcommand{\elsat}\elsat80,3513
\newcommand{\el}\el96,3577
\newcommand{\elh}\elh97,3628
\newcommand{\elp}\elp98,3681
\newcommand{\elpp}\elpp99,3737
\newcommand{\eloh}\eloh100,3795
\newcommand{\eqdef}\eqdef101,3850

rs_macros_general.tex,2137
\newcommand{\RSHIGHLIGHT}\RSHIGHLIGHT15,499
\newcommand{\new}\new20,643
\newcommand{\ex}\ex21,678
\newcommand{\TODO}\TODO25,809
\newcommand{\ACTODO}\ACTODO26,835
\newcommand{\RS}\RS27,904
\newcommand{\ignore}\ignore28,946
\newcommand{\RSCHANGE}\RSCHANGE32,1124
\newcommand{\RSTODO}\RSTODO33,1179
\newcommand{\nota}\nota36,1316
\newcommand{\marg}\marg37,1373
\renewcommand{\marg}\marg38,1423
\newenvironment{rschange}rschange40,1496
\newcommand{\RSNOTE}\RSNOTE42,1551
\renewcommand{\RSNOTE}\RSNOTE44,1650
 \newcommand{\ignoreinshort}\ignoreinshort47,1738
 \newcommand{\ignoreinlong}\ignoreinlong48,1772
\def\makenewenumerate#1#2{\makenewenumerate54,1980
\newenvironment{#1}%56,2027
 \setlength{\labelwidth}width61,2175
\def\newplaintheorem#1#2{\newplaintheorem75,2713
\newenvironment{#1}{\begin{#1plain}\rm }{\end{#1plain}}}77,2775
\newcommand{\sref}\sref98,3488
\newcommand{\noi}\noi99,3524
\newcommand{\pair}\pair105,3651
\newcommand{\triple}\triple106,3718
\newcommand{\tuple}\tuple107,3792
\newcommand{\set}\set108,3855
\newcommand{\imp}\imp109,3906
\newcommand{\limp}\limp110,3957
\renewcommand{\iff}\iff111,4008
\newcommand{\defas}\defas112,4065
\newcommand{\thus}\thus113,4137
\newcommand{\pos}\pos115,4194
\newcommand\cala{\cala123,4346
\newcommand\calb{\calb124,4396
\newcommand\calc{\calc125,4446
\newcommand\cald{\cald126,4496
\newcommand\cale{\cale127,4546
\newcommand\calf{\calf128,4596
\newcommand\calg{\calg129,4646
\newcommand\calh{\calh130,4696
\newcommand\cali{\cali131,4746
\newcommand\calj{\calj132,4796
\newcommand\calk{\calk133,4846
\newcommand\call{\call134,4896
\newcommand\calm{\calm135,4946
\newcommand\caln{\caln136,4996
\newcommand\calo{\calo137,5046
\newcommand\calp{\calp138,5096
\newcommand\calq{\calq139,5146
\newcommand\calr{\calr140,5196
\newcommand\cals{\cals141,5246
\newcommand\calt{\calt142,5296
\newcommand\calu{\calu143,5346
\newcommand\calv{\calv144,5396
\newcommand\calw{\calw145,5446
\newcommand\calx{\calx146,5496
\newcommand\caly{\caly147,5546
\newcommand\calz{\calz148,5596

rs_macros_mc.tex,1492
\newcommand{\nusmv}\nusmv7,256
\newcommand{\PROMELA}\PROMELA8,289
\newcommand{\smv}\smv9,326
\newcommand{\bdds}\bdds11,356
\newcommand{\bdd}\bdd12,395
\newcommand{\dis}\dis14,466
\newcommand{\con}\con15,490
\newcommand{\liff}\liff16,516
\newcommand{\true}\true17,552
\newcommand{\false}\false18,577
\newcommand{\CTL}\CTL19,603
\newcommand{\LTL}\LTL20,642
\newcommand{\E}\E26,700
\newcommand{\A}\A27,727
\newcommand{\G}\G28,754
\newcommand{\F}\F29,781
\newcommand{\U}\U30,808
\newcommand{\R}\R31,835
\newcommand{\X}\X32,862
\newcommand{\AG}\AG33,889
\newcommand{\AF}\AF34,918
\newcommand{\AU}\AU35,947
\newcommand{\AR}\AR36,976
\newcommand{\AX}\AX37,1005
\newcommand{\EG}\EG38,1034
\newcommand{\EF}\EF39,1063
\newcommand{\EU}\EU40,1092
\newcommand{\ER}\ER41,1121
\newcommand{\EX}\EX42,1150
\newcommand{\n}\n44,1180
\newcommand{\kil}\kil45,1212
\newcommand{\ki}\ki46,1257
\renewcommand{\k}\k47,1293
\newcommand{\kl}\kl48,1328
\newcommand{\fkil}\fkil50,1365
\newcommand{\fki}\fki51,1404
\newcommand{\fk}\fk52,1440
\newcommand{\fkl}\fkl53,1470
\newcommand{\gkil}\gkil55,1507
\newcommand{\gki}\gki56,1546
\newcommand{\gk}\gk57,1582
\newcommand{\gkl}\gkl58,1612
\newcommand{\Lkl}\Lkl60,1649
\newcommand{\Lkkll}\Lkkll61,1686
\newcommand{\Lkll}\Lkll62,1726
\newcommand{\Lk}\Lk63,1760
\newcommand{\Mkil}\Mkil65,1787
\newcommand{\Mki}\Mki66,1830
\newcommand{\Mk}\Mk67,1870
\newcommand{\Mkl}\Mkl68,1907

rs_macros_optsmt.tex,4994
\newcommand{\omtproblem}\omtproblem17,461
\newcommand{\omt}\omt18,525
\newcommand{\bomt}\bomt19,575
\newcommand{\omtt}\omtt20,627
\newcommand{\bomtt}\bomtt21,684
\newcommand{\costfs}\costfs24,767
\newcommand{\costfgen}\costfgen25,827
\newcommand{\costfi}\costfi26,886
\newcommand{\costfone}\costfone27,921
\newcommand{\costfM}\costfM28,958
\newcommand{\costs}\costs31,1017
\newcommand{\costgen}\costgen32,1072
\newcommand{\costi}\costi33,1127
\newcommand{\costone}\costone34,1160
\newcommand{\costM}\costM35,1195
\newcommand{\vvgen}\vvgen38,1253
\newcommand{\vvi}\vvi39,1315
\newcommand{\wvgen}\wvgen40,1351
\newcommand{\wvi}\wvi41,1413
\newcommand{\xvgen}\xvgen42,1449
\newcommand{\xvi}\xvi43,1511
\newcommand{\yvgen}\yvgen44,1547
\newcommand{\yvi}\yvi45,1609
\newcommand{\lbgen}\lbgen49,1663
\newcommand{\ubgen}\ubgen50,1726
\newcommand{\ub}\ub51,1789
\newcommand{\lbi}\lbi52,1818
\newcommand{\ubi}\ubi53,1849
\newcommand{\lbone}\lbone54,1880
\newcommand{\ubone}\ubone55,1913
\newcommand{\lbM}\lbM56,1946
\newcommand{\ubM}\ubM57,1977
\newcommand{\lbigen}\lbigen58,2008
\newcommand{\ubigen}\ubigen59,2049
\newcommand{\lbimax}\lbimax60,2090
\newcommand{\ubimin}\ubimin61,2127
\newcommand{\lbonemax}\lbonemax62,2164
\newcommand{\ubonemin}\ubonemin63,2203
\newcommand{\tpredgen}\tpredgen66,2258
\newcommand{\tpredigen}\tpredigen67,2322
\newcommand{\tpredij}\tpredij68,2367
\newcommand{\predgen}\predgen69,2404
\newcommand{\predigen}\predigen70,2464
\newcommand{\predij}\predij71,2507
\newcommand{\predonej}\predonej72,2542
\newcommand{\Agen}\Agen75,2651
\newcommand{\Aj}\Aj76,2701
\newcommand{\aij}\aij77,2728
\newcommand{\bi}\bi78,2780
\newcommand{\cj}\cj79,2830
\newcommand{\ddj}\ddj80,2880
\newcommand{\lj}\lj81,2931
\newcommand{\cgen}\cgen84,2999
\newcommand{\cigen}\cigen85,3064
\newcommand{\cijgen}\cijgen86,3129
\newcommand{\cijone}\cijone87,3194
\newcommand{\cijtwo}\cijtwo88,3255
\newcommand{\cij}\cij89,3316
\newcommand{\conej}\conej90,3373
\newcommand{\cc}\cc92,3433
\newcommand{\bounds}\bounds95,3483
\newcommand{\boundi}\boundi96,3548
\newcommand{\icost}\icost98,3615
\newcommand{\icostgen}\icostgen99,3665
\newcommand{\icosti}\icosti101,3798
\newcommand{\icostij}\icostij102,3864
\newcommand{\icostonej}\icostonej103,3919
\newcommand{\bcost}\bcost105,3986
\newcommand{\cost}\cost106,4036
\newcommand{\mincost}\mincost107,4083
\newcommand{\bound}\bound108,4136
\newcommand{\guess}\guess109,4185
\newcommand{\oldguess}\oldguess110,4234
\newcommand{\oldbound}\oldbound111,4289
\newcommand{\maxboundi}\maxboundi112,4344
\newcommand{\maxboundone}\maxboundone113,4411
\newcommand{\nextsmallerbound}\nextsmallerbound114,4480
\newcommand{\noroom}\noroom115,4551
\newcommand{\mustbe}\mustbe116,4602
\newcommand{\bleft}\bleft117,4653
\newcommand{\bright}\bright118,4702
\newcommand{\pending}\pending119,4752
\newcommand{\tite}\tite121,4810
\newcommand{\ite}\ite122,4856
\newcommand{\costof}\costof124,4902
\newcommand{\costiof}\costiof125,4969
\newcommand{\mcostof}\mcostof126,5010
\newcommand{\mcostiof}\mcostiof127,5079
\newcommand{\C}\C131,5144
\newcommand{\Clemma}\Clemma132,5193
\newcommand{\Csolver}\Csolver133,5231
\newcommand{\TC}\TC137,5273
\newcommand{\incsmttc}\incsmttc139,5403
\newcommand{\smttcost}\smttcost140,5475
\newcommand{\smttc}\smttc141,5539
\newcommand{\smtc}\smtc142,5598
\newcommand{\Tlaint}\Tlaint143,5655
\newcommand{\smttlaint}\smttlaint144,5710
\newcommand{\optsmttc}\optsmttc147,5782
\newcommand{\decproblem}\decproblem149,5847
\newcommand{\optproblem}\optproblem150,5921
\newcommand{\vic}\vic153,5999
\newcommand{\muc}\muc156,6064
\newcommand{\mucgen}\mucgen157,6112
\newcommand{\muci}\muci158,6171
\newcommand{\mut}\mut159,6202
\newcommand{\mub}\mub160,6250
\newcommand{\Jplus}\Jplus163,6317
\newcommand{\Jminus}\Jminus164,6365
\newcommand{\Kplus}\Kplus165,6414
\newcommand{\Kminus}\Kminus166,6462
\newcommand{\Kplusone}\Kplusone167,6511
\newcommand{\Kminusone}\Kminusone168,6562
\newcommand{\Ilaint}\Ilaint172,6636
\newcommand{\IT}\IT173,6693
\newcommand{\I}\I174,6742
\newcommand{\mathsatC}\mathsatC177,6805
\newcommand{\scip}\scip178,6838
\newcommand{\bsolo}\bsolo179,6876
\newcommand{\satforj}\satforj180,6916
\newcommand{\pbclasp}\pbclasp181,6958
\newcommand{\bl}\bl184,7015
\newcommand\mysout{\mysout190,7136
\newcommand\nosout{\nosout191,7188
\definecolor{inecolor192,7240
\definecolor{inecolor193,7282
\def \gbox #1{\gbox194,7325
\newcommand{\fal}\fal195,7364
\newcommand{\tru}\tru196,7416
\newcommand{\mycite}\mycite198,7449
\newcommand{\mcite}\mcite199,7517
\newcommand{\mueuf}\mueuf202,7614
\newcommand{\mulaint}\mulaint203,7666
\newcommand{\infrule}\infrule204,7722
\newcommand{\hyp}\hyp205,7788
\newcommand{\comb}\comb206,7827
\newcommand{\fakeinfrule}\fakeinfrule208,7869

rs_macros_sat.tex,1261
\newcommand{\dpll}\dpll13,424
\newcommand{\zchaff}\zchaff17,541
\newcommand{\satelite}\satelite18,590
\newcommand{\siege}\siege19,642
\newcommand{\berkmin}\berkmin20,690
\newcommand{\minisat}\minisat21,740
\newcommand{\minisattwo}\minisattwo22,790
\newcommand{\pickassign}\pickassign28,924
\newcommand{\picknewassign}\picknewassign29,992
\newcommand{\picktotalassign}\picktotalassign30,1075
\newcommand{\decidebranch}\decidebranch31,1151
\newcommand{\decide}\decide32,1224
\newcommand{\blevel}\blevel33,1278
\newcommand{\analyzeconflict}\analyzeconflict34,1332
\newcommand{\analyzededuction}\analyzededuction35,1406
\newcommand{\backtrack}\backtrack36,1482
\newcommand{\bcp}\bcp37,1542
\newcommand{\satres}\satres40,1637
\newcommand{\unsatres}\unsatres41,1679
\newcommand{\unknownres}\unknownres42,1725
\newcommand{\conflres}\conflres43,1775
\newcommand{\walksat}\walksat46,1858
\newcommand{\basicwalksmt}\basicwalksmt47,1896
\newcommand{\walksmt}\walksmt48,1954
\newcommand{\tpreprocess}\tpreprocess50,2002
\newcommand{\initialtruthassignment}\initialtruthassignment51,2058
\newcommand{\chooseunsatisfiedclause}\chooseunsatisfiedclause52,2132
\newcommand{\nexttruthassignment}\nexttruthassignment53,2208

rs_macros_smt.tex,4995
\newcommand{\proptofol}\proptofol16,473
\newcommand{\foltoprop}\foltoprop17,536
\newcommand{\btot}\btot18,599
\newcommand{\ttob}\ttob19,630
\newcommand{\vi}\vi27,934
\newcommand{\vip}\vip28,980
\newcommand{\mup}\mup29,1029
\newcommand{\muone}\muone30,1074
\newcommand{\mutwo}\mutwo31,1121
\newcommand{\muonetwo}\muonetwo32,1168
\newcommand{\taup}\taup33,1229
\newcommand{\etap}\etap34,1276
\newcommand{\cp}\cp35,1323
\newcommand{\atoms}\atoms37,1366
\newcommand{\T}\T42,1496
\newcommand{\Tone}\Tone43,1545
\newcommand{\Ttwo}\Ttwo44,1590
\newcommand{\Tonetwo}\Tonetwo45,1635
\newcommand{\smt}\smt46,1694
\newcommand{\smtt}\smtt47,1724
\newcommand{\smttt}\smttt48,1779
\newcommand{\smttonettwo}\smttonettwo49,1838
\newcommand{\Ti}\Ti50,1906
\newcommand{\tmany}\tmany51,1949
\newcommand{\smtmany}\smtmany52,2005
\newcommand{\utvpi}\utvpi54,2078
\newcommand{\utvpiint}\utvpiint55,2135
\newcommand{\utvpirat}\utvpirat56,2207
\newcommand{\bool}\bool57,2279
\newcommand{\euf}\euf58,2334
\newcommand{\eq}\eq59,2387
\newcommand{\dl}\dl60,2437
\newcommand{\dlrat}\dlrat61,2488
\newcommand{\dlint}\dlint62,2554
\newcommand{\la}\la63,2620
\newcommand{\larat}\larat64,2671
\newcommand{\laint}\laint65,2737
\newcommand{\nla}\nla66,2803
\newcommand{\nlarat}\nlarat67,2855
\newcommand{\nlaint}\nlaint68,2923
\newcommand{\bv}\bv69,2991
\newcommand{\mem}\mem70,3042
\newcommand{\lists}\lists71,3094
\newcommand{\tonetwo}\tonetwo72,3148
\newcommand{\smteuf}\smteuf74,3205
\newcommand{\smtdl}\smtdl75,3240
\newcommand{\smtdlrat}\smtdlrat76,3273
\newcommand{\smtdlint}\smtdlint77,3312
\newcommand{\smtutvpi}\smtutvpi78,3351
\newcommand{\smtutvpirat}\smtutvpirat79,3390
\newcommand{\smtutvpiint}\smtutvpiint80,3435
\newcommand{\smtla}\smtla81,3480
\newcommand{\smtlarat}\smtlarat82,3513
\newcommand{\smtlaint}\smtlaint83,3552
\newcommand{\smtbv}\smtbv84,3591
\newcommand{\smtmem}\smtmem85,3624
\newcommand{\genmodels}\genmodels88,3661
\newcommand{\Tmodels}\Tmodels89,3702
\newcommand{\laratmodels}\laratmodels90,3738
\newcommand{\laintmodels}\laintmodels91,3782
\newcommand{\lamodels}\lamodels92,3826
\newcommand{\dlmodels}\dlmodels93,3864
\newcommand{\dlintmodels}\dlintmodels94,3902
\newcommand{\dlratmodels}\dlratmodels95,3946
\newcommand{\pmodels}\pmodels96,3990
\newcommand{\TsolverGen}\TsolverGen100,4099
\newcommand{\TsolversGen}\TsolversGen101,4169
\newcommand{\Tsolver}\Tsolver102,4241
\newcommand{\Tsolvers}\Tsolvers103,4280
\newcommand{\Psolver}\Psolver104,4321
\newcommand{\TTsolver}\TTsolver105,4371
\newcommand{\Tonesolver}\Tonesolver106,4427
\newcommand{\Ttwosolver}\Ttwosolver107,4485
\newcommand{\Tonetwosolver}\Tonetwosolver108,4543
\newcommand{\Tisolver}\Tisolver109,4614
\newcommand{\Tisolvers}\Tisolvers110,4668
\newcommand{\TdeduceGen}\TdeduceGen111,4724
\newcommand{\Tonededuce}\Tonededuce112,4794
\newcommand{\Ttwodeduce}\Ttwodeduce113,4852
\newcommand{\Tlemma}\Tlemma115,4911
\newcommand{\Tlemmas}\Tlemmas116,4949
\newcommand{\Tilemma}\Tilemma117,4989
\newcommand{\Tilemmas}\Tilemmas118,5029
\newcommand{\argolib}\argolib125,5150
\newcommand{\barcelogic}\barcelogic126,5197
\newcommand{\blast}\blast127,5250
\newcommand{\clp}\clp128,5293
\newcommand{\csisat}\csisat129,5339
\newcommand{\cvcthree}\cvcthree130,5384
\newcommand{\foci}\foci131,5429
\newcommand{\haRVey}\haRVey132,5470
\newcommand{\intjain}\intjain133,5515
\newcommand{\lifter}\lifter134,5559
\newcommand{\mathsat}\mathsat135,5604
\newcommand{\verifun}\verifun136,5651
\newcommand{\yices}\yices137,5699
\newcommand{\zapato}\zapato138,5742
\newcommand{\zap}\zap139,5789
\newcommand{\zthree}\zthree140,5828
\newcommand{\mathsatfour}\mathsatfour142,5870
\newcommand{\mathsatfive}\mathsatfive143,5922
\newcommand{\myeij}\myeij147,6059
\newcommand{\myeijs}\myeijs148,6107
\newcommand{\mynegeij}\mynegeij149,6157
\newcommand{\eij}\eij150,6213
\newcommand{\eik}\eik151,6260
\newcommand{\ejk}\ejk152,6307
\newcommand{\diseij}\diseij153,6354
\newcommand{\NO}\NO155,6408
\newcommand{\Bool}\Bool156,6467
\newcommand{\BoolGen}\BoolGen157,6521
\newcommand{\BoolT}\BoolT158,6586
\newcommand{\BoolTonetwo}\BoolTonetwo159,6619
\newcommand{\BoolTi}\BoolTi160,6664
\newcommand{\BoolNO}\BoolNO161,6702
\newcommand{\DelBoolNO}\DelBoolNO162,6738
\newcommand{\TsatisfiableGen}\TsatisfiableGen164,6820
\newcommand{\TsatGen}\TsatGen165,6900
\newcommand{\TunsatGen}\TunsatGen166,6964
\newcommand{\Tonesat}\Tonesat167,7032
\newcommand{\Ttwosat}\Ttwosat168,7082
\newcommand{\Toneunsat}\Toneunsat169,7132
\newcommand{\Ttwounsat}\Ttwounsat170,7186
\newcommand{\Tsatisfiable}\Tsatisfiable171,7240
\newcommand{\Psatisfiable}\Psatisfiable172,7288
\newcommand{\Tonesatisfiable}\Tonesatisfiable173,7348
\newcommand{\Ttwosatisfiable}\Ttwosatisfiable174,7414
\newcommand{\Tisatisfiable}\Tisatisfiable175,7480

st_macros.tex,2860
\newcommand{\sttodo}\sttodo1,0
\newcommand{\STNOTE}\STNOTE2,84
\newenvironment{stnote}stnote3,141
\newenvironment{stchange}stchange4,194
\newcommand{\best}\best6,255
\newcommand{\optmathsat}\optmathsat13,475
\newcommand{\optmathsatv}\optmathsatv14,529
\newcommand{\pboptmathsat}\pboptmathsat19,742
\newcommand{\mathsatv}\mathsatv20,791
\newcommand{\pboptmathsatv}\pboptmathsatv21,850
\newcommand{\renc}\renc25,988
\newcommand{\denc}\denc26,1033
\newcommand{\encone}\encone27,1078
\newcommand{\enctwo}\enctwo28,1129
\newcommand{\dirgenerated}\dirgenerated34,1255
\newcommand{\encoded}\encoded35,1313
\newcommand{\oneencoded}\oneencoded36,1355
\newcommand{\twoencoded}\twoencoded37,1408
\newcommand{\bin}\bin43,1522
\newcommand{\lin}\lin44,1562
\newcommand{\ada}\ada45,1602
\newcommand{\of}\of46,1642
\newcommand{\inl}\inl47,1680
\newcommand{\binof}\binof49,1720
\newcommand{\linof}\linof50,1765
\newcommand{\adaof}\adaof51,1810
\newcommand{\binin}\binin53,1856
\newcommand{\linin}\linin54,1901
\newcommand{\adain}\adain55,1946
\newcommand{\bininm}\bininm57,1992
\newcommand{\lininm}\lininm58,2043
\newcommand{\adainm}\adainm59,2094
\newcommand{\optlinof}\optlinof64,2232
\newcommand{\optbinof}\optbinof65,2284
\newcommand{\optadaof}\optadaof66,2336
\newcommand{\optlinin}\optlinin69,2406
\newcommand{\optbinin}\optbinin70,2458
\newcommand{\optadain}\optadain71,2510
\newcommand{\optlininm}\optlininm74,2601
\newcommand{\optbininm}\optbininm75,2655
\newcommand{\optadainm}\optadainm76,2709
\newcommand{\optpblin}\optpblin79,2777
\newcommand{\optpbbin}\optpbbin80,2829
\newcommand{\shortoptlinof}\shortoptlinof84,2911
\newcommand{\shortoptbinof}\shortoptbinof85,2970
\newcommand{\shortoptadaof}\shortoptadaof86,3029
\newcommand{\shortoptlinin}\shortoptlinin89,3116
\newcommand{\shortoptbinin}\shortoptbinin90,3175
\newcommand{\shortoptadain}\shortoptadain91,3234
\newcommand{\gams}\gams98,3451
\newcommand{\logmip}\logmip99,3492
\newcommand{\jams}\jams101,3538
\newcommand{\emp}\emp102,3579
\newcommand{\jamsG}\jamsG104,3619
\newcommand{\logmipG}\logmipG105,3667
\newcommand{\logmipCH}\logmipCH107,3720
\newcommand{\logmipBM}\logmipBM108,3777
\newcommand{\jamsCH}\jamsCH110,3835
\newcommand{\jamsBM}\jamsBM111,3888
\newcommand{\shortlogmipCH}\shortlogmipCH115,3953
\newcommand{\shortlogmipBM}\shortlogmipBM116,4009
\newcommand{\shortjamsCH}\shortjamsCH118,4066
\newcommand{\shortjamsBM}\shortjamsBM119,4118
\newcommand{\bmc}\bmc126,4315
\newcommand{\kind}\kind127,4354
\newcommand{\Deltaublin}\Deltaublin129,4397
\newcommand{\Deltaubbin}\Deltaubbin130,4460
\newcommand{\Deltanconflin}\Deltanconflin132,4524
\newcommand{\Deltanconfbin}\Deltanconfbin133,4600
\newcommand{\step}\step135,4677
\newcommand{\mode}\mode136,4728

tocl_main.tex,2688
\renewcommand{\topfraction}\topfraction8,140
\renewcommand{\bottomfraction}\bottomfraction9,171
\renewcommand{\textfraction}\textfraction10,205
\newcommand{\mytitle}\mytitle54,1141
\newcommand{\newreptheorem}\newreptheorem136,2824
\newenvironment{rep#1}[1]{%rep137,2857
 \def\rep@title{\rep@title138,2885
\section{Introduction}Introduction172,3510
\label{sec:intro}sec:intro173,3533
\section{Background}Background180,3614
\label{sec:background}sec:background181,3635
 \subsection{Linear Generalized Disjunctive Programming}Linear182,3676
 \label{sec:background_lgdp}sec:background_lgdp183,3733
\subsection{SAT and CDCL SAT Solvers}SAT184,3785
\label{sec:background_sat}sec:background_sat185,3823
\subsection{SMT and Lazy SMT Solvers}SMT186,3872
\label{sec:background_smt}sec:background_smt187,3910
\section{Optimization in \smtlaratplus }Optimization190,4000
\label{sec:optsmt}sec:optsmt192,4072
\section{Procedures for \omlarat and \omlaratplus} Procedures194,4135
\label{sec:algorithms}sec:algorithms195,4187
\subsection{An Offline Schema for \omlarat }An196,4228
\label{sec:algorithms_offline}sec:algorithms_offline197,4273
\subsection{An Inline Schema for \omlarat}An199,4340
\label{sec:algorithms_inline}sec:algorithms_inline200,4383
\subsection{Extensions to \omlaratplus}  Extensions202,4441
\label{sec:algorithms_omlaratplus}sec:algorithms_omlaratplus203,4483
\section{Experimental Evaluation}Experimental208,4630
\label{sec:expeval}sec:expeval209,4664
\subsection{Encodings.}Encodings.211,4701
\label{sec:expeval_enc}sec:expeval_enc212,4725
\subsection{Comparison on LGDP Problems}Comparison214,4770
\label{sec:expeval_lgdp}sec:expeval_lgdp215,4811
\subsubsection{The strip-packing problem.}The216,4856
\label{sec:expeval_sp}sec:expeval_sp217,4899
\subsubsection{The zero-wait jobshop problem.}The218,4945
\label{sec:expeval_js}sec:expeval_js219,4992
\subsubsection{Discussion.}Discussion.220,5038
\label{sec:expeval_disc}sec:expeval_disc221,5066
\subsection{Comparison on SMT-LIB Problems}Comparison222,5116
\label{sec:expeval_smtlib}sec:expeval_smtlib223,5160
\subsection{Comparison on SAL Problems}Comparison224,5209
\label{sec:expeval_sal}sec:expeval_sal225,5249
\subsection{Comparison on Pseudo-Boolean SMT Problems}Comparison227,5294
\label{sec:expeval_pb}sec:expeval_pb228,5349
\section{Related work.} %Related235,5510
\label{sec:related}sec:related236,5536
\section{Conclusions and Future Work}Conclusions241,5620
\label{sec:concl}sec:concl242,5658
\appendix252,5896
\section{Appendix: Proof of the Theorems}Appendix:253,5906
\label{sec:appendix}sec:appendix254,5948

todo.tex,17
\section*{*1,0

plan.tex,0

expeval_smtlib_table.tex,0

expeval_sal_table.tex,0

expeval_pb_table.tex,0

expeval_lgdp_sp_table.tex,0

expeval_lgdp_js_table.tex,0

abstract.tex,0


==> algo_binsearch.tex <==
\begin{algorithm}[t]
\caption{\omlarat Procedure based on mixed Linear/Binary Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:binsearch}
}
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE $\langle \varphi, \cost, \lb, \ub \rangle$ $\{$\ub can be $+\infty$$\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
%\isminimum \leftarrow false;
\calm \leftarrow \emptyset
$ \label{algobin:init}
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$
% $ \varphicost \leftarrow \varphi \cup\set \neg(\cost < \currlb)
% \wedge (\cost < \currub)$ 
\label{algobin:constraints}
% \STATE $ \varphicost \leftarrow \varphi  \wedge \neg (\cost < \lb ) \wedge (\cost < \ub)$
% \STATE $\currlb\leftarrow \lb; 
% \currub \leftarrow\ub;
% \isminimum \leftarrow false$
%\STATE $\mincost \leftarrow \currub$  
\WHILE{($\currlb < \currub $ )} \label{algobin:while}
   \IF{(\dopivoting{})} \label{algobin:pivoting}
     \STATE $\pivot \leftarrow \computepivot{}(\currlb,\currub)$ 
%     \STATE $\pivot \leftarrow (\currlb + \currub)/2$ 
     \STATE $\pivotatom \leftarrow (\cost < \pivot)$ 
     \STATE $\vi \leftarrow \vi \cup\set{ \pivotatom}$
   \ENDIF \label{algobin:endpivoting}
   \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmt(\varphicost)$ \label{algobin:smtsolver}
   \IF{$(\status = \satres)$}
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algobin:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}
$ 
\label{algobin:add}
   \ELSE[\status = \unsatres]
   \IF{$({\pivotatom \not\in \eta}) $} 
      \STATE $\currlb \leftarrow \currub$ \label{algobin:end}
   \ELSE %[{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}] 
     \STATE $\currlb \leftarrow \pivot$ \label{algobin:lbound}
     \STATE $\varphicost \leftarrow \varphicost \setminus \set{\pivotatom}$\label{algobin:poppivot}   
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algobin:pushnegpivot}    
   \ENDIF
   \ENDIF
\ENDWHILE
\label{algobin:endwhile}
\RETURN $\pair{\calm}{\currub}$ \label{algobin:return}
\end{algorithmic}
\end{algorithm}
%\vspace{-1.5cm}


==> algo_binsearch.tex.1 <==
% input: phi, lb, ub, eps
% phi = phi & !(cost < lb) & (cost < ub)
% l=lb;u=ub;
% do  {
%   p=(u+l)/2;pivot = (cost < p);
%   <res,mu,confl> = MATHSAT(phi,{pivot})
%   if (res==SAT) {
%     u = mincost(mu);
%     phi = phi & (cost < u) & pivot);
%   }
%   else if (confl=={pivot}) {
%     l = p;
%     phi = phi & !pivot;
%   }
%   else { // res==UNSAT, confl=={}
%     SAT=False;
%   }
% } while (SAT)
% return u;
\begin{algorithm}[t]
\caption{\omlarat Procedure based on mixed Linear/Binary Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:binsearch}
}
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE $\langle \varphi, \cost, \lb, \ub \rangle$ $\{$\ub can be $+\infty$$\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
\isminimum \leftarrow false;
\calm \leftarrow \emptyset
$ \label{algobin:init}
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$
% $ \varphicost \leftarrow \varphi \cup\set \neg(\cost < \currlb)
% \wedge (\cost < \currub)$ 
\label{algobin:constraints}
% \STATE $ \varphicost \leftarrow \varphi  \wedge \neg (\cost < \lb ) \wedge (\cost < \ub)$
% \STATE $\currlb\leftarrow \lb; 
% \currub \leftarrow\ub;
% \isminimum \leftarrow false$
%\STATE $\mincost \leftarrow \currub$  
\WHILE{({\bf  not} \isminimum \ {\bf and} $\currlb < \currub $ )} \label{algobin:while}
   \IF{(\dopivoting{})} \label{algobin:pivoting}
     \STATE $\pivot \leftarrow (\currlb + \currub)/2$ 
     \STATE $\pivotatom \leftarrow (\cost < \pivot)$ 
     \STATE $\vi \leftarrow \vi \cup\set{ \pivotatom}$
   \ENDIF \label{algobin:endpivoting}
   \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmt(\varphicost)$ \label{algobin:smtsolver}
   \IF{$(\status = \satres)$}
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algobin:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}
$ 
\label{algobin:add}
   \ELSE[\status = \unsatres]
   \IF{$({\pivotatom \not\in \eta}) $}
      \STATE $\isminimum \leftarrow true$
   \ELSE %[{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}] 
     \STATE $\currlb \leftarrow \pivot$ \label{algobin:lbound}
     \STATE $\varphicost \leftarrow \varphicost \setminus \set{\pivotatom}$\label{algobin:poppivot}   
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algobin:pushnegpivot}    
   \ENDIF
   \ENDIF
\ENDWHILE
\label{algobin:until}
\RETURN $\pair{\calm}{\currub}$ \label{algobin:return}
\end{algorithmic}
\end{algorithm}
%\vspace{-1.5cm}


==> algo_binsearch.tex.2 <==
% input: phi, lb, ub, eps
% phi = phi & !(cost < lb) & (cost < ub)
% l=lb;u=ub;
% do  {
%   p=(u+l)/2;pivot = (cost < p);
%   <res,mu,confl> = MATHSAT(phi,{pivot})
%   if (res==SAT) {
%     u = mincost(mu);
%     phi = phi & (cost < u) & pivot);
%   }
%   else if (confl=={pivot}) {
%     l = p;
%     phi = phi & !pivot;
%   }
%   else { // res==UNSAT, confl=={}
%     SAT=False;
%   }
% } while (SAT)
% return u;
\begin{algorithm}[t]
\caption{\omlarat Procedure based on mixed Linear/Binary Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:binsearch}
}
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE $\langle \varphi, \cost, \lb, \ub \rangle$ $\{$\ub can be $+\infty$$\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
%\isminimum \leftarrow false;
\calm \leftarrow \emptyset
$ \label{algobin:init}
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$
% $ \varphicost \leftarrow \varphi \cup\set \neg(\cost < \currlb)
% \wedge (\cost < \currub)$ 
\label{algobin:constraints}
% \STATE $ \varphicost \leftarrow \varphi  \wedge \neg (\cost < \lb ) \wedge (\cost < \ub)$
% \STATE $\currlb\leftarrow \lb; 
% \currub \leftarrow\ub;
% \isminimum \leftarrow false$
%\STATE $\mincost \leftarrow \currub$  
\WHILE{($\currlb < \currub $ )} \label{algobin:while}
   \IF{(\dopivoting{})} \label{algobin:pivoting}
     \STATE $\pivot \leftarrow \computepivot{}(\currlb,\currub)$ 
%     \STATE $\pivot \leftarrow (\currlb + \currub)/2$ 
     \STATE $\pivotatom \leftarrow (\cost < \pivot)$ 
     \STATE $\vi \leftarrow \vi \cup\set{ \pivotatom}$
   \ENDIF \label{algobin:endpivoting}
   \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmt(\varphicost)$ \label{algobin:smtsolver}
   \IF{$(\status = \satres)$}
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algobin:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}
$ 
\label{algobin:add}
   \ELSE[\status = \unsatres]
   \IF{$({\pivotatom \not\in \eta}) $} 
      \STATE $\currlb \leftarrow \currub$ \label{algobin:end}
   \ELSE %[{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}] 
     \STATE $\currlb \leftarrow \pivot$ \label{algobin:lbound}
     \STATE $\varphicost \leftarrow \varphicost \setminus \set{\pivotatom}$\label{algobin:poppivot}   
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algobin:pushnegpivot}    
   \ENDIF
   \ENDIF
\ENDWHILE
\label{algobin:endwhile}
\RETURN $\pair{\calm}{\currub}$ \label{algobin:return}
\end{algorithmic}
\end{algorithm}
%\vspace{-1.5cm}


==> algo_linsearch.tex <==
\begin{algorithm}[t]
\caption{\omlarat Procedure based on Linear Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:linsearch}
}  
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE $\langle \varphi, \cost, \lb, \ub \rangle$ 
$\{$ \lb can be $-\infty$, \ub can be $+\infty$, $\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
%\isminimum \leftarrow false;
\calm \leftarrow \emptyset
$
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$ \label{algolin:constraints}
\WHILE{($\currlb < \currub $)} \label{algolin:while}
   \STATE $\tuple{\status,\mu} \leftarrow \incrementalsmt(\varphicost)$ \label{algolin:smtsolver}
   \IF{$(\status = \satres)$}
%\STATE \COMMENT{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algolin:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}$ \label{algolin:add}
\ELSE [\status = \unsatres]
%\STATE $\isminimum \leftarrow true$
\STATE $ \currlb  \leftarrow \currub$
   \ENDIF
\ENDWHILE
%\UNTIL{(\isminimum \ {\bf  or} $\currlb \ge \currub $ {\bf  or} $\currub = -\infty$)} 
\label{algolin:endwhile}
\RETURN \pair{\calm}{\currub} \label{algolin:return}
\end{algorithmic}
%\todo{le tre condizioni sono tutte necessarie?}
\end{algorithm}


==> algo_linsearch.tex.1 <==
\begin{algorithm}[t]
\caption{\omlarat Procedure based on Linear Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:linsearch}
}  
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE $\langle \varphi, \cost, \lb, \ub \rangle$ 
$\{$ \lb can be $-\infty$, \ub can be $+\infty$, $\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
\isminimum \leftarrow false;
\calm \leftarrow \emptyset
$
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$ \label{algolin:constraints}
\WHILE{({\bf  not} \isminimum \ {\bf and} $\currlb < \currub $)} \label{algolin:while}
   \STATE $\tuple{\status,\mu} \leftarrow \incrementalsmt(\varphicost)$ \label{algolin:smtsolver}
   \IF{$(\status = \satres)$}
%\STATE \COMMENT{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algolin:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}$ \label{algolin:add}
\ELSE[\status = \unsatres]
\STATE $\isminimum \leftarrow true$
   \ENDIF
\ENDWHILE
%\UNTIL{(\isminimum \ {\bf  or} $\currlb \ge \currub $ {\bf  or} $\currub = -\infty$)} 
\label{algolin:endwhile}
\RETURN \pair{\calm}{\currub} \label{algolin:return}
\end{algorithmic}
%\todo{le tre condizioni sono tutte necessarie?}
\end{algorithm}


==> algo_mixsearch.tex.1 <==
\begin{algorithm}[t]
\caption{\omlarat Procedure based on mixed Linear/Binary Search.
%\todo{FARE 2 VERSIONI DISTINTE?}
\label{algo:mixsearch}
} 
\algsetup{indent=2em}
\renewcommand{\varphicost}{\vi}
\begin{algorithmic}[1]
\REQUIRE
 $\langle \varphi, \cost, \lb, \ub \rangle$ 
%[\ub can be $+\infty$]
$\{$\ub can be $+\infty$, \lb can be $-\infty$ only with linear search$\}$
\STATE $
\currlb \leftarrow\lb;
\currub \leftarrow\ub;
%\isminimum \leftarrow false;
\pivotatom \leftarrow \top;
\calm \leftarrow \emptyset
$ \label{algomix:init}
\STATE $ \varphicost \leftarrow \varphi \cup \set{\currlblit,\currublit}$
\label{algomix:constraints}
\WHILE{($\currlb < \currub $ )} \label{algomix:while}
   \IF[Binary-search Mode]{(\dopivoting{})} \label{algomix:pivotingcond}
\label{algomix:initpivoting}
     \STATE $\pivot \leftarrow \computepivot{}(\currlb,\currub)$ 
%     \STATE $\pivot \leftarrow (\currlb + \currub)/2$ 
     \STATE $\pivotatom \leftarrow (\cost < \pivot)$ 
     \STATE $\vi \leftarrow \vi \cup\set{ \pivotatom}$ \label{algomix:addpivot}
   \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmtcore(\varphicost)$ \label{algomix:smtsolvercore}\label{algomix:endpivoting}
   \ELSE[Linear-search Mode] 
   \STATE $\tuple{\status,\mu} \leftarrow \incrementalsmt(\varphicost)$ \label{algomix:smtsolver}
%     \STATE $\pivotatom \leftarrow \top$ 
\STATE $\eta\leftarrow \emptyset$
   \ENDIF 
   % \STATE $\tuple{\status,\mu,\eta} \leftarrow \incrementalsmtcore(\varphicost)$ \label{algomix:smtsolver}
   \IF{$(\status = \satres)$}\label{algomix:issat} 
     \STATE $\pair{\calm}{\currub} \leftarrow \minimize(\cost, \mu)$ \label{algomix:min}
     \STATE $\varphicost \leftarrow \varphicost \cup \set{\currublit}
$ 
\label{algomix:add}
   \ELSE[\status = \unsatres]
   \IF{$({\pivotatom \not\in \eta}) $} \label{algomix:unsatcondition}
      \STATE $\currlb \leftarrow \currub$ \label{algomix:end}
   \ELSE %[{$(\status = \unsatres\ {\bf and}\ {\pivotatom \not\in \eta}) $}] 
     \STATE $\currlb \leftarrow \pivot$ \label{algomix:lbound}
     \STATE $\varphicost \leftarrow \varphicost \setminus \set{\pivotatom}$\label{algomix:poppivot}   
     \STATE $\varphicost \leftarrow \varphicost \cup\set{\neg\pivotatom}$ \label{algomix:pushnegpivot}    
   \ENDIF
   \ENDIF
\ENDWHILE
\label{algomix:endwhile}
\RETURN $\pair{\calm}{\currub}$ \label{algomix:return}
\end{algorithmic}
\end{algorithm}
%\vspace{-1.5cm}


==> algorithms_bin.tex.1 <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A Binary-Search procedure for \omlarat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The second \omlarat procedure we describe is based on binary search,
and is displayed in Algorithm~\ref{algo:binsearch}.
%
%\marg{I/O of Alg.\ref{algo:binsearch}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{algo_binsearch}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
The input, initialization and loop conditions of the procedure 
(rows \ref{algobin:init}-\ref{algobin:while}) are
identical to that of Algorithm~\ref{algo:linsearch}, except that here
the lower bound \lb must be mandatorily provided  (if not available, it is
necessary to use Algorithm~\ref{algo:linsearch} instead).

(We temporarily assume that the
heuristic predicate \dopivoting (row~\ref{algobin:pivoting})
 always returns true.)  
%   
At the beginning of the loop, the literal $\pivotatom$ is pushed
into the formula stack (rows
\ref{algobin:pivoting}-\ref{algobin:endpivoting}), so that to
temporarily restrict the cost range to \lpivotrange.
% 
Then \incrementalsmt is invoked on \vi, this time activating the 
feature returning also the subset $\eta$ of formulas in (the formula stack of)
$\vi$ which caused the
unsatisfiability of $\vi$  (see \sref{sec:background_sat}).
%

If \vi is \larat-satisfiable, then the procedures behaves as in
Algorithm~\ref{algo:linsearch}. 
%
If instead \vi is \larat-unsatisfiable, we look at $\eta$ and
distinguish two subcases.  
%
If $\pivotatom$ does not occur in $\eta$,
this means that $\vi\setminus\set{\pivotatom}$ is \larat-inconsistent,
i.e. there is no model in the cost range \currrange. Then the
procedure behaves like Algorithm~\ref{algo:linsearch}, forcing the end
of the loop.
%
Otherwise, 
we can only conclude that there is no model in the cost range \lpivotrange,
so that we still need exploring the cost range \rpivotrange.
Thus \currlb is set to \pivot, \pivotatom is popped from \vi and its negation is pushed into
\vi. Then the search proceeds, investigating the cost range \rpivotrange.


%
Similar consideration to those for Algorithm~\ref{algo:linsearch}
apply for Algorithm~\ref{algo:binsearch}. 
%
We also notice a few more facts.
First, the range-partition strategy here may be even
more aggressive than that of standard binary search, because the
minimun cost \currub returned in row~\ref{algobin:min}
 can be significantly smaller than
\pivot, so that the cost range is more than halved. 

Second, unlike with other domains, the binary-search strategy here
is not ``obviously faster'' than the linear-search one, since
unsatisfiable calls to \incrementalsmt are typically much more
expensive than satisfiable ones, because they must explore the whole
Boolean search space rather than only a portion of it (although with a
higher pruning power, due to the stronger constraint induced by the
presence of \pivot).
%%
Thus, we have a tradeoff between a typically much-smaller number of calls plus
a stronger pruning power in  binary search against an average much
smaller cost of the calls in linear search. 
To this extent, it is also possible to try different values of \pivot 
in the form 
$(1-t)\currlb+t\currub$ for some $t\in\ ]0,1[$. 

\medskip
We notice, however, an important drawback of the ``pure
binary-search'' procedure: if \dopivoting always returned $true$, then
the procedure would not necessarily terminate. 
In fact, 
an SMT solver invoked on $\vi$ may 
return a set $\eta$ containing $\pivotatom$ even 
if $\vi\setminus\pivotatom$ is \larat-inconsistent.~%
% 
\footnote{In a nutshell, a CDCL-based SMT solver implicitly builds a
resolution refutation whose leaves are either clauses in $\vi$ 
or \T-lemmas, and the set $\eta$ represents the subset of clauses 
in $\vi$ which occur as leaves of such proof
(see e.g. \cite{cimattigs11_unsatcore} for details).
If  the SMT solver
is invoked on $\vi$ even $\vi\setminus\pivotatom$ is \larat-inconsistent,
 then it can ``use'' \pivotatom and return 
a proof involving it even though 
another \pivotatom-less proof exists. 
} 
Thus, the procedure might got stuck into a ``Zeno''  infinite loop,~%
\footnote{%
In the famous Zeno's paradox, Achilles never reaches the tortoise for a
similar reason.}
 each time halving the cost range right-bound
(e.g., $[-1,0[$, $[-1/2,0[$, $[-1/4,0[$,..).
% In order to guarantee termination, however, it suffices to introduce
To cope with this fact, we introduce 
an heuristic function \dopivoting which returns $false$ after $k$
consecutive \unsatres results, forcing then a ``linear-search'' call
which finally detects the inconsistency.  (In our implementation,
we have empirically experienced the best performances with $k=1$, since
typically satisfiable calls are significantly cheaper then
unsatisfiable ones.)

Under such hypothesis, as with Algorithm~\ref{algo:linsearch}, 
it is straightforward to see that the procedure terminates, it finds the minimum 
value and requires polynomial memory.
 


%\todo{assume che non ci siano clause discharging per semplicita'}

%\todo{fai notare che in caso sat non hai fatto pop di \pivotatom.}


==> algorithms_inline.tex.1 <==
With the inline schema, the whole optimization procedure is pushed inside
the SMT solver, which is thus called only once. 
%
First, \minimize is embedded within the \Tsolver, so that it can
be called incrementally after it, without restarting it from scratch.  
%
Moreover, the range-minimization loop  is embedded inside the
CDCL Boolean-search loop of the standard lazy SMT schema in
\sref{sec:background_smt}.  
%  (In a
% nutshell, as soon as a new minimum-cost model of cost \currub is found, the unit
% clause \currublit is learned, which causes the CDCL SAT solver 
% to backtrack to level 0 and to restart the search from there.)
%
% A much more sophisticated version is implemented by embedding the
% minimization loop  inside the Boolean search performed by the 
% CDCL-based \smt solver. 
% (We call {\em inline} this variant and {\em offline} that of
% Algorithm~\ref{algo:mixsearch}.)
%This work as follows.


\marg{description of \\inline schema}
\todo{girala come ``modifiche a standard SMT''\\}
The procedure is initialized as in 
%steps \ref{algomix:init}-\ref{algomix:constraints} of
Algorithm~\ref{algo:mixsearch},  steps \ref{algomix:init}-\ref{algomix:constraints}.
%}
Then the CDCL loop starts.

Every time the search of the CDCL solver is at decision level zero,
the range \currrange is updated s.t. 
%
\currub [resp. {\currlb] is assigned the lowest [resp. highest] value
  $\currub_i$ [resp. $\currlb_i$] such that the atom $(\cost <
  \currub_i)$ [resp. $\neg (\cost < \currub_i)$] is currently assigned
  at level 0.  (If $\currub \le \currlb$, then the procedure
  terminates, returning the current value of \currub.) 
  % If the range  is changed, then 
  Then \dopivoting is invoked: if it returns \trueval, then
  \computepivot{}($\currlb,\currub$) returns $\pivot\in\
  ]\currlb,\currub[$, and the (possibly new) atom $\pivotatom\defas
  (\cost < \pivot)$ is decided by the SAT solver.  (This correponds to
  steps \ref{algomix:initpivoting}-\ref{algomix:addpivot} in
  Algorithm~\ref{algo:mixsearch}.)  In either case, then the standard
  lazy SMT search proceeds, until one of the following facts happens:
%
\begin{enumerate} 
\item{\label{item:newub}}  
  an assignment $\mu$ propositionally satisfying \vi is generated
  which is found \T-consistent by the \Tsolver. Then $\mu$ is also
  fed to \minimize, returning the minimum cost \minvalue of $\mu$; 
then the clause $(\cost < \minvalue)$ is 
  learned and used for driving the backjumping mechanism, which forces
  the CDCL SAT solver to backjump to level 0, then unit-propagating
  $(\cost < \minvalue)$. This case corresponds to steps 
\ref{algomix:smtsolver}-\ref{algomix:add} in Algorithm~\ref{algo:mixsearch}, 
restricting the cost range to $[\currlb,\minvalue[$.


\item{\label{item:newlb}} in binary-search mode, a conflict occurs
  s.t. the conflict analysis produces a conflict clause in the form
  $\neg\pivotatom\vee\neg\eta'$ s.t. all literals in $\eta'$ are
  assigned at level 0 (thus $\vi\wedge\pivotatom$ is \T-inconsistent).
  Then the SAT solver backtracks to level 0, unit-propagating
  $\neg\pivotatom$.  This case corresponds to steps
  \ref{algomix:smtsolvercore} and
  \ref{algomix:lbound}-\ref{algomix:pushnegpivot} in
  Algorithm~\ref{algo:mixsearch}, restricting the cost range to
  $[\pivot,\currub[$.


\item a conflict occurs producing a conflict clause $\neg\eta$
  s.t. all literals in $\eta$ are assigned at level 0. Then the CDCL
  SAT solver backtracks to level 0, causing the end of the whole
  procedure.  This case corresponds to step \ref{algomix:end} in
  Algorithm~\ref{algo:mixsearch}.


\end{enumerate}
%
\noindent
Cases \ref{item:newub} and \ref{item:newlb} cause the procedure to
backjump to decision level 0 and hence to restrict the cost range,
similarly to what happens in Algorithm~\ref{algo:mixsearch}.

\marg{not only binary search}
Notice, however, that also other situations may allow for restricting the
cost range: e.g., if 
$\vi\wedge \neg (\cost < \currlb)\wedge(\cost < \currub)\models 
(\cost \bowtie m)$ for some atom $(\cost \bowtie \mvalue)$ occurring in \vi s.t. 
$\mvalue \in \currrange$ and $\bowtie\ \in
\{\le,<,\ge,>\}$, then the SMT solver may backjump to decision level 0 
and propagate $(\cost \bowtie \mvalue)$, which further restricts the cost
range. 



%
\marg{early-pruning as branch \& bound}
Notice that, during the seatch, every partial assignment $\mu$ under
construction contains the
atom $(\cost < \currub)$.  Thus, if a partial assignment $\mu$ is
generated which cannot be expanded into a total one whose cost is
better than $\currub$, then $\mu$ is found \T-inconsistent directly by
early-pruning calls to \Tsolver.  To this extent, in this schema
early-pruning plays the role of ``bounding'' in a branch and bound fashion.




The efficiency of the procedure can be further improved as follows. 


% First, an early-pruning call to \Tsolver is performed also at level 0,
% before the search starts and/or \pivotatom is decided, so that 
\ignore{%
First, an early-pruning call to \Tsolver is performed
  also at level 0, before the first decision is performed, so that to
  cut the search if the current set of unit clauses is
  \T-inconsistent.%
}

\marg{learning \pivotatom}
First, when in step \ref{item:newub} a novel minimum \minvalue is
found, not only $(\cost < \minvalue)$ but also $\pivotatom$ is learned
as unit clause.  Although redundant from the logical perspective since
$\minvalue<\pivot$, the unit clause $\pivotatom$ allows the SAT solver
to reuse the clauses in the form $\neg \pivotatom \vee C'$ which have
been learned when investigating the cost range \lpivotrange.
(In Algorithm~\ref{algo:mixsearch} this is done implicitly, since \pivotatom 
is not popped from \vi before step \ref{algomix:add}.)
%  

\marg{tightening}
Second, in binary-search mode, when in step
\ref{item:newlb} the \Tsolver returns a conflict set in the form
$\eta\cup\{\pivotatom\}$, 
then it is further asked to find the maximum value $\maxvalue$
s.t. $\eta\cup\{(\cost<\maxvalue)\}$ is also \T-inconsistent. (This is done
with a simple modification of the algorithm in \cite{demoura_cav06}.)

If $\maxvalue>\currub$, then the clause
$C^*\defas\neg\eta\vee\neg(\cost<\currub)$ is used for backjumping
and learning instead of $C\defas\neg\eta\vee\neg\pivotatom$.
Eventually, instead of using $C$ for backjumping to level 0 and
propagating $\neg\pivotatom$, the SMT solver may use 
$C^*$ for backjumping to level 0, forcing the procedure to stop.

If $\currub>\maxvalue>\pivot$, then the two clauses 
$C_1\defas\neg\eta\vee\neg(\cost<\maxvalue)$ and 
$C_2\defas\neg\pivotatom\vee(\cost<\maxvalue)$ are 
used for backjumping and learning instead of 
$C\defas\neg\eta\vee\neg\pivotatom$.
In particular, $C_2$ forces backjumping to level 1 
ad propagating the (possibly fresh) atom $(\cost<\maxvalue)$; 
eventually, due to 1UIP, instead of using $C$ for backjumping to level 0 and
propagating $\neg\pivotatom$, the SMT solver may use 
$C_1$ for backjumping to level  0 and
propagating $\neg(\cost<\maxvalue)$, restricting the range to 
$[\maxvalue,\currub[$ rather than to \rpivotrange. 

\ignoreinshort{%
\begin{example}
\marg{esempio tightening}
\label{ex:tightening}
Consider the formula $\vi\defas\psi\wedge(\cost \ge a+15)\wedge(a\ge
0)$ for some $\psi$ in the cost range $[0,16[$. With basic
binary-search, deciding $\pivotatom\defas(\cost<8)$, the \Tsolver
produces the \Tlemma
%
$C\defas 
\neg(\cost \ge a+15)\vee
\neg(a\ge 0)\vee
\neg\pivotatom
$
%
causing backjumping to level 0 and unit-propagating $\neg\pivotatom$
on $C$, restricting the range to $[8,16[$; it takes a sequence of
similar steps to progressivelty restrict the range to $[8,16[$,
$[12,16[$, $[14,16[$, and $[15,16[$.
%
If instead the \Tsolver produces the \Tlemmas
%
$C_1=
\neg(\cost \ge a+15)\vee
\neg(a\ge 0)\vee
\neg(\cost<15)
$
and
$
C_2=\neg\pivotatom \vee (\cost<15)
$,
this first causes backjumping to level 1 
the unit-propagation of $(\cost<15)$ 
after \pivotatom, and then a backjumping on $C_1$ to level zero, 
unit-propagating $\neg(\cost<15)$, which directly restricts the range
to  $[15,16[$.
% 
\end{example}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\todo{---------------------- sono arrivato qui -----------------}


%DONE\todo{descrivere pivoting\\}
%DONE\todo{early-pruning at level 0, spiegare quando termina\\}
%\todo{also $\neg\eta$ can be learned\\}
%DONE\todo{importanza delll'imparare $(\cost < \pivot)$\\}
\todo{issue of 1stUIP vs. LastUIP\\}
%DONE\todo{descrivere tightening\\}
\todo{esempi\\}



==> algorithms_lin.tex.1 <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A Linear-Search procedure for \omlarat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
The first \omlarat procedure we describe is based on linear search,
and is displayed in Algorithm~\ref{algo:linsearch}.
%
%\marg{I/O of Alg.\ref{algo:linsearch}}
It takes as input an instance
of the \omtlcf problem, plus optionally values for \lb and \ub 
(which are implicitly considered to be $-\infty$ and $+\infty$ if not
present), and returns the model \calm of minimum cost and its 
cost (the value \ub if \vi
is \larat-inconsistent).~%
\footnote{%
Notice that by providing a lower bound \lb [resp. an upper bound \ub] 
the user implicitly assumes the responsibility of asserting there is no model 
whose cost is lowers than \lb [there is a model whose cost is \ub].
}
%%%%%%%%%% ALGO QUI
\input{algo_linsearch}
%%%%%%%%%%%%%%%%%%%%%

%\marg{descr. of Alg.\ref{algo:linsearch}}
First, the variables \currlb, \currub (defining the current range) and the flag 
\isminimum are initialized to \lb, \ub and $false$ respectively,
and \calm is initialized to be an empty model.
%
Then the procedure adds to \vi the bound constraints, if
present, which restrict the search within
the range $[\lb,\ub[$ (row \ref{algolin:constraints}).~%
\footnote{Of course literals like \lbliti{-\infty} 
%$\neg (\cost <  -\infty)$ 
and \ubliti{+\infty} 
%  $(\cost < +\infty)$ 
are not added.}
% Notice that if either $lb$ or $ub$ are infinite,
% no bound constraint is learned. 
%
The solution space is then explored iteratively (rows
\ref{algolin:while}-\ref{algolin:endwhile}).
First,  an incremental
\smtlarat solver is invoked on \vi (row \ref{algolin:smtsolver}). 
 (Notice that, given the incrementality of the SMT solver,
 every operation in the form 
``$\vi \leftarrow \vi \cup \set{\phi_i}$" 
[resp. $\vi \leftarrow \vi \setminus\set{\phi_i}$] 
is implemented as a ``push'' [resp. ``pop'']
operation  on the stack representation 
$\vi$, see \sref{sec:background_sat};
it is also very important to recall that 
during the SMT call $\vi$ is updated with 
the clauses which are learned during the 
SMT search.)

If \vi is
\larat-satisfiable, then it is returned \status=\satres and a
\larat-satisfiable truth assignments $\mu$ for $\vi$.
%
Thus \minimize is invoked on $\mu$,~\footnote{%
possibly after applying pure-literal filtering to $\mu$
(see \sref{sec:background_smt}).} returning 
the model \calm for $\mu$ of minimum cost
$\currub$ ($-\infty$ iff the problem in unbounded).
% (row \ref{algolin:min}).  
%(Notice that \currub is $-\infty$ iff the problem in unbounded.)
%
The current solution 
$\currub$ becomes the new upper bound, 
thus the \larat-atom $(\cost < \currub)$
is added to $\vi$ (row \ref{algolin:add}). 
%
If \vi is
\larat-unsatisfiable, then no model in the current cost range
\currrange can be found;
hence the flag \isminimum is set to $true$, forcing the end of the loop. 

The loop terminates when either $\vi$ 
is found unsatisfiable or the problem is found to be unbounded 
(i.e. the optimal solution found is  $-\infty$). 
% In the former case 
% the last solution found is the optimal one (row \ref{algolin:return}).
Then the whole process
terminates, returning the current model \calm and its cost \currub.
%
Notice that the procedure works also if $\lb=-\infty$, or
$\ub=+\infty$, or both. 

%
%\marg{\minimize\\ strict constr.}
%\todo{issue of strict constraints and minimums\\}
%
In a nutshell, \minimize is a simple extension of the 
\TsolverGen{\larat} \cite{demoura_cav06} 
which is invoked after one solution is found, 
  minimizing it by standard Simplex techniques.
%~\footnote{%
%  \begin{remark}
If the input problem contains strict inequalities,
 then \minimize temporarily treats them as non-strict ones and finds
 the minimum-cost 
 solution with standard Simplex techniques. 
%
 If such minimum-cost solution \ar{x}{} of cost $\minvalue$ lays only on
 non-strict inequalities, then \ar{x}{} is a solution; otherwise, 
 for some $\delta>0$ and for every cost $c\in\
 ]\minvalue,\minvalue+\delta]$ there exist a solution of cost $c$.
 (If  needed, such solution is computed using the
 techniques for handling strict inequalities described in
 \cite{demoura_cav06}.)  Thus the value \minvalue is returned, tagged
 as a non-strict minimum, so that the constraint $(\cost\le\minvalue)$ 
 rather than  $(\cost<\minvalue)$ is added to \vi. 
%  \end{remark}
%}

Notice, however, that this latter fact never happens  
if the SMT solver (like \mathsat) implements 
pure-literal filtering (\sref{sec:background_smt}) 
and if no strict inequalities occur non-negated in $\vi$   (which is the
case of most problems in this paper). 
%
In fact, due to pure-literal filtering, the only strict inequalities
which may be fed to \minimize are upper-bound constraints
\currubliti{i}, which by construction do not touch the minimum-cost
solution \ar{x}{} above.
 




\medskip
We remark a few facts about 
%It is important to fully understand 
the behaviour of \incrementalsmt within this algorithm.
% how the steps in
% Algorithm~\ref{algo:linsearch} interact with these of \incrementalsmt. 
%
First, we notice that in Algorithm~\ref{algo:linsearch} all the
literals stating the cost range (i.e., $\neg (\cost < \currlb)$, $(\cost <
\currub)$) are always added to \vi as unit clauses;
thus inside \incrementalsmt these literals are immediately
unit-propagated, becoming part of each truth 
assignment $\mu$ from the very beginning of its construction.
% 
Thus, while building an assignment $\mu$, as soon as novel \T-literals
are added to $\mu$ which prevent it from 
having a \larat-model of cost in  \currrange, 
the \larat-solver invoked on $\mu$ by early-pruning  calls (see
\sref{sec:background_smt}) returns
\unsatres and the \T-lemma $\neg\eta$ describing the conflict,
triggering \T-backjumping and \T-learning. 
%
%  Thus, if a partial assignment $\mu$ is
% generated which cannot be expanded into a total one whose cost is
% better than $\mincost$, then $\mu$ is found \T-inconsistent directly by
% early-pruning calls to \T-solver.  
%
To this extent, \incrementalsmt implicitly plays a
form of branch\&bound: decide a new literal $l$ and
unit-/\T-propagate the literals which derive from $l$ (``branch'') and
backtrack as soon as the current branch can no more be expanded into 
%(up to exponentially-many)
models in the current cost range (``bound'').
To this extent, we remark that also the lower-bound constraint \currlblit 
plays a role in Algorithm~\ref{algo:linsearch}, since it helps pruning the
search inside \incrementalsmt.

Second, the incrementality of the SMT solver 
%\marg{role of \\incrementality}
(see \sref{sec:background_sat} and \sref{sec:background_smt}) 
plays an essential role here, since at every call \incrementalsmt
resumes the status of the search of the end of the previous call, only with 
tighter cost range constraints. (Notice that at each
call here the solver can reuse all previously-learned clauses.)
To this extent, one can see the whole process as only one SMT process, 
which is interrupted and resumed each time a new model is found,
in which cost range constraints are progressively tightened.

%\marg{spostare sopra?}
Third, although each previously-added upper-bound constraint
\currubliti{i-1} is entailed by the new one \currubliti{i} and it is
thus redundant, we deliberately do not pop the former before pushing
the latter, since it ``activates'' by unit-propagation all
previously-learned clauses in the form $\negcurrubliti{i-1} \vee ...$,
which otherwise could not be of help for the embedded SAT solver.

%\marg{inline}
Fourth, we notice that Algorithm~\ref{algo:linsearch} uses the 
SMT solver
%\incrementalsmt 
as a black-box. This is important, since the
source code of most SMT solvers is not publicly available.
%
A more sophisticate version can be implemented, however, if one can
access the source code of the SMT solver (like we do with \mathsat). 
First, \minimize can be embedded within the \Tsolver, so that it can
be called incrementally after \Tsolver, without restarting from scratch.  
%
Moreover, the range-minimization loop (rows
\ref{algolin:while}-\ref{algolin:endwhile}) can be embedded inside the
CDCL Boolean-search loop of the standard SMT paradigm.  (In a
nutshell, as soon as a new minimum-cost model of cost \currub is found, the unit
clause \currublit is learned, which causes the CDCL SAT solver 
to backtrack to level 0 and to restart the search from there.)
%
We call {\em inline} this variant and {\em offline} that of
Algorithm~\ref{algo:linsearch}.

\ignore{%%%%% INLINE VERSION
A more sophisticate version can be implemented by embedding the
minimization loop of lines \ref{algolin:repeat}-\ref{algolin:until} 
inside the CDCL schema, according
to the lazy SMT approach briefly described in section~\ref{sec:backsmt}.
%
The algorithm behaves like that described in section ~\ref{sec:backsmt}.
When a satisfying assignment $\mu$ is found \T-consistent by the \T-solver,
$\mu$ is also fed to $minimize()$; the latter returns the minimum
cost of $\mu$, which becomes the new value of $\mincost$, and the
subset $\eta$ of \la-atoms in $\mu$ involved in the minimum. 
Then the clauses $(\cost < \mincost)$ and $\neg \eta$ 
are learned and used for driving the \T-backjumping mechanism.
%
%Also the atom (cost < pivot) is learned in order to activate the clauses in the form $\neg (cost <
%pivot) \vee ...$
%which have been learned during previous steps in the search.
}


%\todo{importance of incrementality}. 
%\marg{incrementality}
% \todo{parla di further improvements: inlining di minimizer, 
% inlining del loop inside SAT loop.}
%\newpage

\smallskip
%\marg{termination,\\ correctness,\\ polynomial space}
It is straightforward to notice the following facts:
%
 (i) the procedure terminates, 
because there are only a finite number
of candidate truth assignments $\mu$ to be enumerated, and steps
\ref{algolin:min}-\ref{algolin:add} guarantee that the same assignment
$\mu$ will never be returned twice by \incrementalsmt;
%
(ii) it returns a model of minimum cost, because it explores the whole
search space of candidate truth assignments, and for every suitable
assignment $\mu$
\minimize finds the minimum-cost model for $\mu$;
%
 (iii) it
requires polynomial space, under the assumption that the underlying
CDCL SAT solver adopts a polynomial-size clause
 discharging strategy (which is the
case of all SMT solvers, including \mathsat). 



==> algorithms_offline.tex.1 <==
\todo{merge lin e bin into one}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A Linear-Search procedure for \omlarat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fakesubsubsection{Linear Search.} 
%\input{algorithms_lin.tex}
\label{sec:algorithms_lin}
% 
The first \omlarat procedure we describe is based on linear search,
and is displayed in Algorithm~\ref{algo:linsearch}.
%
%\marg{I/O of Alg.\ref{algo:linsearch}}
It takes as input an instance
of the \omtlcf problem, plus optionally values for \lb and \ub 
(which are implicitly considered to be $-\infty$ and $+\infty$ if not
present), and returns the model \calm of minimum cost and its 
cost (the value \ub if \vi
is \larat-inconsistent).~%
\footnote{%
Notice that by providing a lower bound \lb [resp. an upper bound \ub] 
the user implicitly assumes the responsibility of asserting there is no model 
whose cost is lowers than \lb [there is a model whose cost is \ub].
}
%%%%%%%%%% ALGO QUI
\input{algo_linsearch}
%%%%%%%%%%%%%%%%%%%%%

%\marg{descr. of Alg.\ref{algo:linsearch}}
First, the variables \currlb, \currub (defining the current range) 
 are initialized to \lb and \ub respectively,
and \calm is initialized to be an empty model.
%
Then the procedure adds to \vi the bound constraints, if
present, which restrict the search within
the range $[\lb,\ub[$ (row \ref{algolin:constraints}).~%
\footnote{Of course literals like \lbliti{-\infty} 
%$\neg (\cost <  -\infty)$ 
and \ubliti{+\infty} 
%  $(\cost < +\infty)$ 
are not added.}
% Notice that if either $lb$ or $ub$ are infinite,
% no bound constraint is learned. 
%
The solution space is then explored iteratively (rows
\ref{algolin:while}-\ref{algolin:endwhile}).
First,  an incremental
\smtlarat solver is invoked on \vi (row \ref{algolin:smtsolver}). 
 (Notice that, given the incrementality of the SMT solver,
 every operation in the form 
``$\vi \leftarrow \vi \cup \set{\phi_i}$" 
[resp. $\vi \leftarrow \vi \setminus\set{\phi_i}$] 
is implemented as a ``push'' [resp. ``pop'']
operation  on the stack representation 
$\vi$, see \sref{sec:background_sat};
it is also very important to recall that 
during the SMT call $\vi$ is updated with 
the clauses which are learned during the 
SMT search.)

If \vi is
\larat-satisfiable, then it is returned \status=\satres and a
\larat-satisfiable truth assignments $\mu$ for $\vi$.
%
Thus \minimize is invoked on $\mu$,~\footnote{%
possibly after applying pure-literal filtering to $\mu$
(see \sref{sec:background_smt}).} returning 
the model \calm for $\mu$ of minimum cost
$\currub$ ($-\infty$ iff the problem in unbounded).
% (row \ref{algolin:min}).  
%(Notice that \currub is $-\infty$ iff the problem in unbounded.)
%
The current solution 
$\currub$ becomes the new upper bound, 
thus the \larat-atom $(\cost < \currub)$
is added to $\vi$ (row \ref{algolin:add}). 
%
If \vi is
\larat-unsatisfiable, then no model in the current cost range
\currrange can be found;
hence the flag \currlb is set to \currub, forcing the end of the loop. 

The loop terminates when either $\vi$ 
is found unsatisfiable or the problem is found to be unbounded 
(i.e. the optimal solution found is  $-\infty$). 
% In the former case 
% the last solution found is the optimal one (row \ref{algolin:return}).
Then the whole process
terminates, returning the current model \calm and its cost \currub.
%
Notice that the procedure works also if $\lb=-\infty$, or
$\ub=+\infty$, or both. 

%
%\marg{\minimize\\ strict constr.}
%\todo{issue of strict constraints and minimums\\}
%
In a nutshell, \minimize is a simple extension of the 
\TsolverGen{\larat} \cite{demoura_cav06} 
which is invoked after one solution is found, 
  minimizing it by standard Simplex techniques.
%~\footnote{%
%  \begin{remark}
If the input problem contains strict inequalities,
 then \minimize temporarily treats them as non-strict ones and finds
 the minimum-cost 
 solution with standard Simplex techniques. 
%
 If such minimum-cost solution \ar{x}{} of cost $\minvalue$ lays only on
 non-strict inequalities, then \ar{x}{} is a solution; otherwise, 
 for some $\delta>0$ and for every cost $c\in\
 ]\minvalue,\minvalue+\delta]$ there exist a solution of cost $c$.
 (If  needed, such solution is computed using the
 techniques for handling strict inequalities described in
 \cite{demoura_cav06}.)  Thus the value \minvalue is returned, tagged
 as a non-strict minimum, so that the constraint $(\cost\le\minvalue)$ 
 rather than  $(\cost<\minvalue)$ is added to \vi. 
%  \end{remark}
%}

\todo{drop in short?} Notice, however, that this latter fact never happens  
if the SMT solver (like \mathsat) implements 
pure-literal filtering (\sref{sec:background_smt}) 
and if no strict inequalities occur non-negated in $\vi$   (which is the
case of most problems in this paper). 
%
In fact, due to pure-literal filtering, the only strict inequalities
which may be fed to \minimize are upper-bound constraints
\currubliti{i}, which by construction do not touch the minimum-cost
solution \ar{x}{} above.
 




\medskip
We remark a few facts about 
%It is important to fully understand 
the behaviour of \incrementalsmt within this algorithm.
% how the steps in
% Algorithm~\ref{algo:linsearch} interact with these of \incrementalsmt. 
%
First, we notice that in Algorithm~\ref{algo:linsearch} all the
literals stating the cost range (i.e., $\neg (\cost < \currlb)$, $(\cost <
\currub)$) are always added to \vi as unit clauses;
thus inside \incrementalsmt these literals are immediately
unit-propagated, becoming part of each truth 
assignment $\mu$ from the very beginning of its construction.
% 
Thus, while building an assignment $\mu$, as soon as novel \T-literals
are added to $\mu$ which prevent it from 
having a \larat-model of cost in  \currrange, 
the \larat-solver invoked on $\mu$ by early-pruning  calls (see
\sref{sec:background_smt}) returns
\unsatres and the \T-lemma $\neg\eta$ describing the conflict,
triggering \T-backjumping and \T-learning. 
%
%  Thus, if a partial assignment $\mu$ is
% generated which cannot be expanded into a total one whose cost is
% better than $\mincost$, then $\mu$ is found \T-inconsistent directly by
% early-pruning calls to \T-solver.  
%
To this extent, \incrementalsmt implicitly plays a
form of branch\&bound: decide a new literal $l$ and
unit-/\T-propagate the literals which derive from $l$ (``branch'') and
backtrack as soon as the current branch can no more be expanded into 
%(up to exponentially-many)
models in the current cost range (``bound'').
To this extent, we remark that also the lower-bound constraint \currlblit 
plays a role in Algorithm~\ref{algo:linsearch}, since it helps pruning the
search inside \incrementalsmt.

Second, the incrementality of the SMT solver 
%\marg{role of \\incrementality}
(see \sref{sec:background_sat} and \sref{sec:background_smt}) 
plays an essential role here, since at every call \incrementalsmt
resumes the status of the search of the end of the previous call, only with 
tighter cost range constraints. (Notice that at each
call here the solver can reuse all previously-learned clauses.)
To this extent, one can see the whole process as only one SMT process, 
which is interrupted and resumed each time a new model is found,
in which cost range constraints are progressively tightened.

%\marg{spostare sopra?}
Third, although each previously-added upper-bound constraint
\currubliti{i-1} is entailed by the new one \currubliti{i} and it is
thus redundant, we deliberately do not pop the former before pushing
the latter, since it ``activates'' by unit-propagation all
previously-learned clauses in the form $\negcurrubliti{i-1} \vee ...$,
which otherwise could not be of help for the embedded SAT solver.

\ignore{%%%%%%%%%%%% SPOSTATA A SEZ. INLINE
%\marg{inline}
Fourth, we notice that Algorithm~\ref{algo:linsearch} uses the 
SMT solver
%\incrementalsmt 
as a black-box. This is important, since the
source code of most SMT solvers is not publicly available.
%
A much more sophisticate version can be implemented, however, if one can
access the source code of the SMT solver (like we do with \mathsat). 
First, \minimize can be embedded within the \Tsolver, so that it can
be called incrementally after \Tsolver, without restarting from scratch.  
%
Moreover, the range-minimization loop (rows
\ref{algolin:while}-\ref{algolin:endwhile}) can be embedded inside the
CDCL Boolean-search loop of the standard SMT paradigm.  (In a
nutshell, as soon as a new minimum-cost model of cost \currub is found, the unit
clause \currublit is learned, which causes the CDCL SAT solver 
to backtrack to level 0 and to restart the search from there.)
%
We call {\em inline} this variant and {\em offline} that of
Algorithm~\ref{algo:linsearch}.
} %%%%%%%%%%%%%%%

%\todo{importance of incrementality}. 
%\marg{incrementality}
% \todo{parla di further improvements: inlining di minimizer, 
% inlining del loop inside SAT loop.}
%\newpage

\smallskip
%\marg{termination,\\ correctness,\\ polynomial space}
It is straightforward to notice the following facts:
%
 (i) the procedure terminates, 
because there are only a finite number
of candidate truth assignments $\mu$ to be enumerated, and steps
\ref{algolin:min}-\ref{algolin:add} guarantee that the same assignment
$\mu$ will never be returned twice by \incrementalsmt;
%
(ii) it returns a model of minimum cost, because it explores the whole
search space of candidate truth assignments, and for every suitable
assignment $\mu$
\minimize finds the minimum-cost model for $\mu$;
%
 (iii) it
requires polynomial space, under the assumption that the underlying
CDCL SAT solver adopts a polynomial-size clause
 discharging strategy (which is the
case of all SMT solvers, including \mathsat). 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A Binary-Search procedure for \omlarat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fakesubsubsection{Mixed Linear/Binary Search.}
%\input{algorithms_bin.tex}
\label{sec:algorithms_bin}
%
The second \omlarat procedure we describe is based on binary search,
and is displayed in Algorithm~\ref{algo:binsearch}.
%
%\marg{I/O of Alg.\ref{algo:binsearch}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{algo_binsearch}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
The input, initialization and loop conditions of the procedure 
(rows \ref{algobin:init}-\ref{algobin:while}) are
identical to that of Algorithm~\ref{algo:linsearch}, except that here
the lower bound \lb must be mandatorily provided  (if not available, it is
necessary to use Algorithm~\ref{algo:linsearch} instead).
 
(We temporarily assume that the
heuristic predicate \dopivoting (row~\ref{algobin:pivoting})
 always returns \trueval.)  
%   
At the beginning of the loop, 
the value $\pivot\in\ ]\currlb,\currub[$ is computed by the heuristic
function \computepivot{}
(in the simplest form, $\pivot$ is $(\currlb + \currub)/2$), 
the literal $\pivotatom$ is pushed
into the formula stack (rows
\ref{algobin:pivoting}-\ref{algobin:endpivoting}), so that to
temporarily restrict the cost range to \lpivotrange.
% 
Then \incrementalsmt is invoked on \vi, this time activating the 
feature returning also the subset $\eta$ of formulas in (the formula stack of)
$\vi$ which caused the
unsatisfiability of $\vi$  (see \sref{sec:background_sat}).
%

If \vi is \larat-satisfiable, then the procedures behaves as in
Algorithm~\ref{algo:linsearch}. 
%
If instead \vi is \larat-unsatisfiable, we look at $\eta$ and
distinguish two subcases.  
%
If $\pivotatom$ does not occur in $\eta$,
this means that $\vi\setminus\set{\pivotatom}$ is \larat-inconsistent,
i.e. there is no model in the cost range \currrange. Then the
procedure behaves like Algorithm~\ref{algo:linsearch}, forcing the end
of the loop.
%
Otherwise, 
we can only conclude that there is no model in the cost range \lpivotrange,
so that we still need exploring the cost range \rpivotrange.
Thus \currlb is set to \pivot, \pivotatom is popped from \vi and its negation is pushed into
\vi. Then the search proceeds, investigating the cost range \rpivotrange.


%
Similar consideration to those for Algorithm~\ref{algo:linsearch}
apply for Algorithm~\ref{algo:binsearch}. 
%
We also notice a few more facts.
First, the range-partition strategy here may be even
more aggressive than that of standard binary search, because the
minimun cost \currub returned in row~\ref{algobin:min}
 can be significantly smaller than
\pivot, so that the cost range is more than halved. 

Second, unlike with other domains, the binary-search strategy here
is not ``obviously faster'' than the linear-search one, since
unsatisfiable calls to \incrementalsmt are typically much more
expensive than satisfiable ones, because they must explore the whole
Boolean search space rather than only a portion of it (although with a
higher pruning power, due to the stronger constraint induced by the
presence of \pivot).
%%
Thus, we have a tradeoff between a typically much-smaller number of calls plus
a stronger pruning power in  binary search against an average much
smaller cost of the calls in linear search. 
To this extent, it is also possible to try different values of \pivot 
in the form 
$(1-t)\currlb+t\currub$ for some $t\in\ ]0,1[$. 

\medskip
We notice, however, an important drawback of the ``pure
binary-search'' procedure: if \dopivoting always returned \trueval{}, then
the procedure would not necessarily terminate. 
In fact, 
an SMT solver invoked on $\vi$ may 
return a set $\eta$ containing $\pivotatom$ even 
if $\vi\setminus\pivotatom$ is \larat-inconsistent.~%
% 
\footnote{In a nutshell, a CDCL-based SMT solver implicitly builds a
resolution refutation whose leaves are either clauses in $\vi$ 
or \T-lemmas, and the set $\eta$ represents the subset of clauses 
in $\vi$ which occur as leaves of such proof
(see e.g. \cite{cimattigs11_unsatcore} for details).
If  the SMT solver
is invoked on $\vi$ even $\vi\setminus\pivotatom$ is \larat-inconsistent,
 then it can ``use'' \pivotatom and return 
a proof involving it even though 
another \pivotatom-less proof exists. 
} 
Thus, the procedure might got stuck into a ``Zeno''  infinite loop,~%
\footnote{%
In the famous Zeno's paradox, Achilles never reaches the tortoise for a
similar reason.}
 each time halving the cost range right-bound
(e.g., $[-1,0[$, $[-1/2,0[$, $[-1/4,0[$,..).
% In order to guarantee termination, however, it suffices to introduce
To cope with this fact, we introduce 
an heuristic function \dopivoting which returns \falseval after $k$
consecutive \unsatres results, forcing then a ``linear-search'' call
which finally detects the inconsistency.  (In our implementation,
we have empirically experienced the best performances with $k=1$, since
typically satisfiable calls are significantly cheaper then
unsatisfiable ones.)

Under such hypothesis, as with Algorithm~\ref{algo:linsearch}, 
it is straightforward to see that the procedure terminates, it finds the minimum 
value and requires polynomial memory.
 


%\todo{assume che non ci siano clause discharging per semplicita'}

%\todo{fai notare che in caso sat non hai fatto pop di \pivotatom.}


==> background_sat_long.tex <==



\todo{SFRONDARE?\\}
\ignore{% SHORT
We assume the standard syntactic and semantic notions of propositional
logic (including the standard notions of formula, atom, literal, CNF formula,
truth assignment, clause, unit clause).
}%%%% 
%%%%%%%%% BEGIN LONG
We assume the standard syntactic and semantic notions of propositional logic.
Given a non-empty set of primitive propositions  
$\calp = \{\pr{1},\pr{2},\ldots\}$, the
language of propositional logic is the least set of formulas containing 
\calp and the primitive constants $\top$ and $\bot$ (``true'' and ``false'') and closed under the set of standard
propositional connectives $\{\neg,\wedge,\vee,\imp,\iff\}$.
% 
We call a {\em propositional atom} every primitive proposition in \calp,
and  a {\em propositional literal} every propositional atom ({\em
  positive literal}) or its negation ({\em
  negative literal}). 
We implicitly remove double negations: e.g., 
if $l$ is the negative literal $\neg \pr{i}$, by $\neg l$ we mean $\pr{i}$ 
rather than $\neg\neg \pr{i}$. 
%%%%%%%%% END LONG
We represent a truth assignment $\mu$ 
as a conjunction of literals $\bigwedge_i l_i$ (or indifferently as a set of
literals $\{l_i\}_i$) with the intended meaning
that a positive [resp. negative] literal $\pr{i}$ means that $\pr{i}$ is
assigned to true [resp. false].
%%%%%%%%% BEGIN LONG
A propositional formula is in {\em conjunctive
  normal form, CNF,} if it is written as a conjunction of disjunctions
of literals: $\bigwedge_i \bigvee_j l_{ij}$. 
Each disjunction of
literals $\bigvee_j l_{ij}$ is called a {\em clause}.
%
A {\em unit clause} is a clause with only one literal.
%
%%%%%%%%% END LONG

\begin{figure}[t]
  \centering
  \begin{minipage}{.45\textwidth}
    {\tt 
      \begin{tabbing}[c]
        foo \= foo \= foo \= foo \= foo \= \kill
        1.\> SatValue CDCL (formula $\varphi$, assignment $\mu$) \{ \\
        2.\> \>  {\bf while} (1) \{ \\
        3.\> \> \> {\bf while} (1) \{ \\
        4.\> \> \> \> status = bcp($\varphi$, $\mu$); \\
        5.\> \> \> \> {\bf if} (status == \satres) \\
        6.\> \> \> \> \> {\bf return} \satres; \\
        7.\> \> \> \> {\bf else if} (status == \conflres) \{ \\
        8.\> \> \> \> \> blevel = analyze\_conflict($\varphi$, $\mu$); \\
        9.\> \> \> \> \> {\bf if} (blevel == 0) {\bf return} \unsatres; \\
        10.\> \> \> \> \> {\bf else} backtrack(blevel,$\varphi$, $\mu$); \\
        11.\> \> \> \> \} \\
        12.\> \> \> \> {\bf else} break; \\
        13.\> \> \> \} \\
        14.\> \> \> decide\_next\_branch($\varphi$, $\mu$); \\
        15.\> \}\} \\      
      \end{tabbing}
%%       \begin{tabbing}[c]
%%         foo \= foo \= foo \= foo \= foo \= \kill
%%         1.\> SatValue DPLL (formula $\varphi$, assignment $\mu$) \{ \\
%%         2.\> \>  {\bf while} (1) \{ \\
%%         3.\> \> \> decide\_next\_branch($\varphi$, $\mu$); \\
%%         4.\> \> \> {\bf while} (1) \{ \\
%%         5.\> \> \> \> status = deduce($\varphi$, $\mu$); \\
%%         6.\> \> \> \> {\bf if} (status == \satres) \\
%%         7.\> \> \> \> \> {\bf return} \satres; \\
%%         8.\> \> \> \> {\bf else if} (status == \conflres) \{ \\
%%         9.\> \> \> \> \> blevel = analyze\_conflict($\varphi$, $\mu$); \\
%%         10.\> \> \> \> \> {\bf if} (blevel == 0) {\bf return} \unsatres; \\
%%         11.\> \> \> \> \> {\bf else} backtrack(blevel,$\varphi$, $\mu$); \\
%%         12.\> \> \> \> \} \\
%%         13.\> \> \> \> {\bf else} break; \\
%%         14.\> \}\}\} \\      
%%       \end{tabbing}
    } % tt
  \end{minipage}
%\vspace{-.5cm}
  \caption{Schema of a conflict-driven \dpll SAT solver.\label{fig:dpll}}
%\vspace{-.5cm}
%  
\end{figure}
%


The schema of a modern conflict-driven \dpll{} SAT solver 
%adapted from the one presented in \cite{moskewicz01chaff,zhang01learning}, %
%
is reported in Figure~\ref{fig:dpll}  \cite{sil96a,zhang01learning}. 
The propositional formula $\varphi$ is in CNF;  
the assignment $\mu$ is initially empty, and it is updated in a stack-based 
manner.

In the main loop, $\mathtt{decide\_next\_branch}(\varphi, \mu)$ (row
{\tt 14.})
chooses an unassigned 
literal $l$ from $\varphi$ according to some heuristic criterion, and adds it
to $\mu$. (This operation is called \emph{decision}, $l$ is called \emph{decision literal}
end the number of decision literals in $\mu$ after this operation is called
the \emph{decision level} of $l$.)  In the inner loop,
$\mathtt{bcp}(\varphi, \mu)$ 
iteratively deduces literals $l$ deriving from the current assignment and
updates $\varphi$ and $\mu$ accordingly; this step is repeated until either
$\mu$ satisfies $\varphi$, or $\mu$ falsifies $\varphi$, or no more literals
can be deduced, returning \satres, \conflres and \unknownres
respectively. 
%
In the first case, \dpll returns
\satres. 
In the second case, $\mathtt{analyze\_conflict}(\varphi, \mu)$ detects the
subset $\eta$ of $\mu$ which caused the conflict (\emph{conflict set}) and the
decision level $\mathtt{blevel}$ to backtrack. (This process is called {\em
  conflict analysis}, and is described with more details below.)
If $\mathtt{blevel}$ is
$0$, then a conflict exists
even without branching, so that \dpll returns \unsatres. Otherwise,
$\mathtt{backtrack}(\mathtt{blevel}, \varphi, \mu)$ adds the 
{\em blocking clause} $\neg\eta$ to $\varphi$
(\emph{learning}) and backtracks up to blevel (\emph{backjumping}), 
popping out of $\mu$ all literals whose decision level is greater than
\blevel{}, and updating $\varphi$ %and $\mu$ 
accordingly. 
In the third case, \dpll exits the inner
loop, looking for the next decision.



{\bcp} is based on \emph{Boolean Constraint
  Propagation (BCP)}, that is, 
the iterative application of
{\em unit propagation}: if a unit clause $l$ occurs in $\vi$, then $l$
is added to $\mu$, all negative occurrences of $l$ are declared false and 
all clauses with positive occurrences of $l$ are declared satisfied. 
Current SAT solvers include rocket-fast implementations of \bcp{} based 
on the {two-watched-literal scheme}~\cite{moskewicz01chaff}. 
%

\analyzeconflict{} %and \backtrack{} 
works as follows
(see, e.g., \cite{moskewicz01chaff,zhang01learning}). 
Each literal is tagged with its decision level, that is,
the literal corresponding to the $n$th decision and the literals
derived by unit-propagation after that decision are labeled with $n$;
each non-decision literal 
$l$ in $\mu$ is also tagged by a link to the clause $\psi_l$ causing its
unit-propagation (called the {\em antecedent clause} of $l$). 
%
When a clause $\psi$ is falsified by the current assignment 
---in which case we say that a {\em conflict} occurs and $\psi$ is the
{\em conflicting   clause}--- 
a {\em conflict clause} $\psi'$ is computed from $\psi$ s.t. $\psi'$ contains only 
one literal $l_u$ which has been assigned at the last decision level. 
%
$\psi'$ is computed starting  from $\psi'=\psi$ by iteratively
resolving  $\psi'$ with the antecedent clause $\psi_l$ of
some literal $l$ in $\psi'$ (typically the last-assigned literal in $\psi'$, see
\cite{zhang01learning}), until some stop criterion is met.
%
E.g., with the {\em 1st-UIP Scheme} it is always picked the
last-assigned literal in $\psi'$, and the process stops as soon as
$\psi'$ contains only one literal $l_u$ assigned at the last decision
level;
%with the {\em last-UIP Scheme}, $l_u$ must be the last decision literal;
with the {\em Decision Scheme}, $\psi'$ must contain
only decision literals, including the last-assigned one.

%\newpage
\todo{accennare a clause deleting. Safe clause deleting
  policies, polynomiality\\} 
\todo{accennare ai restarts?\\} 
%\todo{incremental \& unsat-core extraction\\} 
\marg{incremental}
%
Many modern CDCL SAT solvers provide a {\em stack-based 
  incremental interface} (see e.g. \cite{eensorensson:sat2003}), by
which it is possible to push/pop (the blocks of clauses corresponding
to) sub-formulas $\phi_i$ into a stack of formulas
$\Phi\defas\set{\phi_1,...,\phi_k}$, and check incrementally the
satisfiability of $\bigwedge_{i=1}^k \phi_i$. 
%
The interface maintains the {\em status} of the search from one call
to the other, in particular it records the learned clauses.
Consequently, when invoked on
$\Phi$ %$\Phi\defas\set{\phi_1,...,\phi_k}$
the solver can reuse a clause $C$ which was learned during a previous
call on some $\Phi'$ %$\Phi'\defas\set{\phi'_1,...,\phi'_{k'}}$
if $C$ was derived only from clauses %in $\Phi'$
which are still in $\Phi$;~\footnote{%
  provided $C$ was not deleted in the meantime.%
} in particular, if $\Phi'\subseteq\Phi$, then the solver can reuse
all clauses learned while solving $\Phi'$.  \marg{unsat-core}
%
Another important feature of many incremental CDCL SAT
solvers is the capability, when $\Phi$ is found unsatisfiable, of
returning the subset of formulas in $\Phi$ which caused the
unsatisfiablity of $\Phi$. 
%
(This is a subcase of the more
  general problem of finding the {\em unsatisfiable core} of a
  formula, see e.g. \cite{lynce_unsatcore_sat04}.)
Notice that such subset is not unique, and it is not
necessarily minimal. 


==> expeval_sal_disc.tex <==
\begin{stchange}
\STNOTE{Dove lo mettiamo?}

\begin{figure}[t]
  \centering
%
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth,bb=51 50 654 295]{plots_paper/clauses_log.eps}\\
 \end{tabular} 
 \caption{Comparison of the ratio of best configuration of \optmathsat
 (\optlinin{}) to the best configuration of \gams  (\logmipBM on ``\enctwo encoded'' benchmarks) and the number of disjunctions.}
\label{fig:plots_clauses}
%\vspace{-.7cm}
\end{figure}

The figure~\ref{fig:plots_clauses} shows that 
\optmathsat outperforms \gams on SAL benchmarks 
because of the complexity of the formulas.
On LGDP problems \optmathsat and \gams compete, 
but when the number of disjunctions increases
on SAL and SMT-LIB benchmarks,
\optmathsat performs dramatically better.
We believe that this is due to the fact that 
\optmathsat deals with Boolean connectives natively 
and handles the Boolean and the theory-specific
components of reasoning separately, whilst \gams 
tools uses MILP solvers. 

\end{stchange}


==> plan.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PIANO PER SOTTOMISSIONE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\footnotesize
\begin{verbatim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
VENERDI'
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ROBERTO:
** FIRST COMPLETE DRAFT OF SECTION 4 
** FIRST COMPLETE DRAFT OF SECTION 2.2 and 2.3
-------------------------------------------------------------------
SILVIA:
** FIRST COMPLETE DRAFT OF SECTION 2.1
** START SECTION 5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SABATO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ROBERTO:
** FIRST COMPLETE DRAFT OF SECTION 3 
** START SECTION 1
** START SECTION 7 
** START SECTION 6
** REVISED DRAFT OF SECTION 2 
** REVISED DRAFT OF SECTION 4
-------------------------------------------------------------------
SILVIA:
** FIRST COMPLETE DRAFT OF SECTION 5
** REVISED DRAFT OF SECTION 2.1
** FIRST DRAFT OF SECTION 6 (only LGDP) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DOMENICA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ROBERTO:
** FIRST AND REVISED DRAFT OF SECTION 1
** FIRST AND REVISED DRAFT OF SECTION 7
** REVISED DRAFT OF SECTION 3 
** FIRST COMPLETE DRAFT OF SECTION 6 (adding SMT for OPTIM.) 
-------------------------------------------------------------------
SILVIA:
** REVISED DRAFT OF SECTION 5
** REVISED DRAFT OF SECTION 6
** PREPARARE TARBALL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LUNEDI'
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ROBERTO E SILVIA:
- RILEGGERE TUTTO
- SOTTOMETTERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% NOTA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SECTION 6 NECESSARY?
\end{verbatim}
\normalsize


==> plots_paper/lgdp/table_js.tex <==
%\documentclass[12pt]{article}                                                  

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}

{\scriptsize 
\begin{tabular}{|l||r|r||r|r||r|r||r|r||r|r||r|r||r|r|}
\hline
\multirow{3}{*}{Procedure} & \multicolumn{14}{|c|}{Job-shop} \\
\cline{2-15}
  & \multicolumn{2}{|c||}{$I=9,$} 
  & \multicolumn{2}{|c||}{$I=10,$}
  & \multicolumn{2}{|c||}{$I=11,$} 
  & \multicolumn{2}{|c||}{$I=12,$}
  & \multicolumn{2}{|c||}{$I=11,$}
  & \multicolumn{2}{|c||}{$I=11,$} 
  & \multicolumn{2}{|c|}{\multirow{2}{*}{Total}} \\
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=8$}
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=9$} 
  & \multicolumn{2}{|c||}{$J=10$}
  & \multicolumn{2}{|c|}{}\\
\cline{2-15}
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time \\
\hline \hline

\multicolumn{15}{|c|}{Directly Generated Benchmarks} \\
\hline
\optlinof{5} & 100 & 386 & 100 & 1854 & 97 & 9396 & 57 & 14051 & 100 & 9637 & 99 & 10670 & 553 & 45995\\
\hline 
\optlinin{5} & 100  & 317 & 100 & 1584 & 100 & 8100 & 77 & 18046 & 100 &7738 & 100 & 7433 & \best{577} & \best{43228}\\ 
\hline
\optbinof{5} & 100 & 726 & 100 & 3817 & 88 & 13222 & 38 & 12529 & 92 & 14183 & 90 & 13287 & 508 & 57764\\ 
\hline
\optbinin{5} & 100 & 602 & 100 & 3270 & 97 & 12878 & 54 & 16234 &  96 & 13159 & 96 & 12350 & 543 & 58493\\
\hline
\optadain{5} & 100 & 596 & 100 & 3230 & 97 & 12262 & 53 & 14810 & 96 & 12805 & 96 & 12125 & 542 & 55828\\
\hline \hline

\jamsBM & 100 & 268 & 100 & 1113 & 100 & 4734 & 87 & 17067 & 100 & 4941 & 100 & 6122 & \best{587} & \best{34245} \\ 
\hline
\jamsCH & 84 & 23830 & 4 & 1596 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 363 & 89 & 25789 \\
\hline
\logmipBM & 100 & 267 & 100 & 1114 & 100 & 4718 & 87 & 17108 & 100 & 4962 & 100 & 6174 & \best{587} & \best{34343} \\
\hline 
\logmipCH & 84 & 23871 & 4 & 1622 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 338 & 89 & 25831 \\
\hline \hline


\multicolumn{15}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\optlinin{5} & 100 & 324 & 100 & 1571 & 100 & 7739 & 74 & 16494 & 100 & 7175 & 100 & 7504 & 574 & 40807 \\ 
\hline \hline

\multicolumn{15}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline
\optlinin{5} & 100 & 336 & 100 & 1578 & 100 & 7762 & 71 & 16589 & 100 & 7726 & 100 & 7706 & 571 & 41697\\ 
\hline \hline

\multicolumn{15}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\optlinin{5} & 100 & 320 & 100 & 1533 & 100 & 7623 & 68 & 15120 & 100 & 7216 & 100 & 7598 & 568 & 39410 \\
\hline \hline

\multicolumn{15}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\jamsBM & 100 & 239 & 100 & 1128 & 100 & 5516 & 84 & 19949 & 100 & 6667 & 100 & 4176 & \best{584} & \best{37675} \\
\hline
\jamsCH & 100 & 14527 & 46 & 17887 & 0 & 0 & 0 & 0 & 1 & 497 & 0 & 0 & 147 & 32911 \\
\hline
\logmipBM & 100 & 240 & 100 & 1122 & 100 & 5510 & 83 & 19489 &  100 & 6684 & 100 & 4180 & 583 & 37225 \\
\hline 
\logmipCH & 100 & 14465 & 47 & 18206 & 0 & 0 & 0 & 0 & 1 & 495 & 0 & 0 & 148 & 33166 \\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline  
\jamsBM & 100 & 319 & 100 & 1865 & 100 & 12470 & 45 & 15704 & 97 & 13189 & 96 & 15773 & \best{538} & \best{59320} \\ 
\hline
\jamsCH & 95 & 22435 & 18 & 8030 & 2 & 671 & 0 & 0 & 1 & 526 & 3 & 1043 & 119 & 32723 \\
\hline
\logmipBM & 100 & 319 & 100 & 1871 & 100 & 12440 & 45 & 15747 & 98 & 13661 & 95 & 15102  & \best{538} & \best{59140} \\
\hline 
\logmipCH & 95 & 22401 & 18 & 7991 & 1 & 163 & 0 & 0 & 1 & 437 & 3 & 1020  & 118 & 32012 \\
\hline
\end{tabular}
}
%\end{center}
%\end{table}


%\end{document}                                                                 



==> plots_paper/lgdp/table_js_short.tex <==
%\documentclass[12pt]{article}                                                  

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}

{\scriptsize 
\begin{tabular}{|l||r|r||r|r||r|r||r|r||r|r||r|r||r|r|}
\hline
\multirow{3}{*}{Procedure} & \multicolumn{14}{|c|}{Job-shop} \\
\cline{2-15}
  & \multicolumn{2}{|c||}{$I=9,$} 
  & \multicolumn{2}{|c||}{$I=10,$}
  & \multicolumn{2}{|c||}{$I=11,$} 
  & \multicolumn{2}{|c||}{$I=12,$}
  & \multicolumn{2}{|c||}{$I=11,$}
  & \multicolumn{2}{|c||}{$I=11,$} 
  & \multicolumn{2}{|c|}{\multirow{2}{*}{Total}} \\
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=8$}
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=8$} 
  & \multicolumn{2}{|c||}{$J=9$} 
  & \multicolumn{2}{|c||}{$J=10$}
  & \multicolumn{2}{|c|}{}\\
\cline{2-15}
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time \\
\hline \hline

\multicolumn{15}{|c|}{Directly Generated Benchmarks} \\
\hline
\shortoptlinof{5} & 100 & 386 & 100 & 1854 & 97 & 9396 & 57 & 14051 & 100 & 9637 & 99 & 10670 & 553 & 45995\\
\hline 
\shortoptlinin{5} & 100  & 317 & 100 & 1584 & 100 & 8100 & 77 & 18046 & 100 &7738 & 100 & 7433 & \best{577} & \best{43228}\\ 
\hline
\shortoptbinof{5} & 100 & 726 & 100 & 3817 & 88 & 13222 & 38 & 12529 & 92 & 14183 & 90 & 13287 & 508 & 57764\\ 
\hline
\shortoptbinin{5} & 100 & 602 & 100 & 3270 & 97 & 12878 & 54 & 16234 &  96 & 13159 & 96 & 12350 & 543 & 58493\\
\hline
\shortoptadain{5} & 100 & 596 & 100 & 3230 & 97 & 12262 & 53 & 14810 & 96 & 12805 & 96 & 12125 & 542 & 55828\\
\hline \hline

\shortjamsBM & 100 & 268 & 100 & 1113 & 100 & 4734 & 87 & 17067 & 100 & 4941 & 100 & 6122 & \best{587} & \best{34245} \\ 
\hline
\shortjamsCH & 84 & 23830 & 4 & 1596 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 363 & 89 & 25789 \\
\hline
\shortlogmipBM & 100 & 267 & 100 & 1114 & 100 & 4718 & 87 & 17108 & 100 & 4962 & 100 & 6174 & \best{587} & \best{34343} \\
\hline 
\shortlogmipCH & 84 & 23871 & 4 & 1622 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 338 & 89 & 25831 \\
\hline \hline


\multicolumn{15}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\shortoptlinin{5} & 100 & 324 & 100 & 1571 & 100 & 7739 & 74 & 16494 & 100 & 7175 & 100 & 7504 & 574 & 40807 \\ 
\hline \hline

\multicolumn{15}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline
\shortoptlinin{5} & 100 & 336 & 100 & 1578 & 100 & 7762 & 71 & 16589 & 100 & 7726 & 100 & 7706 & 571 & 41697\\ 
\hline \hline

\multicolumn{15}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\shortoptlinin{5} & 100 & 320 & 100 & 1533 & 100 & 7623 & 68 & 15120 & 100 & 7216 & 100 & 7598 & 568 & 39410 \\
\hline \hline

\multicolumn{15}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\shortjamsBM & 100 & 239 & 100 & 1128 & 100 & 5516 & 84 & 19949 & 100 & 6667 & 100 & 4176 & \best{584} & \best{37675} \\
\hline
\shortjamsCH & 100 & 14527 & 46 & 17887 & 0 & 0 & 0 & 0 & 1 & 497 & 0 & 0 & 147 & 32911 \\
\hline
\shortlogmipBM & 100 & 240 & 100 & 1122 & 100 & 5510 & 83 & 19489 &  100 & 6684 & 100 & 4180 & 583 & 37225 \\
\hline 
\shortlogmipCH & 100 & 14465 & 47 & 18206 & 0 & 0 & 0 & 0 & 1 & 495 & 0 & 0 & 148 & 33166 \\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline  
\shortjamsBM & 100 & 319 & 100 & 1865 & 100 & 12470 & 45 & 15704 & 97 & 13189 & 96 & 15773 & \best{538} & \best{59320} \\ 
\hline
\shortjamsCH & 95 & 22435 & 18 & 8030 & 2 & 671 & 0 & 0 & 1 & 526 & 3 & 1043 & 119 & 32723 \\
\hline
\shortlogmipBM & 100 & 319 & 100 & 1871 & 100 & 12440 & 45 & 15747 & 98 & 13661 & 95 & 15102  & \best{538} & \best{59140} \\
\hline 
\shortlogmipCH & 95 & 22401 & 18 & 7991 & 1 & 163 & 0 & 0 & 1 & 437 & 3 & 1020  & 118 & 32012 \\
\hline
\end{tabular}
}
%\end{center}
%\end{table}


%\end{document}                                                                 



==> plots_paper/lgdp/table_js_tot.tex <==
%\documentclass[12pt]{article}                                                  

%\usepackage{multirow}                                                          
%\newcommand{\logmipCH}{\textsc{LogMIP(CH)+CPLEX}}                              
%\newcommand{\logmipBM}{\textsc{LogMIP(BM)+CPLEX}}                              
%\newcommand{\jamsCH}{\textsc{JAMS(CH)+CPLEX}}                                  
%\newcommand{\jamsBM}{\textsc{JAMS(BM)+CPLEX}}                                  
%\newcommand{\optlinin}{\textsc{OPT-MathSAT-Lin-IN}}                            
%\newcommand{\optbinin}{\textsc{OPT-MathSAT-Bin-IN}}   
%\newcommand{\optbinins}{\textsc{OPT-MathSAT-Bin-IN+S2}}                            
%\newcommand{\optlinof}{\textsc{OPT-MathSAT-Lin-OF}}                            
%\newcommand{\optbinof}{\textsc{OPT-MathSAT-Bin-OF}}                            

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}

\begin{figure}[t]
  \centering

%{\scriptsize
\begin{tabular}{|l||r|r|}
\hline
\multirow{2}{*}{Procedure} & \multicolumn{2}{|c|}{Job-shop} \\
\cline{2-3}
  & \#s. & time \\
\hline \hline

\multicolumn{3}{|c|}{Directly Generated Benchmarks} \\
\hline
\optlinof{} & 553 & 45995\\
\hline 
\optlinin{} & 577 & 43228\\ 
\hline
\optbinof{} & 508 & 57764\\ 
\hline
\optbinin{} & 543 & 58493\\
\hline
\optadain{} & 542 & 55828\\
\hline \hline

\jamsBM & 587 & 34245 \\ 
\hline
\jamsCH & 89 & 25789 \\
\hline
\logmipBM & 587 & 34343 \\
\hline 
\logmipCH & 89 & 25831 \\
\hline \hline


\multicolumn{3}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\optlinin{}  & 574 & 40807 \\ 
\hline \hline

\multicolumn{3}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline
\optlinin{} & 571 & 41697\\ 
\hline \hline

\multicolumn{3}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\optlinin{} & 568 & 39410 \\
\hline \hline

\multicolumn{3}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\jamsBM & 584 & 37675 \\
\hline
\jamsCH & 147 & 32911 \\
\hline
\logmipBM & 583 & 37225 \\
\hline 
\logmipCH & 148 & 33166 \\
\hline \hline

\multicolumn{3}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline  
\jamsBM & 538 & 59320 \\ 
\hline
\jamsCH & 119 & 32723 \\
\hline
\logmipBM & 538 & 59140 \\
\hline 
\logmipCH  & 118 & 32012 \\
\hline
\end{tabular}
%}
\caption{Table: results (\# of solved instances, cumulative time in
   seconds for solved instances) for \optmathsat and \gams on 100 
   random samples each of the job-shop problem, 
   for $J=8,9,10$ stages and $I=9,10,11$ jobs.
%
\optbinin{} (right).
\label{fig:plots_js}
}  
%\vspace{-.3cm}
\end{figure}


%\end{center}
%\end{table}


%\end{document}                                                                 



==> plots_paper/lgdp/table_sp.tex <==
%\documentclass[12pt]{article}                                                  

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}
%{\scriptsize

{\scriptsize
\begin{tabular}{|l||r|r||r|r||r|r||r|r||r|r||r|r||r|r|}
\hline
\multirow{4}{*}{Procedure} & \multicolumn{14}{|c|}{Strip-packing} \\
\cline{2-15}
 & \multicolumn{6}{|c||}{$W=\sqrt{N}/2$} & \multicolumn{6}{|c||}{$W=1$} &
 \multicolumn{2}{|c|}{\multirow{2}{*}{Total}}\\
\cline{2-13}
  & \multicolumn{2}{|c||}{$N=9$} 
  & \multicolumn{2}{|c||}{$N=12$} 
  & \multicolumn{2}{|c||}{$N=15$} 
  & \multicolumn{2}{|c||}{$N=9$} 
  & \multicolumn{2}{|c||}{$N=12$} 
  & \multicolumn{2}{|c||}{$N=15$} 
  & \multicolumn{2}{|c|}{} \\

\cline{2-15}
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time \\
\hline \hline 

\multicolumn{15}{|c|}{Directly Generated Benchmarks} \\
\hline  
\optlinof{} & 100 & 53 & 100 & 605 & 94 & 8160 & 100 & 749 & 89 & 3869 & 54 & 5547 & 537 & 18983\\
\hline 
\optlinin{} & 100	& 12 & 100 & 144 & 100 & 3518 & 100 & 173 & 94 & 2127 & 74 & 6808 & \best{568} & \best{12782}\\
\hline 
\optbinof{} & 100 & 50 & 100 & 625 & 89 & 8346 & 100 & 588 & 89 & 5253 & 45 & 5611 & 523 & 20473\\ 
\hline 
\optbinin{} & 100 & 14 & 100 & 211 & 98 & 4880 & 100 & 202 & 94 & 2985 & 65 & 8101 & 557 & 16393\\
\hline
\optadain{} & 100 & 13 & 100 & 192 & 99 & 5574 & 100 & 214 & 94 & 2675 & 63 & 7949 & 556 & 16617\\
\hline \hline
\jamsBM & 100 & 230 & 78 & 10177 & 12 & 1180 & 100 & 158 & 91 & 3878 & 51 & 6695 & \best{432} & \best{22318} \\
\hline 
\jamsCH & 100 & 2854 & 27 & 2393 & 1 & 417 & 100 & 1906 & 70 & 7471 & 17 & 4032 & 315 & 19073\\
\hline 
\logmipBM & 100 & 229 & 78 & 10159 & 12 & 1192 & 100 & 157 & 91 & 3866 & 51 & 6720 & \best{432} & \best{22323} \\
\hline 
\logmipCH & 100 & 2851 & 27 & 2414 & 1 & 424 & 100 & 1907 & 70 & 7440 & 17 & 4037 & 315 & 19073\\
\hline \hline 

\multicolumn{15}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\optlinin{} & 100 & 12 & 100 & 144 & 100 & 3563 & 100 & 183 & 94 & 2169 & 73 & 6466 & 567 & 12537 \\
\hline \hline

\multicolumn{15}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline 
\optlinin{} & 100 & 13 & 100 & 166 & 100 & 5919 & 100 & 195 & 94 & 2156 & 74 & 7080 & 568 & 15529\\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\optlinin{} & 100 & 13 & 100 & 141 & 100 & 5574 & 100 & 172 & 94 & 2148 & 74 & 6650 & 568 & 12618\\
\hline \hline 

\multicolumn{15}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\jamsBM & 100 & 389 & 68 & 8733 & 12 & 1934 & 100 & 162 & 89 & 5565 & 47 & 7313 & \best{416} & \best{24096}\\
\hline 
\jamsCH & 99 & 980 & 46 & 6099 & 2 & 769 & 100 & 726 & 72 & 7454 & 17 & 3505 & 336 & 19533 \\
\hline 
\logmipBM & 100 & 390 & 68 & 8723 & 12 & 1946 & 100 & 163 & 89 & 5547 & 47 & 7299 & \best{416} & \best{24068}\\
\hline 
\logmipCH & 99 & 981 & 54 & 5480 & 12 & 735 & 100 & 725 & 74 & 7433 & 17 & 3542 & 346 & 18896 \\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline  
\jamsBM & 100 & 190 & 81 & 8460 & 11 & 2066 & 100 & 159 & 89 & 2960 & 56 & 8142 & 437 & 21977\\
\hline 
\jamsCH & 98 & 3799 & 24 & 2137 & 1 & 292 & 100 & 2402 & 68 & 7926 & 16 & 3429 & 307 & 19985\\
\hline 
\logmipBM & 100 & 191 & 81 & 8462 & 11 & 2071 & 100 & 159 & 90 & 2964 & 56 & 8206 & \best{438} & \best{22053} \\
\hline 
\logmipCH & 98 & 3807 & 24 & 2133 & 1 & 312 & 100 & 2388 & 68 & 7915 & 17 & 4027 & 308 & 20582\\
\hline 
\end{tabular}
}

%}
%\end{center}
%\end{table}

%\end{document}                                                                 



==> plots_paper/lgdp/table_sp_short.tex <==
%\documentclass[12pt]{article}                                                  

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}
%{\scriptsize

{\scriptsize
\begin{tabular}{|l||r|r||r|r||r|r||r|r||r|r||r|r||r|r|}
\hline
\multirow{4}{*}{Procedure} & \multicolumn{14}{|c|}{Strip-packing} \\
\cline{2-15}
 & \multicolumn{6}{|c||}{$W=\sqrt{N}/2$} & \multicolumn{6}{|c||}{$W=1$} &
 \multicolumn{2}{|c|}{\multirow{2}{*}{Total}}\\
\cline{2-13}
  & \multicolumn{2}{|c||}{$N=9$} 
  & \multicolumn{2}{|c||}{$N=12$} 
  & \multicolumn{2}{|c||}{$N=15$} 
  & \multicolumn{2}{|c||}{$N=9$} 
  & \multicolumn{2}{|c||}{$N=12$} 
  & \multicolumn{2}{|c||}{$N=15$} 
  & \multicolumn{2}{|c|}{} \\

\cline{2-15}
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time \\
\hline \hline 

\multicolumn{15}{|c|}{Directly Generated Benchmarks} \\
\hline  
\shortoptlinof{} & 100 & 53 & 100 & 605 & 94 & 8160 & 100 & 749 & 89 & 3869 & 54 & 5547 & 537 & 18983\\
\hline 
\shortoptlinin{} & 100	& 12 & 100 & 144 & 100 & 3518 & 100 & 173 & 94 & 2127 & 74 & 6808 & \best{568} & \best{12782}\\
\hline 
\shortoptbinof{} & 100 & 50 & 100 & 625 & 89 & 8346 & 100 & 588 & 89 & 5253 & 45 & 5611 & 523 & 20473\\ 
\hline 
\shortoptbinin{} & 100 & 14 & 100 & 211 & 98 & 4880 & 100 & 202 & 94 & 2985 & 65 & 8101 & 557 & 16393\\
\hline
\shortoptadain{} & 100 & 13 & 100 & 192 & 99 & 5574 & 100 & 214 & 94 & 2675 & 63 & 7949 & 556 & 16617\\
\hline \hline
\shortjamsBM & 100 & 230 & 78 & 10177 & 12 & 1180 & 100 & 158 & 91 & 3878 & 51 & 6695 & \best{432} & \best{22318} \\
\hline 
\shortjamsCH & 100 & 2854 & 27 & 2393 & 1 & 417 & 100 & 1906 & 70 & 7471 & 17 & 4032 & 315 & 19073\\
\hline 
\shortlogmipBM & 100 & 229 & 78 & 10159 & 12 & 1192 & 100 & 157 & 91 & 3866 & 51 & 6720 & \best{432} & \best{22323} \\
\hline 
\shortlogmipCH & 100 & 2851 & 27 & 2414 & 1 & 424 & 100 & 1907 & 70 & 7440 & 17 & 4037 & 315 & 19073\\
\hline \hline 

\multicolumn{15}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\shortoptlinin{} & 100 & 12 & 100 & 144 & 100 & 3563 & 100 & 183 & 94 & 2169 & 73 & 6466 & 567 & 12537 \\
\hline \hline

\multicolumn{15}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline 
\shortoptlinin{} & 100 & 13 & 100 & 166 & 100 & 5919 & 100 & 195 & 94 & 2156 & 74 & 7080 & 568 & 15529\\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\shortoptlinin{} & 100 & 13 & 100 & 141 & 100 & 5574 & 100 & 172 & 94 & 2148 & 74 & 6650 & 568 & 12618\\
\hline \hline 

\multicolumn{15}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\shortjamsBM & 100 & 389 & 68 & 8733 & 12 & 1934 & 100 & 162 & 89 & 5565 & 47 & 7313 & \best{416} & \best{24096}\\
\hline 
\shortjamsCH & 99 & 980 & 46 & 6099 & 2 & 769 & 100 & 726 & 72 & 7454 & 17 & 3505 & 336 & 19533 \\
\hline 
\shortlogmipBM & 100 & 390 & 68 & 8723 & 12 & 1946 & 100 & 163 & 89 & 5547 & 47 & 7299 & \best{416} & \best{24068}\\
\hline 
\shortlogmipCH & 99 & 981 & 54 & 5480 & 12 & 735 & 100 & 725 & 74 & 7433 & 17 & 3542 & 346 & 18896 \\
\hline \hline

\multicolumn{15}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline  
\shortjamsBM & 100 & 190 & 81 & 8460 & 11 & 2066 & 100 & 159 & 89 & 2960 & 56 & 8142 & 437 & 21977\\
\hline 
\shortjamsCH & 98 & 3799 & 24 & 2137 & 1 & 292 & 100 & 2402 & 68 & 7926 & 16 & 3429 & 307 & 19985\\
\hline 
\shortlogmipBM & 100 & 191 & 81 & 8462 & 11 & 2071 & 100 & 159 & 90 & 2964 & 56 & 8206 & \best{438} & \best{22053} \\
\hline 
\shortlogmipCH & 98 & 3807 & 24 & 2133 & 1 & 312 & 100 & 2388 & 68 & 7915 & 17 & 4027 & 308 & 20582\\
\hline 
\end{tabular}
}

%}
%\end{center}
%\end{table}

%\end{document}                                                                 



==> plots_paper/lgdp/table_sp_tot.tex <==
%\documentclass[12pt]{article}                                                  

%\begin{document}                                                               
%\title{}                                                                       
%\author{}                                                                      
%\date{}                                                                        
%\maketitle                                                                     

%\begin{table}[t]
%\begin{center}
%{\scriptsize

\begin{figure}[t]
  \centering
{\small
\begin{tabular}{|l||r|r||r|r||r|r||r|r|}
\hline
\multirow{4}{*}{Procedure} & \multicolumn{8}{|c|}{Strip-packing} \\
\cline{2-9}
 & \multicolumn{8}{|c|}{$W=\sqrt{N}/21$ and $W=1$} \\
\cline{2-9}
  & \multicolumn{2}{|c||}{$N=9$} 
  & \multicolumn{2}{|c||}{$N=12$} 
  & \multicolumn{2}{|c||}{$N=15$} 
  & \multicolumn{2}{|c|}{Total} \\
\cline{2-9}
  & \#s. & time 
  & \#s. & time 
  & \#s. & time 
  & \#s. & time \\
\hline \hline 

\multicolumn{9}{|c|}{Directly Generated Benchmarks} \\
\hline  
\optlinof{} & 200 & 802 & 189 & 4474 & 148 & 13707 & 537 & 18983\\
\hline  
\optlinin{} & 200 & 185 & 194 & 2271 & 174 & 10326 & 568 & 12782\\
\hline 
\optbinof{} & 200 & 638 & 189 & 5878 & 134 & 13957 & 523 & 20473\\ 
\hline 
\optbinin{} & 200 & 216 & 194 & 3196 & 163 & 12981 & 557 & 16393\\
\hline
\optadain{} & 200 & 227 & 194 & 2867 & 162 & 13523 & 556 & 16617\\
\hline \hline

\hline  
\jamsBM & 200 & 388 & 169 & 14055 & 63 & 7875 & 432 & 22318 \\
\hline 
\jamsCH & 200 & 4760 & 97 & 9864 & 18 & 4449 & 315 & 19073\\
\hline 
\logmipBM & 200 & 386 & 169 & 14025 & 63 & 7912 & 432 & 22323\\
\hline 
\logmipCH & 200 & 4758 & 97 & 9854 & 18 & 4461 & 315 & 19073\\
\hline \hline

\multicolumn{9}{|c|}{ \renc Encoded Benchmarks} \\
\hline  
\optlinin{} & 200 & 195 & 194 & 2313 & 173 & 10029 & 567 & 12537 \\
\hline \hline

\multicolumn{9}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline 
\optlinin{} & 200 & 208 & 194 & 2322 & 174 & 12999 & 568 & 15529\\
\hline \hline

\multicolumn{9}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\optlinin{} & 200 & 185 & 194 & 2289 & 174 & 10144 & 568 & 12618\\
\hline \hline 

\multicolumn{9}{|c|}{ \encone Encoded Benchmarks} \\
\hline 
\jamsBM & 200 & 551 & 157 & 14298 & 59 & 9247 & 416 & 24096\\
\hline 
\jamsCH & 199 & 1706 & 118 & 13553 & 19 & 4274 & 336 & 19533 \\
\hline 
\logmipBM & 200 & 553 & 157 & 14270 & 59 & 9245 & 416 & 24068\\
\hline 
\logmipCH & 199 & 1706 & 128 & 12913 & 19 & 4277 & 346 & 18896 \\
\hline \hline 

\multicolumn{9}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline 
\jamsBM & 200 & 349 & 170 & 11420 & 67 & 10208 & 437 & 21977\\
\hline 
\jamsCH & 198 & 6201 & 92 & 10063 & 17 & 3721 & 307 & 19985\\
\hline 
\logmipBM & 200 & 350 & 171 & 11426 & 67 & 10277 & 438 & 22053 \\
\hline 
\logmipCH & 198 & 6195 & 92 & 10048 & 18 & 4339 & 308 & 20582\\
\hline 
\end{tabular}
}
\caption{Table: results (\# of solved instances, 
cumulative time in seconds for solved instances) 
for \optmathsat and \gams (using \logmip and \jams) 
on 100 random instances each of the strip-packing problem
for $N$ rectangles, where $N=9,12,15$, and width $W=\sqrt{N}/2$
and 100 random instances with $W=1$.}
\label{fig:plots_sp_all}
%\vspace{-.7cm}
\end{figure}


%\end{document}                                                                 



==> plots_paper/smtlib/smtlib_table.tex <==
%\documentclass[12pt]{article}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

\begin{table}[t]
\begin{center}
{\footnotesize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
Solver & \#inst. & \#term. & \#c.term. & \#c.term.+warn. & \#wrong.term. & \#term.unf. & time\\
\hline
\multicolumn{8}{|c|}{sc}\\
\hline
\optlinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
\hline
\optbinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 108\\
\hline
\optadain{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
\hline
\optlinin{5} \encone & 108 & 108 & 108 & 108 & 0 & 0 & 124\\
\hline
\optlinin{5} \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 121\\
\hline
\jamsBM \encone & 108 & 108 & 107 & 81 & 0 & 1 & 404\\
\hline
\jamsCH \encone & 108 & 108 & 108 & 5 & 0 & 0 & 357\\
\hline
\logmipBM \encone & 108 & 108 & 107 & 81 & 0 & 1 & 407 \\
\hline
\logmipCH \encone & 108 & 108 & 108 & 5 & 0 & 1 & 373\\
\hline
\jamsBM \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 1487\\
\hline
\jamsCH \enctwo & 108 & 82 & 82 & 82 & 0 & 0 & 8537\\
\hline
\logmipBM \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 1490\\
\hline
\logmipCH \enctwo & 108 & 82 & 82 & 82 & 0 & 0 & 8307\\
\hline
\hline
\multicolumn{8}{|c|}{uart}\\
\hline
\optlinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
\optbinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 89\\
\hline
\optadain{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
\optlinin{5} \encone & 36 & 36 & 36 & 36 & 0 & 0 & 89\\
\hline
\optlinin{5} \enctwo & 36 & 36 & 36 & 36 & 0 & 0 & 105\\
\hline
\jamsBM \encone & 36 & 33 & 33 & 12 & 0 & 0 & 253\\
\hline
\jamsCH \encone & 36 & 36 & 0 & 0 & 0 & 36 & 0\\
\hline
\logmipBM \encone & 36 & 34 & 34 & 13 & 0 & 0 & 848\\
\hline
\logmipCH \encone & 36 & 36 & 0 & 0 & 0 & 36 & 0\\
\hline
\jamsBM \enctwo & 36 & 29 & 29 & 29 & 0 & 0 & 3022\\
\hline
\jamsCH \enctwo & 36 & 3 & 3 & 3 & 0 & 0 & 838\\
\hline
\logmipBM \enctwo & 36 & 29 & 29 & 29 & 0 & 0 & 2932\\
\hline
\logmipCH \enctwo & 36 & 3 & 3 & 3 & 0 & 0 & 809\\
\hline
\hline
\multicolumn{8}{|c|}{tta\_startup}\\
\hline
\optlinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 822\\
\hline
\optbinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 732\\
\hline
\optadain{5} & 24 & 24 & 24 & 24 & 0 & 0 & 821\\
\hline
\optlinin{5} \encone & 24 & 24 & 24 & 24 & 0 & 0 & 455\\
\hline
\optlinin{5} \enctwo & 24 & 24 & 24 & 24 & 0 & 0 & 766\\
\hline
\jamsBM \encone & 24 & 8 & 8 & 5 & 0 & 0 & 554\\
\hline
\jamsCH \encone & 24 & 24 & 0 & 0 & 0 & 24 & 0\\
\hline
\logmipBM \encone & 24 & 8 & 8 & 5 & 0 & 24 & 544\\
\hline
\logmipCH \encone & 24 & 24 & 0 & 0 & 0 & 24 & 0\\
\hline
\jamsBM \enctwo & 24 & 11 & 11 & 11 & 0 & 0 & 1432\\
\hline
\jamsCH \enctwo & 24 & 1 & 1 & 1 & 0 & 0 & 32\\
\hline
\logmipBM \enctwo & 24 & 10 & 10 & 10 & 0 & 0 & 870\\
\hline
\logmipCH \enctwo & 24 & 1 & 1 & 1 & 0 & 0 & 33\\
\hline
\hline
\multicolumn{8}{|c|}{TM}\\
\hline
\optlinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 566\\
\hline
\optbinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 518\\
\hline
\optadain{5} & 15 & 15 & 15 & 15 & 0 & 0 & 581\\
\hline
\optlinin{5} \encone & 15 & 15 & 15 & 15 & 0 & 0 & 716\\
\hline
\optlinin{5} \enctwo & 15 & 15 & 15 & 15 & 0 & 0 & 603\\
\hline
\jamsBM \encone & 15 & 14 & 13 & 13 & 0 & 1 & 348\\
\hline
\jamsCH \encone & 15 & 14 & 14 & 10 & 0 & 0 & 201\\
\hline
\logmipBM \encone & 15 & 14  & 13 & 13 & 0 & 1 & 348\\
\hline
\logmipCH \encone & 15 & 14 & 14  & 10 & 0 & 0 & 201\\
\hline
\jamsBM \enctwo & 15 & 13 & 12 & 12 & 0 & 1 & 894\\
\hline
\jamsCH \enctwo & 15 & 12 & 12 & 12 & 0 & 0 & 465\\
\hline
\logmipBM \enctwo & 15 & 13 & 12 & 12 & 0 & 1 & 901\\
\hline
\logmipCH \enctwo & 15 & 12 & 12 & 12 & 0 & 0 & 461\\
\hline
\hline
%\multicolumn{5}{|c|}{miplib}\\
%\hline
%\optlinin & 2 & 0 & 6 & 8 \\
%\hline
%\jamsBM & 0 & 0 & 8 & 8 \\
%\hline
%\jamsCH & 2 & 0 & 6 & 8 \\
%\hline
%\logmipBM & 0 & 0 & 8 & 8 \\
%\hline
%\logmipCH & 2 & 0 & 6 & 8 \\
%\hline
%\hline
\multicolumn{8}{|c|}{sal}\\
\hline
\optlinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optbinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optadain{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optlinin{5} \encone & 10 & 10 & 10 & 10 & 0 & 0 & 463\\
\hline
\optlinin{5} \enctwo & 10 & 10 & 10 & 10 & 0 & 0 & 2\\
\hline
\jamsBM \encone & 10 & 7 & 6 & 5 & 1 & 0 & 2 \\
\hline
\jamsCH \encone & 10 & 10 & 1 & 0 & 0 & 9 & 0 \\
\hline
\logmipBM \encone & 10 & 7 & 6 & 5 & 1 & 0 & 2 \\
\hline
\logmipCH \encone & 10 & 10 & 1 & 0 & 0 & 9 & 0 \\
\hline
\jamsBM \enctwo & 10 & 10 & 6 & 6 & {\bf 4} & 0 & 348 \\
\hline
\jamsCH \enctwo & 10 & 10 & 6 & 6 & 0 & 0 & 38\\
\hline
\logmipBM \enctwo & 10 & 10 & 6 & 6 & {\bf 4} & 0 & 348\\
\hline
\logmipCH \enctwo & 10 & 6 & 6 & 6 & 0 & 0 & 38\\
\hline
\hline
\multicolumn{8}{|c|}{check}\\
\hline
\optlinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optbinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optadain{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optlinin{5} \encone & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optlinin{5} \enctwo & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\jamsBM \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0 \\
\hline
\jamsCH \encone  & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipBM \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipCH \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline 
\jamsBM \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0 \\
\hline
\jamsCH \enctwo  & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipBM \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipCH \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\end{tabular}
}
\caption{\label{table:generalresults}
Encoding1:
Number of solved and correctly-solved problems 
for \optmathsat 
{-BIN-LIN} and   \logmip  and \jams CH/BN, 
on the five groups of smt-lib
  \larat satisfiable  instances.
% ST: i check fanno parte dei benchmark QF_LRA come gli altri
%, plus the ``chack'' instance.
}
\end{center}
\end{table}

%\end{document}


==> plots_paper/smtlib/smtlib_table_tot.tex <==
%\documentclass[12pt]{article}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

%\begin{table}[t]
%\begin{center}
{\scriptsize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Procedure} & \multicolumn{7}{|c|}{SMT-LIB/QF\_LRA formulas} \\
\cline{2-8}
& \#inst. & \#term. & \#correct & \#correct-warn. & \#wrong & \#unfeas. & time\\
\hline
\optlinin{5} & 194 & 194 & 194 & \best{194} & 0 & 0 & \best{1604}\\
\hline
\optbinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1449\\
\hline
\optadain{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1618\\
\hline \hline
\multicolumn{8}{|c|}{ \encone-\renc Encoded Benchmarks} \\
\hline
\optlinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1820\\
\hline \hline
\multicolumn{8}{|c|}{ \enctwo-\renc Encoded Benchmarks} \\
\hline 
\optlinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1597\\
\hline \hline
\multicolumn{8}{|c|}{ \encone Encoded Benchmarks} \\
\hline
\jamsBM & 194 & 171 & 167 & 116 & 1 & 3 & 1561\\
\hline
\jamsCH & 194 & 193 & 123 & 15 & 0 & 70 & 558\\
\hline
\logmipBM & 194 & 172 & 168 & \best{117} & 1 & 3 & \best{2149}\\
\hline
\logmipCH & 194 & 193 & 123 & 15 & 0 & 70 & 574\\
\hline \hline
\multicolumn{8}{|c|}{ \enctwo Encoded Benchmarks} \\
\hline 
\jamsBM & 194 & 172 & 166 & \best{166} & 4 & 2 & \best{7183}\\
\hline
\jamsCH & 194 & 105 & 104 & 104 & 0 & 1 & 9910\\
\hline
\logmipBM & 194 & 171 & 165 & 165 & 4 & 2 & 6541 \\
\hline
\logmipCH & 194 & 105 & 104 & 104 & 0 & 1 & 9648\\
\hline
\end{tabular}
%}
%\label{table:smtlib_generalresults}
%\caption{Results (\# of generated instances, 
%\# of terminated, \# of terminated corrected,
%\# of terminated corrected without warning, \# of terminated
%wrongly, \# of terminated unfeasible) 
%for all the inline versions of \optmathsat and all the \gams tools, 
%on a subset of smt-lib \larat satisfiable instances.
%% ST: i check fanno parte dei benchmark QF_LRA come gli altri
%%, plus the ``chack'' instance.
}
%\end{center}
%\end{table}

%\end{document}


==> plots_paper/smtlib/stat_enc1.tex <==
%\documentclass[12pt]{article}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

\begin{table}[t]
\begin{center}
{\footnotesize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
Solver & \#inst. & \#term. & \#c.term. & \#c.term.+warn. & \#wrong.term. & \#term.unf. & time\\
\hline
\multicolumn{8}{|c|}{sc}\\
\hline
\optlinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
\hline
\optbinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 108\\
\hline
\optadain{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
%\hline
%\optlinin{5} \encone & 108 & 108 & 108 & 108 & 0 & 0 & 124\\
\hline
\jamsBM \encone & 108 & 108 & 107 & 81 & 0 & 1 & 404\\
\hline
\jamsCH \encone & 108 & 108 & 108 & 5 & 0 & 0 & 357\\
\hline
\logmipBM \encone & 108 & 108 & 107 & 81 & 0 & 1 & 407 \\
\hline
\logmipCH \encone & 108 & 108 & 108 & 5 & 0 & 1 & 373\\
\hline
\hline
\multicolumn{8}{|c|}{uart}\\
\hline
\optlinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
\optbinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 89\\
\hline
\optadain{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
%\optlinin{5} \encone & 36 & 36 & 36 & 36 & 0 & 0 & 89\\
%\hline
\jamsBM \encone & 36 & 33 & 33 & 12 & 0 & 0 & 253\\
\hline
\jamsCH \encone & 36 & 36 & 0 & 0 & 0 & 36 & 0\\
\hline
\logmipBM \encone & 36 & 34 & 34 & 13 & 0 & 0 & 848\\
\hline
\logmipCH \encone & 36 & 36 & 0 & 0 & 0 & 36 & 0\\
\hline
\hline
\multicolumn{8}{|c|}{tta\_startup}\\
\hline
\optlinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 822\\
\hline
\optbinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 732\\
\hline
\optadain{5} & 24 & 24 & 24 & 24 & 0 & 0 & 821\\
\hline
%\optlinin{5} \encone%\optlinin{5} \encone & 24 & 24 & 24 & 24 & 0 & 0 & 455\\
%\hline
\jamsBM \encone & 24 & 8 & 8 & 5 & 0 & 0 & 554\\
\hline
\jamsCH \encone & 24 & 24 & 0 & 0 & 0 & 24 & 0\\
\hline
\logmipBM \encone & 24 & 8 & 8 & 5 & 0 & 24 & 544\\
\hline
\logmipCH \encone & 24 & 24 & 0 & 0 & 0 & 24 & 0\\
\hline
\hline
\multicolumn{8}{|c|}{TM}\\
\hline
\optlinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 566\\
\hline
\optbinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 518\\
\hline
\optadain{5} & 15 & 15 & 15 & 15 & 0 & 0 & 581\\
\hline
%\optlinin{5} \encone & 15 & 15 & 15 & 15 & 0 & 0 & 716\\
%\hline
\jamsBM \encone & 15 & 14 & 13 & 13 & 0 & 1 & 348\\
\hline
\jamsCH \encone & 15 & 14 & 14 & 10 & 0 & 0 & 201\\
\hline
\logmipBM \encone & 15 & 14  & 13 & 13 & 0 & 1 & 348\\
\hline
\logmipCH \encone & 15 & 14 & 14  & 10 & 0 & 0 & 201\\
\hline
\hline
%\multicolumn{5}{|c|}{miplib}\\
%\hline
%\optlinin & 2 & 0 & 6 & 8 \\
%\hline
%\jamsBM & 0 & 0 & 8 & 8 \\
%\hline
%\jamsCH & 2 & 0 & 6 & 8 \\
%\hline
%\logmipBM & 0 & 0 & 8 & 8 \\
%\hline
%\logmipCH & 2 & 0 & 6 & 8 \\
%\hline
%\hline
\multicolumn{8}{|c|}{sal}\\
\hline
\optlinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optbinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optadain{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
%\optlinin{5} \encone & 10 & 10 & 10 & 10 & 0 & 0 & 463\\
%\hline
\jamsBM \encone & 10 & 7 & 6 & 5 & 1 & 0 & 2 \\
\hline
\jamsCH \encone & 10 & 10 & 1 & 0 & 0 & 9 & 0 \\
\hline
\logmipBM \encone & 10 & 7 & 6 & 5 & 1 & 0 & 2 \\
\hline
\logmipCH \encone & 10 & 10 & 1 & 0 & 0 & 9 & 0 \\
\hline
\hline
\multicolumn{8}{|c|}{check}\\
\hline
\optlinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optbinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optadain{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
%\optlinin{5} \encone & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
%\hline
\jamsBM \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0 \\
\hline
\jamsCH \encone  & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipBM \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipCH \encone & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline 
\end{tabular}
}
\caption{\label{table:generalresults}
Encoding1:
Number of solved and correctly-solved problems 
for \optmathsat 
{-BIN-LIN} and   \logmip  and \jams CH/BN, 
on the five groups of smt-lib
  \larat satisfiable  instances.
% ST: i check fanno parte dei benchmark QF_LRA come gli altri
%, plus the ``chack'' instance.
}
\end{center}
\end{table}


%\end{document}


==> plots_paper/smtlib/stat_enc1_tot.tex <==
%\documentclass[12pt]{article}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

\begin{table}[t]
\begin{center}
{\footnotesize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
Solver & \#inst. & \#term. & \#c.term. & \#c.term.+warn. & \#wrong.term. & \#term.unf. & time\\
\hline
\multicolumn{8}{|c|}{QFLRA}\\
\hline
\optlinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1604\\
\hline
\optbinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1449\\
\hline
\optadain{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1618\\
\hline
\optlinin{5} \encone & 194 & 194 & 194 & 194 & 0 & 0 & 1820\\
\hline
\jamsBM \encone & 194 & 171 & 167 & 116 & 1 & 3 & 1561\\
\hline
\jamsCH \encone & 194 & 193 & 123 & 15 & 0 & 70 & 558\\
\hline
\logmipBM \encone & 194 & 172 & 168 & 117 & 1 & 3 & 2149 \\
\hline
\logmipCH \encone & 194 & 193 & 123 & 15 & 0 & 70 & 574\\
\hline 
\end{tabular}
}
\caption{\label{table:generalresults}
Encoding1:
Number of solved and correctly-solved problems 
for \optmathsat 
{-BIN-LIN} and   \logmip  and \jams CH/BN, 
on the five groups of smt-lib
  \larat satisfiable  instances.
}
\end{center}
\end{table}


%\end{document}


==> plots_paper/smtlib/stat_enc2.tex <==
%\documentclass[12pt]{article}

%\newcommand{\logmipCH}{\textsc{LogMIP(CH)+CPLEX}}
%\newcommand{\logmipBM}{\textsc{LogMIP(BM)+CPLEX}}
%\newcommand{\jamsCH}{\textsc{JAMS(CH)+CPLEX}}
%\newcommand{\jamsBM}{\textsc{JAMS(BM)+CPLEX}}
%\newcommand{\optlinin}{\textsc{OPT-MathSAT-Lin-IN}}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

\begin{figure}[t]
\begin{center}
{\footnotesize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
Solver & \#inst. & \#term. & \#c.term. & \#c.term.+warn. & \#wrong.term. & \#term.unf. & time\\
\hline
\multicolumn{8}{|c|}{sc}\\
\hline
\optlinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
\hline
\optbinin{5} & 108 & 108 & 108 & 108 & 0 & 0 & 108\\
\hline
\optadain{5} & 108 & 108 & 108 & 108 & 0 & 0 & 116\\
\hline
%\optlinin{5} \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 121\\
%\hline
\jamsBM \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 1487\\
\hline
\jamsCH \enctwo & 108 & 82 & 82 & 82 & 0 & 0 & 8537\\
\hline
\logmipBM \enctwo & 108 & 108 & 108 & 108 & 0 & 0 & 1490\\
\hline
\logmipCH \enctwo & 108 & 82 & 82 & 82 & 0 & 0 & 8307\\
\hline
\hline
\multicolumn{8}{|c|}{uart}\\
\hline
\optlinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
\optbinin{5} & 36 & 36 & 36 & 36 & 0 & 0 & 89\\
\hline
\optadain{5} & 36 & 36 & 36 & 36 & 0 & 0 & 98\\
\hline
%\optlinin{5} \enctwo & 36 & 36 & 36 & 36 & 0 & 0 & 105\\
%\hline
\jamsBM \enctwo & 36 & 29 & 29 & 29 & 0 & 0 & 3022\\
\hline
\jamsCH \enctwo & 36 & 3 & 3 & 3 & 0 & 0 & 838\\
\hline
\logmipBM \enctwo & 36 & 29 & 29 & 29 & 0 & 0 & 2932\\
\hline
\logmipCH \enctwo & 36 & 3 & 3 & 3 & 0 & 0 & 809\\
\hline
\hline
\multicolumn{8}{|c|}{tta\_startup}\\
\hline
\optlinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 822\\
\hline
\optbinin{5} & 24 & 24 & 24 & 24 & 0 & 0 & 732\\
\hline
\optadain{5} & 24 & 24 & 24 & 24 & 0 & 0 & 821\\
\hline
%\optlinin{5} \enctwo & 24 & 24 & 24 & 24 & 0 & 0 & 766\\
%\hline
\jamsBM \enctwo & 24 & 11 & 11 & 11 & 0 & 0 & 1432\\
\hline
\jamsCH \enctwo & 24 & 1 & 1 & 1 & 0 & 0 & 32\\
\hline
\logmipBM \enctwo & 24 & 10 & 10 & 10 & 0 & 0 & 870\\
\hline
\logmipCH \enctwo & 24 & 1 & 1 & 1 & 0 & 0 & 33\\
\hline
\hline
\multicolumn{8}{|c|}{TM}\\
\hline
\optlinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 566\\
\hline
\optbinin{5} & 15 & 15 & 15 & 15 & 0 & 0 & 518\\
\hline
\optadain{5} & 15 & 15 & 15 & 15 & 0 & 0 & 581\\
\hline
%\optlinin{5} \enctwo & 15 & 15 & 15 & 15 & 0 & 0 & 603\\
%\hline
\jamsBM \enctwo & 15 & 13 & 12 & 12 & 0 & 1 & 894\\
\hline
\jamsCH \enctwo & 15 & 12 & 12 & 12 & 0 & 0 & 465\\
\hline
\logmipBM \enctwo & 15 & 13 & 12 & 12 & 0 & 1 & 901\\
\hline
\logmipCH \enctwo & 15 & 12 & 12 & 12 & 0 & 0 & 461\\
\hline
\hline
%\multicolumn{5}{|c|}{miplib}\\
%\hline
%\optlinin & 2 & 0 & 6 & 8 \\
%\hline
%\jamsBM & 0 & 0 & 8 & 8 \\
%\hline
%\jamsCH & 2 & 0 & 6 & 8 \\
%\hline
%\logmipBM & 0 & 0 & 8 & 8 \\
%\hline
%\logmipCH & 2 & 0 & 6 & 8 \\
%\hline
%\hline
\multicolumn{8}{|c|}{sal}\\
\hline
\optlinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optbinin{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
\optadain{5} & 10 & 10 & 10 & 10 & 0 & 0  & 2\\
\hline
%\optlinin{5} \enctwo & 10 & 10 & 10 & 10 & 0 & 0 & 2\\
%\hline
\jamsBM \enctwo & 10 & 10 & 6 & 6 & {\bf 4} & 0 & 348 \\
\hline
\jamsCH \enctwo & 10 & 10 & 6 & 6 & 0 & 0 & 38\\
\hline
\logmipBM \enctwo & 10 & 10 & 6 & 6 & {\bf 4} & 0 & 348\\
\hline
\logmipCH \enctwo & 10 & 6 & 6 & 6 & 0 & 0 & 38\\
\hline
\hline
\multicolumn{8}{|c|}{check}\\
\hline
\optlinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optbinin{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
\optadain{5}  & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
\hline
%\optlinin{5} \enctwo & 1 & 1 & 1 & 1 & 0 & 0 & 0,012\\
%\hline
\jamsBM \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0 \\
\hline
\jamsCH \enctwo  & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipBM \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline
\logmipCH \enctwo & 1 & 1 & 0 & 0 & 0 & {\bf 1} & 0\\
\hline 
\end{tabular}
}
\caption{\label{table:generalresults}
Encoding2: 
Number of solved and correctly-solved problems 
for \optmathsat 
and   \logmip  and \jams CH/BM, 
on the five groups of smt-lib
  \larat satisfiable  instances.
%, plus the ``chack'' instance.
}
\end{center}
\end{figure}


%\end{document}


==> plots_paper/smtlib/stat_enc2_tot.tex <==
%\documentclass[12pt]{article}

%\begin{document}
%\title{}
%\author{}
%\date{}
%\maketitle

\begin{table}[t]
\begin{center}
{\footnotesize 
\begin{tabular}{|l||c|c|c|c|c|c|c|}
\hline
Solver & \#inst. & \#term. & \#c.term. & \#c.term.+warn. & \#wrong.term. & \#term.unf. & time\\
\hline
\multicolumn{8}{|c|}{QFLRA}\\
\hline
\optlinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1604\\
\hline
\optbinin{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1449\\
\hline
\optadain{5} & 194 & 194 & 194 & 194 & 0 & 0 & 1618\\
\hline
\optlinin{5} \enctwo & 194 & 194 & 194 & 194 & 0 & 0 & 1597\\
\hline
\jamsBM \enctwo & 194 & 172 & 166 & 116 & 4 & 2 & 7183\\
\hline
\jamsCH \enctwo & 194 & 105 & 104 & 104 & 0 & 1 & 9910\\
\hline
\logmipBM \enctwo & 194 & 171 & 165 & 165 & 4 & 2 & 6541 \\
\hline
\logmipCH \enctwo & 194 & 105 & 104 & 104 & 0 & 1 & 9648\\
\hline 
\end{tabular}
}
\caption{\label{table:generalresults}
Encoding1:
Number of solved and correctly-solved problems 
for \optmathsat 
{-BIN-LIN} and   \logmip  and \jams CH/BN, 
on the five groups of smt-lib
  \larat satisfiable  instances.
}
\end{center}
\end{table}


%\end{document}


==> rs_macros_colors.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% cambiate in modo da gestire le animazioni
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newcommand{\blue}[1]{\textcolor{blue}{#1}}
% \newcommand{\darkblue}[1]{\textcolor{blue}{#1}}
% \newcommand{\lightblue}[1]{\textcolor{lightblue4}{#1}}
% \newcommand{\red}[1]{\textcolor{red}{#1}}
% \newcommand{\green}[1]{\textcolor{darkgreen}{#1}}
% \newcommand{\lightgreen}[1]{\textcolor{palegreen1}{#1}}
% \newcommand{\violet}[1]{\textcolor{violet}{#1}}
% \newcommand{\darkviolet}[1]{\textcolor{darkviolet}{#1}}
% \newcommand{\darkgrey}[1]{\textcolor{darkgrey}{#1}}
% \newcommand{\palegrey}[1]{\textcolor{lightgrey}{#1}}
% \newcommand{\gray}[1]{\textcolor{gray}{#1}}
% \newcommand{\white}[1]{\textcolor{white}{#1}}
% \newcommand{\black}[1]{\textcolor{black}{#1}}
% \newcommand{\orange}[1]{\textcolor{orange}{#1}}
% \newcommand{\darkorange}[1]{\textcolor{darkorange3}{#1}}
%\newcommand<>{\orange}{\color#1{orange}}

\newcommand<>{\blue}{\color#1{blue}}
\newcommand<>{\darkblue}{\color#1{blue}}
\newcommand<>{\lightblue}{\color#1{lightblue4}}
\newcommand<>{\red}{\color#1{red}}
\newcommand<>{\green}{\color#1{darkgreen}}
\newcommand<>{\lightgreen}{\color#1{palegreen1}}
\newcommand<>{\violet}{\color#1{violet}}
\newcommand<>{\darkviolet}{\color#1{darkviolet}}
\newcommand<>{\darkgrey}{\color#1{darkgrey}}
\newcommand<>{\palegrey}{\color#1{lightgrey}}
\newcommand<>{\gray}{\color#1{gray}}
\newcommand<>{\white}{\color#1{white}}
\newcommand<>{\black}{\color#1{black}}
\newcommand<>{\orange}{\color#1{orange}}
\newcommand<>{\darkorange}{\color#1{darkorange3}}


==> rs_macros_dl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\en}[2]{{#1}e{#2}}
\newcommand{\den}[4]{\en{#1}{#2}/\en{#3}{#4}}

\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\msf}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\snomed}{\textsc{Snomed-CT}\xspace}
\newcommand{\geneonto}{\textsc{GeneOntology}\xspace}
\newcommand{\nci}{\textsc{NCI}\xspace}
\newcommand{\galen}{\textsc{Galen}\xspace}

\newcommand{\shsnomed}{\textsc{Snomed09}\xspace} 
\newcommand{\shnci}{\textsc{NCI}\xspace} 
\newcommand{\shgalen}{\textsc{notGalen}\xspace}
\newcommand{\shfullgalen}{{\textsc{fullGalen}}\xspace}
\newcommand{\shgeneontology}{{\textsc{GeneOnt.}}\xspace}

\newcommand{\conj}{\sqcap}
\newcommand{\disj}{\sqcup}
\newcommand{\exr}[2]{{\exists}#1.#2}

\newcommand{\subs}{\sqsubseteq}
\newcommand{\sups}{\sqsupseteq}
\newcommand{\norm}{\triangleq}
\newcommand{\comp}{\circ}

\newcommand{\topt}{\ensuremath{\top}\xspace}
\newcommand{\bott}{\ensuremath{\bot}\xspace}
\newcommand{\conjt}[2]{\ensuremath{#1 \sqcap #2}\xspace}
\newcommand{\disjt}[2]{\ensuremath{#1 \sqcup #2}\xspace}
\newcommand{\exrt}[2]{\ensuremath{{\exists}#1.#2}\xspace}
\newcommand{\equivt}[2]{\ensuremath{#1 \equiv #2}\xspace}
\newcommand{\subst}[2]{\ensuremath{#1 \sqsubseteq #2}\xspace}
\newcommand{\supst}[2]{\ensuremath{#1 \sqsupseteq #2}\xspace}
%\newcommand{\eqdef}{\stackrel{def}{=}}
%\newcommand{\defas}{\ensuremath{\stackrel{\text{\tiny def}}{=}}\xspace}
 
\newcommand{\pr}[1]{\ensuremath{p_{#1}}\xspace}
\newcommand{\prc}[1]{\ensuremath{p_{[#1]}}\xspace}
\newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
\newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}

\newcommand{\goal}{\ensuremath{C_i\subs_\T D_i}\xspace}
\newcommand{\goalsure}{\ensuremath{C_i~\subs_\T~D_i}\xspace}
\newcommand{\tgoal}[1]{\ensuremath{C_i\subs_{#1} D_i}\xspace}
\newcommand{\igoal}[1]{\ensuremath{{C_{#1} \subs_\T D_{#1}}}\xspace}
\newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
\newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
\newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}

\newcommand{\assumptiongoal}{\ensuremath{\{\neg\prc{D_i},\prc{C_i}\}}\xspace}
\newcommand{\assumptionsgoal}{\ensuremath{\{\neg\sgoal\}}\xspace}

\newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
\newcommand{\wffsubs}{\ensuremath{\phi_{\T{}}}\xspace}
\newcommand{\wffsubsnotrans}{\ensuremath{\phi_{\T{}}^{notrans}}\xspace}
\newcommand{\wffmina}{\ensuremath{\wffsubs^{one}}\xspace}
\newcommand{\wffminarule}{\ensuremath{\phi_{\T(po)}^{one}}\xspace}
\newcommand{\wffminaT}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffminaTrule}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffallmina}{\ensuremath{\wffsubs^{all}}\xspace}
\newcommand{\wffallminarule}{\ensuremath{\phi_{\T{}(po)}^{all}}\xspace}
\newcommand{\wffallminaT}[1]{\ensuremath{\phi_{#1}^{all}}\xspace}
\newcommand{\wffallminaTrule}[1]{\ensuremath{\phi_{#1 (po)}^{all}}\xspace}
\newcommand{\wffallminaO}{\ensuremath{\phi_{\T^*}^{all}}\xspace}
\newcommand{\wffallminaruleO}{\ensuremath{\phi_{\T^*(po)}^{all}}\xspace}

\newcommand{\pinpointingwff}{\ensuremath{\Phi^{\goal}}\xspace}
\newcommand{\pinpointingwffall}{\ensuremath{\Phi^{all}}\xspace}

\newcommand{\hatT}{\ensuremath{\hat{\T}}\xspace}
\newcommand{\Tp}{\ensuremath{\ensuremath{\mathcal{T'}}\xspace}}

\newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}















\newcommand{\el}{\ensuremath{\mathcal{EL}}\xspace}
\newcommand{\elh}{\ensuremath{\mathcal{ELH}}\xspace}
\newcommand{\elp}{\ensuremath{\mathcal{EL^{+}}}\xspace}
\newcommand{\elpp}{\ensuremath{\mathcal{EL^{++}}}\xspace}
\newcommand{\eloh}{\ensuremath{\mathcal{ELOH}}\xspace}
\newcommand{\eqdef}{\stackrel{def}{=}}


% \newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
% \newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}
% \newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
% \newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
% \newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}
% \newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
% \newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}






 

